Impact of Point Spread Function Higher Moments Error on Weak Gravitational Lensing II: A Comprehensive Study

Weak gravitational lensing, or weak lensing, is one of the most powerful probes for dark matter and dark energy science, although it faces increasing challenges in controlling systematic uncertainties as \edit{the statistical errors become smaller}. The Point Spread Function (PSF) needs to be precisely modeled to avoid systematic error on the weak lensing measurements. The weak lensing biases induced by errors in the PSF model second moments, i.e., its size and shape, are well-studied. However, Zhang et al. (2021) showed that errors in the higher moments of the PSF may also be a significant source of systematics for upcoming weak lensing surveys. Therefore, the goal of this work is to comprehensively investigate the modeling quality of PSF moments from the $3^{\text{rd}}$ to $6^{\text{th}}$ order, and estimate their impact on cosmological parameter inference. We propagate the \textsc{PSFEx} higher moments modeling error in the HSC survey dataset to the weak lensing \edit{shear-shear correlation functions} and their cosmological analyses. We find that the overall multiplicative shear bias associated with errors in PSF higher moments can cause a $\sim 0.1 \sigma$ shift on the cosmological parameters for LSST Y10. PSF higher moment errors also cause additive biases in the weak lensing shear, which, if not accounted for in the cosmological parameter analysis, can induce cosmological parameter biases comparable to their $1\sigma$ uncertainties for LSST Y10. We compare the \textsc{PSFEx} model with PSF in Full FOV (\textsc{Piff}), and find similar performance in modeling the PSF higher moments. We conclude that PSF higher moment errors of the future PSF models should be reduced from those in current methods to avoid a need to explicitly model these effects in the weak lensing analysis.

==> processed_comments.tex <==
% %
% %\item In appendix, proof the symmetry of the shear response to moments. This will be useful when we discuss dimensionality reduction somewhere in Section 5. \done
% %
% %\item Mention \textsc{TreeCorr} and \textsc{ngmix}. \done
% %
% %
% %   

% %\rachel{The paper doesn't seem to cite the Schmitz paper.  You should comment on it, especially now that you include more of the higher moment errors in this study than in the previous one.}\tianqing{I have add the reference in the introduction.}

% %\rachel{Some comments on high-level organization:
% %\begin{itemize}
%     %\item It seems like you are missing some (brief) background on weak lensing measurements, because you describe in section 3.2 the biases on WL 2PCF, without really defining those 2PCF or saying how they are measured or explaining their cosmological importance. \done
%     %\item My recommendation would be to turn section two into a `Background' section including some brief material on WL and PSFs followed by the material on PSF higher moments. \done
%     %\item In general, a second paper in a series should extensively reference the previous one.  But I checked the reference list and you seem to not have referenced the first paper even once.  You should identify a place to do that early on and generally refer back to it in other places, e.g., in the simulations section you can comment on how your setup relates to that from the previous paper.
% %\end{itemize}
% %}

% % \begin{tcolorbox}
% % \begin{itemize}

%     % \item Find a way to gain control over the higher moment quantitatively. This involves method to measure the higher moments for a given PSF; change the higher moments given a base PSF; reconstruct PSF given higher moments.  \rachel{Basically done.}
    
%     % \item Answer how individual higher moments error in PSF modeling affect weak lensing shear measurement: How sensitive is shear bias to each higher moments? Is the sensitivity converging to zero when the moments goes higher? Do they cause multiplicative or additive bias? What is the key parameter that determine the sensitivity. Find mathmatical explanation to the image simulation results if possible.  \rachel{Mostly done with perturbed Gaussian simulations, but mathematical explanation is lacking.  Focus on symmetries that may simplify the problem for all shape measurement method, rather than deriving analytical expressions for specific methods and combinations of moments?}
    
    
% %     \item Investigate how the current PSF modeling algorithm do to model the higher moments. Investigate if  there is a higher level connection between the goodness of modeling and other condition (such as seeing, ellipticity etc.) \rachel{Code is set up, but need to increase sample size to draw conclusions.  May need to investigate potential contamination in star sample.}
    
% %     \item Combining the previous two entries, predict the level of shear bias caused by higher moments for the current level in total. \rachel{Have to scope out what's needed to do this.}
    
% %     \item Higher level suggestion for further PSF modeling algorithm. This is based on what the results suggest the future PSF model should focus on. \rachel{TBD} 
    
% %     \item Place requirements on HOME \rachel{TBD}
    
% % \end{itemize}

% % \end{tcolorbox}

% %\rachel{Watch out for how you refer to software.  Example: you refer to \textsc{Piff} in multiple ways.  It is \textsc{Piff}, not PIFF or \textsc{Piff}.  Please clean/homogenize that and look for other packages like \textsc{PSFEx} for which you might need to clean up references.}\tianqing{Done for now, but still need to mention \textsc{TreeCorr} and \textsc{ngmix} in the Method Section.} \tianqing{Mention TreeCorr and ngmix, as well as citation to metacalibration.} \rachel{No, this still needs work.  I still see lots of instances of \textsc{PIFF}, which should be \textsc{Piff} -- these look different both in the tex and the compiled version, and we should use what the \textsc{Piff} paper uses.} \rachel{There are similar issues with \textsc{HealPix} versus Healpix versus healpix.} \tianqing{I think it's \textsc{HEALPix}, and \textsc{healpy} \textsc{numpy} (all lower cases), but sometimes capitalize some letter like \textsc{Astropy} and \textsc{SciPy}. Tricky tricky.}

% %\rachel{We discussed this in a few separate figure captions, so let me bring this here as a top-level statement.  In a few places you mentioned that you felt the labels in figures were large enough, even though not meeting the nominal criterion of `same size as figure text'.  I did want to mention that this is not my criterion - it is one that the MNRAS editors will impose, and they do not in general compromise just because individual authors think it is OK.  So I do encourage you to review the figures with this in mind, and consider whether the labels need to be increased in size.  For some, the text still appears noticeably smaller than the paper text, and since it will not be up to you, it's mostly a question of how much you want to be adjusting the figures now while the scripts are fresh in your mind, versus at the very end of the referee process.}\tianqing{Sorry many small font size texts slipped through. I have made another thorough inspection on the font sizes and adjust some. Only in a few instances the font is still a little bit smaller than the normal text because it will be overcrowded otherwise. }

% %\rachel{I suggest adding a few refs for galaxy-galaxy lensing and a few for cosmic shear, from DES/KiDS/HSC.}\done

% %\rachel{True, but I think it would be appropriate to provide a reference to a more general paper about PSFs and PSF modeling.}\tianqing{Yes, I have added three more reference to the wide-field PSF, instrumental PSF, and PSF interpolation.}

%  %\rachel{I suggest revisiting the wording of this outline.  e.g., it is not true that you do XYZ in section 2 as the text says.  It's just where you provide background.  The methods are not until section 3 and results not until section 4.  }\tianqing{Fixed} 
 
%  %\rachel{Next sentence is missing a statement of where this happens:}\tianqing{Fixed} \rachel{But this makes the outline very strange: Previous sentence and next one start with `In Section 3, we\dots'  Why are they not combined?  An outline should really be quite brief and repeating references to sections is probably unnecessary; or if you do it, there should be clarifying words like `Also in Section 3, we\dots' so it doesn't look too strange.}\tianqing{I change to `We also introduce ...' without mention Section 3 again.} 
 
 
 
% %PSF modeling error can cause weak lensing shear biases. Previous study has focus on quantifying the second moment error of PSF modeling, and come up with a set of formalism to project the error to shear correlation functions bias. 

% %In our previous paper, we stepped into analysis of shear bias that associate with higher moment. We modify PSF to generate light profile that has different radial kurtosis, and observe the relation between the PSF kurtosis modeling bias and the shear measurement bias with image simulations. We also looked at real data to predict the level of shear bias caused by PSF HOME given the current PSF modeling quality. The conclusion is that the kurtosis bias of the current model will cause $0.1 \%$ shear bias. 

% %However, in the last paper, we didn't look at impact from individual higher moment, but as a whole. We didn't have method to change the higher moment as our will so the experiment is less controlled. We didn't cover most higher moment so the conclusion is not complete. 

% %\rachel{You have updated the outline of this section, so you need to update here too.}\tianqing{Fixed}


% %\rachel{I suggest giving the equations and explanations in this section a very careful read to make sure terms are properly defined where they are used and equations are correct.  For example, $u$ and $v$ are used in equation 1 but they are not really defined until equation 6.  Equation 2 seems to be missing a minus sign inside of the exponential.  Equation 2 uses $x_0$ but you do not define or discuss what it means\dots and the other equations and their explanations seem to be missing statements about what you've assumed about the centroid.  And so on - I think this section needs some very careful reading and thinking to check the equations and explanations.  For each equation, examine every symbol and ask yourself whether it is clearly defined in an appropriate place, and consider whether the equation has any assumptions that have not been explained.}\tianqing{I have checked the specification of the equation, the equation order, and unified the symbol.}

% % \rachel{This equation (and some others) will be easier to read with some strategic clean-up.  For example: differentials should use mathrm, i.e. $\mathrm{d}x$.  With a long integral, you should insert some spaces for readability using the math spacing commands (https://www.overleaf.com/learn/latex/Spacing$\_$in$\_$math$\_$mode\#Spaces).  And in general exponents should go on what is being exponentiated, not on its arguments, i.e. $u^p(x,y)$ OR $[u(x,y)]^p$, but not $u(x,y)^p$.  I'm mentioning this here but it's a more general comment that could apply elsewhere.}\tianqing{Alright, I will take care of other equations regarding the spacing and the readability. I removed $(x,y)$ after $u$ and $v$, look much better to me now.} \rachel{To me that is very confusing, because if $u$ and $v$ have the same arguments as $\omega$ and $I$, then you should either show arguments on all of them or none of them.  Showing arguments for some functions but not others might make readers think that the ones without arguments shown don't have arguments.  I really suggest using $u^p(x,y)$ or $[u(x,y)]^p$ rather than $u^p$ etc.}\done


% %\rachel{missing minus sign? $x_0$ undefined?} \tianqing{Fixed}
% %\rachel{inconsistency - before you said it was centered at $(0,0)$}\tianqing{Oh thanks, no need to include the centroid. }

% %\rachel{I suggest suppressing the tick marks and labels, as they are just a distraction - you don't really derive any meaning from them.  And if they are omitted, I think the labels for the basis functions will stand out more.  You should say in the caption how the color scale on each panel is to be interpreted.}
%     %\rachel{I suggest zooming in a little more, as currently the basis functions are shown in the inner 10\% of the panel -- there's a lot of blank space around them.} \tianqing{Doubled the size, same for Fig.~\ref{fig:moment_basis}}
    

% %\rachel{This is notationally confusing, because $\sigma$ provided by that module is not the same $\sigma$ as in Eq.~\eqref{eq:def_sigma}.}\tianqing{Eh, yes. This is not what I use to solve $\sigma$ and $e_1, e_2$. I have updated the definition. }
% % \begin{align}
% %     M_{02} &= \sqrt{ \frac{\sigma^4}{c - (1+c)^2 \,  e_2^2 /4 }   }\\
% %     M_{20} &= c M_{02}\\
% %     M_{11} &= \frac{1}{2} e_2 \, (M_{02}+M_{20}),
% % \end{align}
% % where $c = (1+e_1)/(1-e_1)$ is an intermediate quantity. 
% % \rachel{You seem to switch between $M_{xx}$-type notation for second moments and $M_{pq}$-type notation for moments in general, including second moments -- but you've not said so explicitly.} \tianqing{Sorry! This is an escaped fish - I am going to use $M_{pq}$ throughout the paper.} \rachel{Hmmm, I think what confuses me still is that you've written equation 4-6 in terms of $M_{00}$, $M_{11}$, $M_{01}$.  But the second moments were previously defined with the subscripts summing to 2.  So these cannot be second moments - but from equations 4-6 it seems they must be.  Can you check the section for consistency of second moments?  Also, if I'm right that equations 4-6 need to be fixed, then I think equations 7-9 are simply expressions inverting them - right?  I don't think it's necessary to write the expression and its inverse, you can simply say that you take the measured values of $e_1, e_2, \sigma$ and invert them to get the moments.}\tianqing{Yes, done.}


% %\rachel{In this subsection, you talk about shapelets with just one reference to use of shapelets.  There is a ton of literature on this topic and I think it's worth citing more than one example, even if you do refer to one of them as a comprehensive reference.}\done


% %\rachel{Need to be more precise: is it showing $I(r,\theta)$?  $\psi_{pq}$?}\tianqing{Yes they are $\psi_{pq}$. }. 


% %\rachel{absolute value of the residual?}\tianqing{Yes, fixed} 

% % \begin{equation}
% % \label{eq:def_sigma}
% %     \sigma = \frac{1}{F^{(0)}} \int \mathrm{d}r  r^2 I(\boldsymbol{x}) \omega(\boldsymbol{x}),
% % \end{equation}
% % where $F^{(0)}$, the normalization factor, is the total flux of the light profile. $\omega(\boldsymbol{x})$ is the weight function defined in Eq.~\eqref{eq:def_weight_function}.
% %\rachel{You already defined $\sigma$ in the previous section.  When redefining a symbol, you should ask whether they are the same quantity (in which case could you articulate this as the estimator for a previously-defined quantity?) or different (in which case you should relabel one of them).  Also, I am confused why the integral is not $\int r\, dr\, d\theta$ to integrate over the whole surface brightness profile, or $2\pi r \, dr$ (which would mean you are missing a $2\pi$)?} \tianqing{Sorry, now that I have defined $\sigma$ and $e_1, e_2$ at the previous section, I deleted the ill-defined $\sigma$ here. }



%  %\rachel{My comment about tick labels and color scales from figure 1 applies here too. Also the caption does not have enough explanation to understand what this is. }

% %\rachel{Or they could be a void or any number of specific objects.  I am not sure that naming one specific object is useful here, without indicating that it's an example - it could cause more confusion than anything else.}\tianqing{I have indivated that these are examples.} 


% %\rachel{The formalism you provide is not exclusively for cosmic shear - it can be used for g-g lensing, etc.  This needs some rephrasing.  Perhaps you should say that to describe cosmic shear we need a way to parametrize the lensing shape distortions, and say this is how it is done?} 

% %\rachel{there is no such thing as tangential shear along the x/y axes.  Tangential shear is a term that is reserved for the specific case that you have one object lensing another.  $g_1$ and $g_2$ is simply the shear (not tangential) along the x/y axes}\tianqing{I see, fixed.}, 

% %\rachel{citation needed}\tianqing{Fixed} 


% %\rachel{The logic here feels a bit funny.  What's in section 3.2 sounds like it should go after image simulations and measurements in real data, and perhaps shortly before what's in section 3.5.  Can you check the section ordering?} \tianqing{I have changed the order of the subsection, moving the derivation for weak lensing 2PCF after the real data.}

% %\rachel{Need to give paper reference and mention the relevant section of the paper that defines the material you are summarizing.}\done 

% %\rachel{You sometimes refer to workflow and something workflow.  Should pick and use one consistently.} \tianqing{Yes, change all to ``workflow''.}

% %\rachel{Inconsistency: in later sections, you consider the PSF model to be the one after convolving with the pixel response, since that's what you use for measurements.  Here, you consider the true PSF to be the one before convolving with the pixel response.  Should consolidate language, and I personally encourage you to change this instance to be consistent with what you do later: `The two galaxy profiles are convolved with the true effective PSF, introduced in detail in Section~\ref{sec:psf_profile}; it includes the convolution with a pixel response function ($0.2\arcsec$).  The convolved profiles are then sampled at the centers of pixels, generating the postage stamp images.' }\tianqing{Yes, thanks. Fixed.} 

% %\rachel{I think at this point the RHS should have $\hat{g}$ rather than $g$, since you use the measured shears, right?}\tianqing{Correct, fixed all in the paper.}


%     %\rachel{Text of diagram is too small.  Diagram has typo, `shaplets'.}\tianqing{Increased font size and unified font styles, typo cleared. }

% %\rachel{I am a little confused what the next paragraph is adding.  It seems to describe the same process as the previous paragraph, just giving a little more detail? Such as specifying the use of Metacal/ngmix.  Is there a reason to not simply give those details in the previous paragraph, and omit this one?}\tianqing{Thanks for spotting this. I think we can safely remove the first two sentences and move the Metacal sentence to the previous paragraph. }
%  %\rachel{why true and observed?  True is what you put in the simulation, so I think you only need metacal for observed shear, right?}\tianqing{The shear are indeed evaluated twice to eliminate bias caused by measurement methods. I have removed ``true shear''  and ``observed shear'' here and added another sentence that explains why we estimate shear twice afterward. } \rachel{Yes, understood that you estimate it twice.  But in each case, the truth is the same known value, and what you are getting is the difference between two shear estimates to remove the impact of certain biases.  So I would not call one of them the `true shear', but rather the `shear estimated using the true PSF'.  I see you've made that fix below, but it might make sense to do a search for any other instances that confuse `true shear' versus `estimated shear using the true PSF'.  (And then you can just comment out this thread.)}\tianqing{Yes, I've checked. $\Delta\hat{g}$ is defined in Section~\ref{sec:sim_workflow} correctly.} 
% %We estimate the shear twice -- once with the true PSF and once with the biased PSF -- and take the difference as an estimate of the shear biases associated with the PSF higher moment errors. 

% %\rachel{acronym was not defined}\tianqing{Okay, abandon the BPD } 

% %In real weak lensing surveys, large amount of galaxies are needed in order to measure the coherent shape signal, i.e., the shear. In our image simulation, we avoid this complexity by adapting an approach from \citet{Massey:2006ha}, creating a 90-degree rotated counterpart for each galaxy, before the artificial shear is applied. The original and rotated galaxy are refereed as the 90-degree rotated pair. With the 90-degree rotated pair, shear can be measured per galaxy, as we enforce the average shape to be zero.

% %\rachel{under what conditions?  For astronomical light profiles and large values of $j$?  Convergence is really only a well-defined concept in specific conditions.}\tianqing{Is `Gaussian-like profile' a proper description for ground PSF?}, 


% %\rachel{Need to say what this notation with commas and angle brackets indicates.}\tianqing{I changed this equation to the style of Eq. 13, with different upper limit of $j$.}

% %\rachel{I am confused what this adds to the previous definition of $T_{ij}$.}\tianqing{Nothing. I have removed it. }

% %\rachel{Is there a reason to introduce this new notation with curly brackets?}\tianqing{Nah, you are right I should keep them consistent. }. 

% %\rachel{Should $M_{0j}$ in the numerator be $M_{0i}$?}\tianqing{Yes, fixed.}

%  %\rachel{I'm confused - I thought before you said that the base PSF does not include the pixel response, but the model and true PSFs do include it when we discussed this before.  This sentence seems to say that the model and true PSFs don't include them either?  But then later in the section it says it does.  I think the previous sentence should say `Note that the base PSFs do not include the pixel response function, but the model and true PSFs do include it.' ?}\tianqing{Copy, confirmed.} 

% %\rachel{Note that I fixed this - it said the base PSF was expanded into the shapelets basis, then said that the image includes the pixel response -- but the base PSF by definition does not include the pixel response.  So there were two contradictory sentences.  I have fixed it to emphasize that it's a rendered image including the pixel response that is expanded in the shapelets basis.  Please check/confirm this text.}\tianqing{Confirmed. I have done a search and fixed the rest. } %\rachel{I actually didn't realize this.  Can we discuss this choice and its impact?  It seems to me that if you want to modify the effective PSF model then the simplest thing is to shapelets expand the effective PSF rather than the PSF without pixel convolution.  Are the moment vectors $M$ and $M'$ measured on the effective PSF or is this also without PSF convolution?  The text implies it is the latter but I don't think that's what we want to do.}\tianqing{Ah, my bad, the image expanded is pixel-convolved. I was looking at an old function and got this wrong.  You are right about this, Fixed.} 

% %\rachel{What is meant by `index-free'?  You already used this symbol before, so what is meant to change in this usage?}\tianqing{I have removed this sentence, it did not add any info.}

% %\rachel{That equation has no symbol $\mathbf{\Delta b}$ in it.  Consider homogenizing notation?}\tianqing{Yes, I have homogenize all $\delta$ to $\Delta$ in Section 3.1.3.} 

%  %\rachel{I think we discussed this but I still think the table is ambiguous: is the $\sigma$ given here the measured one of the pixel response-convolved profile?  Or the one you used to instantiate the base PSFs?  I would see this being read either way.}\tianqing{Yeah, sorry this is indeed really confusing. The $\sigma$s here are the ones of the pixel-convoluted (or `effective') PSFs, not the parameters we use to define the base PSF. } 

%  %\rachel{I have commented out the next few sentences because they should really go in the subsubsections below rather than in this preamble - it's a better to keep the details all together and keep this preamble high level.  I've worked those details into the appropriate place.} 
% %The dataset for \textsc{PSFEx} is the star catalog of the HSC public data release \citep[PDR1;][]{2018PASJ...70S...8A}.
% %The dataset for \textsc{Piff} \citep{2021MNRAS.501.1282J} is the HSC Release Candidate 2 (RC2)\footnote{Detailed description of the RC2 dataset can be found in \url{https://dmtn-091.lsst.io/v/DM-15448/}.}, which consists of two HSC SSP-Wide tracts  %\rachel{is it one tract, i.e. `an HSC SSP-Wide tract'?  Or several tracts, i.e., `several HSC SSP-Wide tracts'?  The mix of singular and plural here needs to be fixed.  Below you mentioned use of 3 tracts so I think it should be plural but I wanted to encourage you to check.}\tianqing{It was wrong here, should be 2 wide tracts + 1 ultradeep tract.} 
% %and one HSC SSP-UltraDeep tract. The RC2 dataset is reprocessed biweekly using the latest version of Rubin's LSST science pipelines \citep{2017ASPC..512..279J}.   %\rachel{This definitely needs more explanation.  There is no way somebody outside of Rubin DM will know what this means.}\tianqing{I have added a one-line description to the HSC RC2 dataset at the main text, and a footnote with the URL to the best description I can find online.}
% %
% %
% %

% %dataset %\rachel{unclear why repeated `data\dots for the PSFEx data'?} \tianqing{Wanted to highlight that the PSFEx and PIFF are using different dataset, should say `dataset'. It is sometimes meaningless frankly, I have searched through the text and delete some.}

% %\rachel{This section could be much shorter; I suggest describing the cuts used (or listing them in a table) but you don't need to re-describe all the motivation or provide the table.}\tianqing{I have shorten this section, I think all have left are what these cuts are, and the difference between this and the previous paper. }
% % \rachel{Good job shortening this subsection!  I think, however, that you can do further: the table is unnecessary.  You give the final number of stars in the text, and somebody who really wants to know the minutiae of how important each individual cut is can look at the previous paper (the conclusions don't vary too much by field).} \tianqing{Done.} \rachel{If you remove the table then you have to remove the repeated references to the table in the text (it's there several times as an undefined reference).}

% %The details of the \textsc{PSFEx} modeling and the image coaddition are described in Section~3.3 of \citet{2018PASJ...70S...5B}. %% moved this earlier to get a more logical flow

% %Particularly, for objects with $\code{iblendedness\_abs\_flux} > 0.001$. 

% %Since we use all six HSC fields, we have significantly more stars compared to \citet{2021arXiv210705644Z}. 

% %\rachel{citation needed}\tianqing{This is the same paper as the citation 2 lines above, should I reinstate it?} 

% %\rachel{should not use vague/qualitative and congratulatory language in a journal article}\tianqing{Done}. 

% % \rachel{should `patch' be `tract'?}\tianqing{Yes.}, 
% %\rachel{Let us discuss this dataset in light of the PSF WG telecon - I am pretty concerned.}

% % Reordered text for logical flow: should talk about the images just once, not two separate times.

% %\rachel{You probably already know this, but the $m$ in this section is very confusing, since it's not multiplicative bias (which is what $m$ meant in the previous subsection).}\tianqing{Yes, sorry for the chaos. I have change the moments to $M$ and multiplicative bias to $m$. The moment bias and fluctuation of moment bias are $B[M_{pq}]$ and $\tilde{B}[M_{pq}]$}

% %\rachel{Why is the next sentence here -- should this go in section 2.1 defining the moments, and simply refer to the equations here?}\tianqing{Fair, this sentence should be removed.} 
% %We use the doubly-subscripted notation $M_{pq}$ for the  $p^{\text{th}}$ order moment on the x-axis and the  $q^{\text{th}}$ order moment on the y-axis. 

% %\rachel{In some places you have a subscript `true' and in others, `truth' -- should use search/replace to make these consistent across the paper.}\tianqing{Noted. I have change all subscripts from `truth' to `true'. It is unchanged only when the `truth' is used as a noun . } 

% %\rachel{before you called this `bias fluctuation', not `moment fluctuation' - should adopt terminology and use it {\em consistently}}\tianqing{Fixed and did a search through. } for 

% %\rachel{This implies they are strictly positive.  Is that true?  If not, I would say `the absolute value of the differences\dots'}\tianqing{Fixed} %\rachel{I am not sure about the `are bounded within 10\%' -- do you simply mean that the difference is $\le 10$\%?  If so, I would say that as it's less ambiguous}\tianqing{Yes, the differences for individual galaxies are $\le 10$\%}.

% %\rachel{Is that obvious?  I think that's only true if the discrepancy is a random variable, which I would not necessarily expect.} \tianqing{In our test, we are sampling PSF residual randomly so they are independent samples -- which is not necessary true in a real ensemble of galaxies. So I think it is easier to just state how much ensemble error we get from the test than making statement based on some assumptions. }

% %\rachel{In what's below, I think you don't need to step through quite as much of the math.  I would simply state the assumptions you make along the way, and give a combined result for the shear-shear correlation including both the multiplicative and additive terms.  Also, watch out for placement of tildes on top of quantities with subscripts (they are all misplaced in the text and equations after this point).}\tianqing{I have largely reduce the length of the derivation and fixed the tilde and hat issue. } \rachel{I don't think you even need equations 21 or 23 - just jump to 22 and 24.  But I would suggest going even further and just showing a new equation that shows the combined impact of additive and multiplicative biases (combining what's in 22 and 24).}\tianqing{OK. Done.} \rachel{Hm, OK, you didn't do the combined equation.  Do you have any thoughts on how readers will use these equations after this point?  My concern was that if you have equations 21 and 22, you never have any equation showing the impact of both additive and multiplicative bias together, which is why I was recommending omitting equations 21 and 22 in favor of a single combined equation with both additive and multiplicative bias.} \tianqing{Okay, I though showing additive and multiplicative separately would give more space in explaining each of them. I have combined them in the same expression now. }

% %\rachel{what does superposition mean in this context?}\tianqing{A superposition of two fields sort of? Maybe it's not the appropriate word here.} \rachel{I think it would be more standard to say `they can be written as the sum of the averages and fluctuations'}\tianqing{Fixed} 

% %\rachel{it was suggested in that paper but without explicit demonstration, whereas there is a Massey et al paper that demonstrates this explicitly, so I think you should cite that one instead} \done, 


% %\rachel{I suggest avoiding new terminology such as `moment reduction' (which is used without being explicitly defined).  The term `dimensionality reduction' is a well-understood term in the field, so I suggest you use that (in this subsubsection title and elsewhere in the paper).  You're reducing the dimensionality of the data vector of the moments, but there is nothing particularly special about that requiring a new term.}\tianqing{I have change the term to ``dimensionality reduction (for the PSF moments)''. }

% %We design the following preliminary tests to reduce number of the higher moments. 

% %\rachel{FWHM is an acronym, so it should not be in math mode here or elsewhere.}\tianqing{fixed.}   %\rachel{This is the PSF-convolved size or no?  I think I forgot we had used something so small.}\tianqing{You mean pixel-convolved? The current value is, but still quite small.} . 

% %\rachel{Something to think about in this notation: in the above equation, in one place $g$ means shear, and in another place it refers to galaxy.  Perhaps $\sigma_g$ should be $\sigma_\text{gal}$ throughout the paper to avoid this?}\tianqing{good suggestion, I have changed the $\sigma_g$ to $\sigma_\text{gal}$. } %\rachel{not clear - I see that $\sigma_\text{gal}$ is used in some places in this paper, but in the above equation you've used $\sigma_\text{g}$.}\tianqing{Fixed.}

% %\rachel{Note that $\bar{M}_{pq}$ is not in the equation so it's unclear why it is part of the explanation of this equation?  Also LHS is confusing I think.}\tianqing{Oops, I have fixed the notation. It should be the average of the bias, which is $\langle B[M_{pq}] \rangle$, the LHS is in the average multiplicative of p,q -- in Equation 22.}. \rachel{OK, but the text describing the equation does not talk about $\langle B[M_{pq}] \rangle$, it talks about $\bar{M}_{pq}$ which is not in the equation.  My original comment was that the text needs to be fixed to describe the actual equation, and I think that is still the case.} \tianqing{Okay, sorry I got it wrong. Now it should be fixed. } 

% %\rachel{This language needs work.  `front' and `bottom' are not opposites of each other.  It should either be `front' and `back', or `top' and `bottom'.} \tianqing{Yup, front to back and vice versa sounds good.}

% %\rachel{Need to say what is done if the results disagree - are you inclusive or \dots?} 

% %\rachel{Subsection title is a bit misleading.  This section is not really about the CosmoDC2 catalog. Rather, it's about how you use a synthetic galaxy catalog to estimate certain quantities.  I suggest renaming to reflect the methodology you are communicating about, rather than calling it `CosmoDC2 catalog'.} \tianqing{How about ``Mock Catalog Simulations''?}

% %\rachel{hmm, why first 3 years?  I don't know of any limitation of that sort.}\tianqing{I remember seeing this somewhere, but I couldn't find it now. }. 

% %The base PSF for the mock catalog simulations is a Kolmogorov profile.  %% Sentence is extraneous, given that the rest of the details of the simulated PSF are given below.

% %\rachel{I didn't realize that - I thought you use the shapes in the catalog.  How sensitive are the results to this choice?}\tianqing{The test to support this is in the footnote.}, 

% %\rachel{it looks like linear fits are also shown as lines?}\tianqing{They are all fitted by quadratic functions, just the leading term is zero for the 4\textsuperscript{th} moments. I have added a note at the end. }, 

% %\rachel{The figure is so small that I can't really read it, but I thought you were only showing 3rd and 4th, not 4th and 6th?  The top row is nonlinear so it has to be odd.  Speaking of `so small', this should really be wider than 1 column.  Same for figure 6.}\tianqing{I have fixed the caption for this one and the size for this plot and Figure 5.}  
%   %\rachel{%Unclear what `averaged elliptical' means.  That seems like a {\em very} round disc.  
% %Is the PSF FWHM given here the effective FWHM or the Kolmogorov one?} %\tianqing{It is the average absolute value of the ellipticity.}
% %\rachel{I thought we use shape noise cancellation, so it's not just the shape given in the table but also the version with negative $e_1$ and $e_2$.  Is that right?  If so, should mention that to avoid the table giving the wrong impression about the sims.}\tianqing{I have added a $\pm$ sign for the ellipticities, and addressed the FWHM being the size of the effective PSF}

% % \rachel{Can you comment on your tests of how accurate is the linearity assumption?} \tianqing{It is now commented in the footnote, same for the assumption that constant ellipticity works just fine. }

% %\rachel{another place with inconsistent format - need to search/replace}\tianqing{Fixed} 

% %\rachel{need to use their requested references in the documentation - there are papers to cite and an attribution statement to include}\done 

% %\rachel{next phrase does not make sense, need to fix}\tianqing{Fixed}

% %\rachel{should this be \textsc{HEALPix}?  Can you do a search/replace to get these more systematically?}\tianqing{Yes, done.} 

%  %\rachel{There is nothing to prevent us from evaluating that correlation.  It just won't be accurate because of the smoothing by the pixel size.}\tianqing{Sorry, which correlation?} \rachel{$\langle\tilde{c}_{pq}(\mathbf{x})  \tilde{c}_{uv}(\mathbf{x+\theta})\rangle$ -- you said we cannot evaluate it, but really the issue is that it will be somewhat inaccurate.  This could be fixed, for example, by changing `we are unable to evaluate' to `we cannot accurately evaluate'.}\tianqing{Thanks, fixed.} %\rachel{I don't understand (a) how you can work under the pixel scale or (b) why being able to do so is a disadvantage.  Can you clarify?  Should this say we cannot work below the pixel scale?}\tianqing{Sorry, it should be ``\dots that we are unable to evaluate \dots''.}

% %\rachel{You should comment on how the pixel scale corresponds to the scales we care about for cosmic shear.}\tianqing{I think this is a good place to point to another Appendix needed: sensitivity of cosmology to angular scale, something we investated with the Fisher code. } \rachel{I don't think you need anything nearly that complicated.  Simply state, briefly, what scales are presumed to be used for cosmological analysis in your Fisher matrix, and how that relates to the resolution of your map.}\tianqing{Addressed}


% % \begin{figure*}
% %     \centering
% %     \includegraphics[width=2.0\columnwidth]{plot/additive_multiplicative.pdf}
% %     \caption{A demonstration that additive and multiplicative biases co-exist given $\Delta M_{pq} = 0.005$.  \rachel{Caption needs explanation of the figure: what is being plotted and how does it support the conclusion that you are trying to demonstrate?  My naive reading is that this figure shows only additive bias since all the curves are flat, so I don't really see how it supports the idea that additive and multiplicative biases co-exist.}}
% %     \label{fig:bias_type_moment}
% % \end{figure*}

% %\rachel{$R_2$ is not related to detectability in a direct way - should revisit how this is explained}\tianqing{Change to ``how well-resolved a galaxy is''.},

% %\rachel{Need to say what is done with that - how do you connect that to the science goal of this work.}\done

% %\rachel{I think some of the notation here may need updates -- Husni has been working on his paper and any updates should be propagated here.  I am also fairly skeptical that we need to give a full intro to the Fisher matrix, which is standard machinery used in the field, in this paper.  My recommendation is to reduce this part.}\tianqing{I have updated some notations according to Husni's paper. }

% %\rachel{What is missing is a high-level statement of what analysis are you forecasting?  Is this tomographic shear-shear with 5 bins?  You mention very briefly that the $C_\ell$ is the cosmic shear, but you don't say anything about tomographic binning.  I would personally suggest opening the section with a statement that you are forecasting the impact of the PSF higher moment errors on tomographic shear-shear with 5 bins for the full LSST dataset (Y10), as I think that context will be helpful to any reader as they try to follow the section.} \tianqing{I have reduce a lot of general introduction to the Fisher forecasting and added some high-level description about what the fisher forecasting is serving in our analysis. }


% %The Fisher Information is defined as 
% %\begin{equation}
% %    I(\theta) = \text{Var}(s_\theta (X)) 
% %\end{equation}
% %where $s_\theta (X_i) = \sum_i \frac{\partial log p_\theta(X_i)}{\partial \theta}$ is the score function, $p_\theta(X)$ is the likelihood.
% %The Fisher Information, viewed as the curvature of the log-likelihood, is typically used to construct an asymptotic confidence set on the parameter vector $\theta$ due to the fact that the error in estimating $\theta$, 
% %$\sqrt{n} (\hat{\theta} - \theta)$ converges in probability towards a $\text{Normal}\left(\mu=0,\sigma^2=I^{-1}\right)$

% %\rachel{The entry for $h$ is a bit odd.  Surely you are actually setting $h=0.6727$, but the table entry implies that you are setting $h\times 100 \, \km~s^{-1} \text{Mpc}^{-1}$ to that value?} \tianqing{Yeah, sorry ``$100 \, \km~s^{-1} \text{Mpc}^{-1}$'' is meant to be the unit of $h$, does this make sense now?} \rachel{  No, $h$ is by definition a dimensionless constant, i.e., $H_0\equiv 100h \, \km~\text{s}^{-1} \text{Mpc}^{-1}$.}\tianqing{Oh...} 

% %\rachel{how?  did you do a convergence test or \dots?}\tianqing{I didn't. It seems that Husni did it in his paper.}, 

% %\rachel{Is that an absolute step size, or relative?  If relative, need to explain how you handled parameters with a fiducial value of 0.}\tianqing{That's an absolute step step-size.}

% %\rachel{Is this true for multiplicative bias?  There I thought you simply fit $m(z)$ and then evaluate it at $z_i$ and $z_j$}\tianqing{You are right, the $\Delta \xi$ for multiplicative is directly calculated from $m(z)$ in Eq.~\eqref{eq:multiplicative_tomo}. This line is only for the additive biases.} 


% %\rachel{This equation does not make sense.  If there are $M$ data points and $N$ parameters, then $I^{-1}$ is $N\times N$, $\Delta C_\ell$ is $M\times 1$, $\text{Cov}^{-1}$ is $M\times M$, and $\frac{\partial C_{\ell}}{\partial p}$ is $M\times 1$.  For this to be a mathematically well-defined expression, you would need to make the following changes (at minimum): (1) Take the transpose of $\Delta C_\ell$, so its dimensionality is $1\times M$.  If you do this, then you can multiply it by something that is $M\times M$, otherwise you cannot.  (2) Take a single element of $I^{-1}$ rather than the entire matrix, or make $b_p$ into a vector covering all parameters, so that the left- and right-hand side have the same dimensionality.} \rachel{I was also wondering why the notation is changing.  Before you implied that a specific parameter would be referred to as $p_i$ (in equation 30) and now it doesn't have an index.  I would personally suggest $b(p_i)$ to denote bias of parameter $i$, and $\frac{\partial C_{\ell}}{\partial p_i}$ to denote the derivative of the data vector with respect to a specific parameter $i$.} \rachel{As a final point, I think it will be easier for readers to follow if you were to clearly indicate that 3 of the elements of equation 33 are vectors, and that you have adopted an implicit summation in equations 30 and 33.  This could be done, for example, by using the MNRAS convention in the author guide for indicating vectors and matrices, and/or by including dot product symbols explicitly.}\tianqing{Thanks for the suggestions. The approach I am taking: (1) calculate the bias for one parameter in the equation, and use the convention $B[]$ in this paper to express bias on some variable. (2) Use a sum notation on $j$, I think this makes it clear that only $i$ is left after the summation.}



% %\rachel{I was wondering why you omit the text about priors?  In practice, anybody who sees you are doing a forecast will want to know whether you include any priors, both because it can affect stability of the forecasts and the actual results.} \tianqing{I wasn't even awared that Fisher forecast also has prior information! It is included in the Fisher matrix, so I updated Eq. 30. I have also included all the prior information I use in the Table 3. }
% %We use Gaussian priors on all the parameters. In practice, this is equivalent to adding $\frac{1}{\sigma^2}$ to the diagonal elements of the Fisher information matrix. The are chosen to be uninformative and are added mainly for numerical stability. Priors on the parameters were set to be the same as in the DESC SRD.


% %\rachel{Caption should comment on the plot in some way - what is a key conclusion we should get from this?} %\rachel{Text labels on plot are too small -- probably these cannot be side by side, and need to be wider than they currently are.  Also, need to comment on symlog axis scaling} \tianqing{The box plot and correlation matrix are now separated to two plots. }


% %\rachel{Here you need to provide some justification that this is sufficient to achieve the goals you've outlined for the section (it's not obvious - may need to point to previous paper).}\tianqing{I add two sentences of justification. } 

% %\note{Seems like this paragraph can be put into the method section.} \rachel{I am not so sure about that.  It seems to me that this subsection relies on several complex figures, and it is valuable to provide a clear guide to what you are trying to achieve, without requiring people to flip back to previous sections (though of course the detailed methodology should stay in the method section).  You should then make sure that the rest of the section clearly addresses the two points you've mentioned here as (a) and (b).} \tianqing{I think the points are addressed in this section.}


% %\rachel{We had previously discussed just showing 3rd and 4th moments for some of these figures, and adding a statement that the patterns apply to 5th and 6th.  Reading the text together with the figures, I think that change would be beneficial, as the main points really are captured by the 3rd and 4th moments (and it makes the figures simpler).} \tianqing{Yes, I have change most figure to 3-4th moments and claim the same pattern by text for 5-6th moments.} 

% %\rachel{How does this relate to the galaxy and PSF parameters you talked about in the methods section?  If possible, it would be better to summarize it like `the galaxy and PSF parameters are given in row X of table Y, and there is no weak lensing shear included' or `the galaxy and PSF parameters are given in the Nth paragraph of section such-and-such' rather than listing them again here.}\tianqing{I have created a table, to which we are referring here. } 

% %\rachel{Do you have enough dynamic range in $\Delta M_{p,q}$ for this to be meaningful?  Also, is it really the case that if $\Delta M_{p,q}$ is negative then the shear bias has the same sign as for positive $\Delta M_{p,q}$ (which is implied by a quadratic)?  My concern would be what if it's cubic and you don't quite have the dynamic range to tell, but that would have very different implications for negative signs.  Maybe this is obvious from symmetry considerations and I didn't think it through enough\dots} \tianqing{Goood point! I have make sure that all moments residuals are within this range, and the negative range is newly added. We can see even clearer that the dependences are quadratic. } 

% %\rachel{I think you need some statement like `at fixed $\Delta M_{p,q}$' for this comparison to be meaningful.}\tianqing{Yeah, added in the last sentence.} 

% %\rachel{I suggest `has the opposite sign' rather than `is opposite
% %}\done. 

% %\rachel{ref needed}\done

% %\rachel{Comment on what you would get if you showed them (i.e., anything useful to say about patterns etc.)}\done

% %\rachel{Should there be a $\Delta$ in front of $M_{pq}$?  i.e. this is about the shear bias when you get $M_{pq}$ wrong?}  \rachel{A multiplicative bias of 1--2 is very high, and I did not think you tested the regime where the moments are wrong by 1, so I am a bit confused.} \tianqing{Yeah, the column name should say $\frac{m_{pq}}{\Delta M_{pq}}$. This magnitude is just the derivative, the actual denominator $\Delta M_{pq}$ is at $\sim 0.001$ magnitude, so the multiplicative is not that big.} 
% %\rachel{The next sentence is cut off in the middle and changes to a different sentence after `we apply':}\tianqing{Fixed} 

% %\rachel{shouldn't there be a $\Delta$ in the denominator?} \tianqing{I have made the symbols consistent -- Using $B[M_{pq}]$ as the modeling error}, 

% %\rachel{The plot itself seems to only show additive bias, since the slope appears to be 0.  Should rethink the figure design to achieve your goals here.  I also wonder if you might be better off with e.g. just a table listing the $m$ and $c$ values for this particular experiment for each moment, rather than showing points that you fit to a line?}\tianqing{I have replaced the plot with a table, showing the m and c for third and fourth moments. }

% %\rachel{I'm confused why you choose a different range of radius ratios (which is implied by using $\sigma$ from 0.1--0.9 for Gaussian, but HLR from 0.1--0.9 for Sersic.}\tianqing{Yeah there is no reason for that. Essentially, if we set $R_{2, \text{min}} = 0.3$, we cannot detect anything smaller than 0.2 \arcsec, this set a lower limit to the galaxy size. The upper limit to it needs to cover most of the measurable galaxies in DC2, which is fulfiled by $3 \arcsec$. } 

% %\rachel{That sounds like you are showing examples for individual galaxies.  I suggest saying something like `Examples of moment residual maps across the survey area\dots'.}\tianqing{Thanks, done.}

% % The spatial structure of the PSF moment residuals are important information for modeling the weak lensing systematics associated to the PSF higher-moments error, as shown in Section~\ref{sec:2pcf_deriv}. To measure the spatial correlation, we first shift all the moment residual to zero-averaged fluctuation,
% % \begin{equation}
% % \delta [M_{pq}] (x)  =  B[M_{pq}](x) - \langle B[M_{pq}] \rangle. 
% % \end{equation}
% % We measure the auto- and cross-correlation of all 300 fluctuation-combinations, with scale from $1 \arcsec$ to $200 \arcsec$. These 2PCF data vectors, including their covariance matrices, are gigantic data to visualize and analysis, which further motivate the data reduction that will be elaborated in the next sub-section. 




% %\rachel{Fig.~\ref{fig:correlation_matrix} needs some work; currently it is too large to even show the caption on the page (it is simply missing from the compiled version).  Some suggestions: (1) in the top panel, use a symlog vertical axis, so that you don't need to make the range so wide for just 2 points.  (2) For the bottom plot, consider just showing the 2nd-4th moments, assuming that enough of the patterns are evident.} \done 

% %\rachel{This is a bit confusing, since errorbar is often used for uncertainty on the mean, but here you are using it to denote a range.  I would suggest using a box plot instead, with errorbars indicating the uncertainty on the mean.}\tianqing{Okay, the mean residual is skrinked and log-scaled. } \rachel{I am not sure what you mean by `the mean residual is skrinked'.} \tianqing{Me neither, I don't know what I was saying... So now I am showing the box plot, for PSFEx on pdr dataset and PIFF on the RC2 dataset. }

% %\rachel{Next sentence does not make sense, can you please rewrite?  I am not sure what it is trying to say:}\tianqing{This is a quick consistency check on the bias on the radial kurtosis. I have rewritten. } 

% %We observe that the (0,6) and (6,0) moments are also biased, but differently for the two PSF modeling methods. This finding suggests that the kurtosis is not the sole factor that will contribute to the multiplicative shear bias in practice, as we will further explore in Section~\ref{sec:res:prelim}.  %\rachel{You have not illustrated that the wider range is due to noise.  How do you know it's not some intrinsic variation?}\tianqing{Yes, I don't think the old statement make much sense. I think the utility of this paragraph is to discuss whether the moment error here is matching what we find in the previous paper, so I think it is more important to focus on `it is not just kurtosis, the 6th moments are correlated with them, and do matter` message. }

% %\rachel{You need to say, in words, what this means -- what trend does this indicate, and what does it mean that Piff is doing better?} 

% % Although we have learnt some pattern from looking at the average and correlation function, we have not understood enough about the PSF modeling quality, especially about the spatial pattern, because of the challenge to visualize such high dimensional data vector. In the next sub-section, we will tackle this challenge by reducing the number of moments that actually matter to the weak lensing signal.

% %\rachel{I am not sure the logic of this section makes sense.  YOu start by saying you measured these moments (truth and residual) and their correlation functions.  Then you completely ignore the correlation functions and talk about mean values and correlation coefficients.  So why don't you simply say you measured the moments - mean values and correlation coefficients - and then present results for those quantities\dots and only talk about correlation functions in subsequent sections?}\tianqing{Yes, I think we can just ignore the description of correlation function here, since there is sufficient discription about it in the later subsections where it is used.} \rachel{The last paragraph still talks about correlation functions, so I think whatever changes you made are incomplete.}\tianqing{This section now only talks about average and correlation function of the PSFEx and PIFF data.}


% %\rachel{Plot title `Multiplicative Bias in Preliminary' does not make sense (preliminary is not a noun).}\tianqing{Fixed} %\rachel{I suggest trying a symlog vertical scale.} \rachel{Caption needs some work.  It's not clear how to interpret `preliminary' or how this figure was constructed.  At the minimum, should make clear that this is based on an ensemble.}\tianqing{Yes, I shall help the readers get enough information by just looking at the plots. } \rachel{Caption says this is symlog scale, but it is clearly linear - should the figure be updated? }\tianqing{Yeah, sorry it wasn't updated. }

% %\rachel{not sure what this means, can you clarify?}\tianqing{Sorry `positional-insensitive' means that we just need the average across the field. This is clarified. }. 

% %\rachel{Should be capital M?}\tianqing{Yes} 

% %\rachel{not clear what this means}\tianqing{I used `..be composed by..' instead of `..be composed of..'. It's corrected. } 

% %\rachel{information?  or systematic bias?}\tianqing{systematic bias.} 

% %\rachel{the text on the top two panels is too small}\tianqing{Fixed}  %\rachel{Here too, `preliminary' needs some explanation.  For the top panel, please think carefully about how you can help readers contextualize this signal -- perhaps by comparison with a cosmological signal?  I suggest making the bottom panel have a symlog vertical axis, and putting some horizontal or vertical lines indicating the cutoff points beyond which you consider the moments unimportant.  (Or shaded regions.) } \tianqing{Yeah, I have changed this plot significantly, and add a detailed-caption. I am trying to cover all the basic information by only the caption, so that readers can get what I am doing by just reading the figures and captions. }
%     %\rachel{If you are trying to create contrast then you should not use red and green, as people who are color blind cannot distinguish them.  You should use a color blind-friendly color palette and choose two colors from there.  Also, the text on the top two panels is too small.  Finally, the legends on the top two panels needs significant work.  It's not clear what distinction you are trying to get at with the wording `Remained' vs `Removed'; also the name of the methods used in the text is `back-to-front' and `front-to-back', but here it is different.} \rachel{The caption sometimes uses $\delta$ for quantities that the figure calls $\Delta$.  Should be consistent here and elsewhere.}\tianqing{Clear.}}

% %\rachel{not clear to me what the rest of the sentence means}\tianqing{I have rewritten this sentence.} 

% %\rachel{you list 7, not 5}\tianqing{Fixed} 

% %\rachel{In practice, when will this become relevant?  For a real measurement, we care about $\xi_\pm$ which has contributions from both shear components, so I think you should elaborate on when/how this becomes relevant.}\tianqing{Yeah, the higher moments only impact the $\xi_+$, which is why we only propagate further with $\delta \xi_+$.} \rachel{I think you may have misunderstood my question.  I was reacting to the fact that in your description of figure 10, you say you are showing the additive biases on $\langle g_1 g_1\rangle$ and $\langle g_2 g_2\rangle$ separately -- not combining them to show biases on $\xi_+$.  I was {\em not} arguing that you need to show $\xi_-$; rather, I was arguing that the plot doesn't show the quantity you care about ($\xi_+$) directly.} \tianqing{Okay I see. The $\langle g_1 g_1\rangle$ and $\langle g_2 g_2\rangle$ is shown because it helps the reader understand the two groups. What really matters $\xi_+$ is shown in Figure \ref{fig:add_prelim}. I have re-referred Figure \ref{fig:add_prelim} to address this. }


% %\rachel{This subsection is not really about CosmoDC2; CosmoDC2 is just a tool you use to get a result.  I suggest making the subsection heading reflect the result rather than the tool you use to get the result.}\tianqing{Changed from `CosmoDC2' to  `Testing on Mock Galaxy Catalogs'}

% %Describe how the delta g is calculated for each galaxy (bpd galaxy + generated residual field)

% %Multiplicative bias in DC2 field, redshift dependence


% %\rachel{I think this needs a conclusion, like `Since this seems potentially significant, we have to carry out a forecast of the impact of this redshift-dependent multiplicative bias using the full quadratic formula in Fig.~\ref{fig:redshift_mul}.'?}\tianqing{Added.} %\note{need to be very careful with the conclusion here: if we look at the fitting, the linear dependence is $m_0 \sim 0.1$ per cent, which is very similar with what we found previously.} \rachel{Yeah, I don't think we can draw this conclusion just yet.}\tianqing{Yes, actually, looking at the fisher forecast results for multiplicative biases, the cosmological parameter shift is somewhat consistent with the linear part of m(z).} \rachel{So does this paragraph need to change?}\tianqing{Yes, I have change the conclusion on the multiplicative bias here. }

% %Additive biases in DC2 field, tomographic binning.

%  %\rachel{Should show linear part of the symlog scale with a shaded region.  Also, I'm not convinced you need quite as many data points as you have included -- you could probably rebin by a factor of 2--3, and the figure would look significantly cleaner.}\done 

% % We fit the weak lensing 2PCF additive biases %\rachel{additive biases only?}\tianqing{Yes} 
% % with angular scale using three fitting functions: (a) exponential + constant; (b) exponential; (c) power law. We then transform the real space biases to the Fourier space biases using the wigner transformation. In Fig.~\ref{fig:xi_fitting} \rachel{Do we really need the top panel of this figure, separate from figure 12? How do the points differ?  There are no errorbars on this one, which is certainly a deficiency when assessing fit quality.  So I'm not convinced we need something separate; I think figure 15 could simply show the fit results in addition to data and errorbars.}\tianqing{I think the top panel is important for understand how the data is fitted by three different models, which reflect in different parameter shift in the following plot. Now the points are equipped with errorbar, and we are only looking at $<c_i c_j>$, so the results change a bit.} \rachel{I think I am missing something basic.  I thought that the points in the top of figure 13 are the same as the points in figure 12.  Is that the case or not?  It certainly appears to be the case.  If it is, then we don't need both figures.  If it is not, then the caption to figure 13 should say how these data relate to the data from figure 12.}\tianqing{Yeah, top panel of Figure 13 is the same as Figure 12. With the updated fitting scheme (double-exp.), we can just show Figure 12 for sure.}, we show the three fittings to the additive biases on the 2PCF $\xi_+$, and the resulting cosmological parameters shifts predicted by the Fisher forecasts. We can see that both (a) and (b)  scheme describes the small scale ($\leq 1 \arcmin$) well. However, (b) scheme overestimate the mid-range ($\sim 1 \arcmin$ to $\sim 10 \arcmin$), which is crucial to the cosmology, as shown in Appendix II. At larger scale, (b) scheme tends to fall-off, and (a) scheme levels. The power law (c) scheme remains relatively accurate throughout the entire range. 

% %\rachel{Caption doesn't say what the figure is about.  There is no description of what is causing this shift.} \rachel{I would suggest that you either make the bottom panel wider so it can be read more easily, or show only the cosmological parameters that are easily constrained with weak lensing (omit $n_s$, $h$, $\Omega_b$) so there are fewer panels and the ones that remain are more meaningful and more easily read.} \tianqing{It is wider and the font is larger now. } \rachel{The font is about 3x smaller than the paper text.  It needs to be the same size as the paper text (MNRAS requirement, but also a courtesy to your readers).  If you have to go beyond single-column width and/or omit some of the parameters that are poorly constrained by WL to achieve this, you should do so.}  \rachel{If possible, it would be valuable to put the traditional diagonal panels with the 1D posteriors, and/or make some indication on the 2D plots of the bias to guide the eye (i.e. mark the centers of the contours so the shift is more evident).}\tianqing{I think the font of the labels are big enough to be visible now. The center of the contour are marked with an `x'. I don't think the 1-d contours are necessary because they are all just Gaussian distributions.  }

% %\rachel{What happened to multiplicative biases?  You seem to have focused on the additive ones only, if I understood the text correctly, but it's not clear why.}


% %\rachel{$m_0=0.0005$ for what?  Presumably this is about something from earlier in this paper, but it's not clear where}\tianqing{I have added this to the Method section and refereed to it here.}, 

%  %\rachel{This one has the same aesthetic problem as figure 13.  It's also pretty uninformative.  I would suggest that the text should simply state the magnitude of parameter shifts from this exercise, and omit the figure entirely.} \tianqing{Yeah,I've removed the figure.}

% %\rachel{Subsection is missing a punch line, which I think (?) should be a conclusion that for the current level of PSF higher moment modeling errors in \textsc{PSFEx}, the resulting cosmological parameter biases are caused entirely by additive shear biases and not multiplicative ones.}\done



% % \begin{figure}
% %     \includegraphics[width=1.0\columnwidth]{plot/cosmology_multiplicative.pdf}
% %     \caption{The shifts on cosmological parameters caused by the redshift-dependent multiplicative biases $m(z)$. The parameter shifts are much subtle than the ones caused by the additive biases, if untreated. }
% %     \label{fig:cosmology_mul}
% % \end{figure}


% % We also spend some effort analyzing the shear bias caused by the 3rd moment in an optical perspective. We express the Coma $Z_3^{1,-1}$ and Trefoil $Z_3^{3,-3}$ in terms of the third moments, 

% % \begin{align}
% %     &Z_3^1 = m_{30} + m_{12}\\
% %     &Z_3^{-1} = m_{21} + m_{03}\\
% %     &Z_3^3 = m_{30} - 3 m_{12}\\
% %     &Z_3^{-3} = 3 m_{21} - m_{02}.
% % \end{align}

% % By modifying the third moments, we can modify a single component of Coma or Trefoil. In Figure \ref{fig:coma_trefoil_mc}, we can see that the shear bias caused by coma and trefoil is additive. We can also notice that the coma can cause more trouble to $g_1$ than others. This is within expection because the coma causes an asymmetry between the x-axis and y-axis: a common cause for the $g_1$ bias. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=1.0\columnwidth]{plot/coma_trefoil_mc.png}
% %     \caption{Shear bias response to the 3rd, 4th, 5th and 6th PSF moments. }
% %     \label{fig:coma_trefoil_mc}
% % \end{figure}

% % \section{Real Data Higher moment}

% % \subsection{HSC maps}

% %\rachel{Should this phrase say something about the odd moments?  I thought it was going to be about ignoring the odd moments compared to the even ones, but the sentence doesn't mention `odd'.}\tianqing{You are right. I missed a few words in the sentence, feels like I was having a blackout.} 

% %\rachel{Need to say something about correcting for any second moment errors.}\done 

% %\rachel{`two datasets' is vague, needs clarification}\done. 

% %\rachel{This paragraph needs context.  Is this here because you view this as a prerequisite to assessing which moments are needed to do tests of cosmological parameter recovery?} \tianqing{Add a one line motivation for doing preliminary tests. }

% %\rachel{Which parameters?}\tianqing{Looking at the Fisher forecast, it's all parameters. }

% %\rachel{MNRAS convention is to put the references before appendices.}\done

% %\rachel{Need to review this for papers that are actually published.  For example the GalSim paper for some reason is a reference to arxiv rather than to the published version.  Should update that and any others that are published.}\tianqing{I have looked at all the arXiv that we are referring, and updated all those with a published version.}

% % Note from Rachel: for the figure numbering to be done properly in the appendix, the figures have to go after a specific appendix has been defined.  That's why I moved up this section heading.



% %\rachel{This appendix really lacks a narrative to hold it together.  I have tried to flag places where you could put text to improve this, but I encourage you to generally consider how to clearly indicate what you are doing at each step.}\tianqing{Yeah, sorry that this section was pooly described. It should look much better now. }


% %\rachel{In what's below, you sometimes refer to $M_1$ or $M_2$, and sometimes to $M_{pq}$.  Should clarify what the two different notations are indicating.}\tianqing{Fixed}


% %\rachel{should these be $\Delta\hat{g}$ for consistency with the equation below?}\tianqing{Fixed} 


% %\rachel{should this be $M_{pq}(x,y)$?}\tianqing{Fixed} 

% %\rachel{should this be $M_{pq}(x,y)$?}\tianqing{Fixed} 

% %\rachel{You've now defined four theorems, but it is not at all obvious what is happening next.  You should introduce each new step in your explanation clearly and say what you are doing.}\done

% %\rachel{In the bullet points below, should all the $M$ be $M_{pq}$, for consistency with the rest of the section?}\tianqing{Fixed}

% %\rachel{This sign implies there is a convention, but you haven't stated the convention.  What direction is a positive/negative rotation?}\tianqing{Fixed}

%     %\item $\mathcal{R}''(M(x,y)) = M(-x,-y)$ -- a function to rotate by $180^\circ$.  \rachel{This one is not used for the entire rest of this appendix; is it needed?}\tianqing{good point, it was used before but not now, so I can take it out. }


% %\rachel{Here too, you need to say what you are doing.  Why are you introducing these cases, what are you trying to do?}\done

% %\rachel{Please check/confirm previous sentence.  I thought it is important to explicitly articulate the lessons here.}\tianqing{That is absolutely correct.}
% %\rachel{Should the $m$ be $M$?}\tianqing{Fixed}


% %\rachel{Correct me if I am wrong, but we kind of knew this had to be true from case 2?  If so, should comment on the connection between these cases.}\tianqing{Yeah, they are extremely similar. We always flip the coordinate on the even axis.}


% % \rachel{Here too, it is not clear where you are going or what you are trying to do here:} We can also operate on $y$:
% % \begin{equation}
% %     M_{qp}(x,y) = M_{pq}(y,x) = -M_{pq}(-y,x) = - \mathcal{R}'(M_{pq}(x,y)).
% % \end{equation}

% %\rachel{Why are the $M$'s now $m$'s?}\tianqing{Fixed}

% %\rachel{Should $m$ be $M$?}\done

% %\rachel{You should comment on how this relates to what you see in figure 4.}\done

% %\rachel{A Jacobian is a matrix that relates two things to each other.  The text needs to say what two specific things are being related by this Jacobian.}\tianqing{Fixed} 

% %\rachel{of what?}\tianqing{Fixed} 


% %\rachel{of what?}\tianqing{Fixed}
% %\rachel{of what?}\tianqing{Fixed} 
% %\rachel{coefficients?}\tianqing{Fixed}, 
% %\rachel{Not clear what this means.  It looks like a $12\times12$ matrix}\tianqing{Fixed. It starts from the second moments} 

% %\rachel{Not clear what this means.  I see the top row has a value with magnitude -1.0 and one with -0.06, so it seems like the maximum magnitude is 1.0.  I see another row that has values -0.01, 0.71, -0.71, so it's not clear to me in what sense this is normalized to 1.}\tianqing{The $L^2$ norm is normalized to 1. $T_ij$ is rounded to the second digits, so $\sqrt{1-0.06^2} = 0.998$ is rounded to 1.0...} 
%     The sizes of the circles %\rachel{of what?}\tianqing{Fixed} 
% %\rachel{What are the numbers on the figure?  The Jacobian entries?}  \rachel{The red and blue make the numbers unreadable.  Need to work on the aesthetics.}\tianqing{Fixed} 
%     %\rachel{Should the labels on the figure be $M$ rather than $m$?}
% %\rachel{Need to explain what are the images shown on the left column and bottom row.}\done  %\rachel{Figure needs a takeaway message.}\tianqing{Fixed}
%  %\rachel{Consider your readers who are skimming through figures - you should say in words what $T_{ij}$ is (briefly) so they can derive some understanding of the figure without carefully reading the entire text to find the explanation.}
% %\rachel{as per MNRAS convention, you should move the figure definition into this appendix so that it is labeled figure C1}\tianqing{Fixed}, 
% %\rachel{not clear what this last phrase means}\tianqing{Does this make sense now?}. 

% %\rachel{Not clear what this means.  It looks like a $12\times12$ matrix}\tianqing{Fixed. It starts from the second moments} 
% %\rachel{Not clear what this means.  I see the top row has a value with magnitude -1.0 and one with -0.06, so it seems like the maximum magnitude is 1.0.  I see another row that has values -0.01, 0.71, -0.71, so it's not clear to me in what sense this is normalized to 1.}\tianqing{The $L^2$ norm is normalized to 1. $T_ij$ is rounded to the second digits, so $\sqrt{1-0.06^2} = 0.998$ is rounded to 1.0...} 
% %\rachel{of what?}\tianqing{Fixed} 
% %\rachel{What are the numbers on the figure?  The Jacobian entries?}  \rachel{The red and blue make the numbers unreadable.  Need to work on the aesthetics.}\tianqing{Fixed} 
%     %\rachel{Should the labels on the figure be $M$ rather than $m$?}
% %\rachel{Need to explain what are the images shown on the left column and bottom row.}\done  %\rachel{Figure needs a takeaway message.}\tianqing{Fixed}
% %\rachel{Consider your readers who are skimming through figures - you should say in words what $T_{ij}$ is (briefly) so they can derive some understanding of the figure without carefully reading the entire text to find the explanation.}

% %\rachel{as per MNRAS convention, you should move the figure definition into this appendix so that it is labeled figure C1}\tianqing{Fixed}, 
% %\rachel{not clear what this last phrase means}\tianqing{Does this make sense now?}. 

% %\rachel{Need some takeaway here.  Also need to enlarge font in the figure so it's the same size as the font in the main text.  Finally, the caption and figure say different moments -- the figure says (0,4) and (4,2), while the caption says (1,3) and (4,2).  Should check and make sure they are consistent.} %\rachel{Consider moving example to the appendix?}\tianqing{Yup, it is in the appendix, and referred to in the main text. }  


% %\rachel{Appendix is not referred to from the text - should find a suitable place to do that.}\tianqing{Add the reference of this appendix in Section~\ref{sec:dc2_method} and Section~\ref{sec:res:dc2}}

% %\rachel{HSC has 6 fields - should this be `HSC survey data' or a specific, named HSC field?}\tianqing{They are from all six fields, specified.} 
% %\rachel{language here may also need updating - it's not clear what `the HSC field data' means}\tianqing{Fixed}
% %\rachel{of what?}\tianqing{fixed}
% %\rachel{The figure is impossibly tiny.  Remember the font/labels need to be the same size as the text in the paper, and you may need to modify the figure size or the figure itself to achieve this and also show the features you are trying to show.} \tianqing{Sorry, it's now enlarged. Also fixed the labels and legend.} \rachel{To me the text in the figure is still a lot smaller than the text in the paper.  I think you need to make both panels larger and have one on top and the other on the bottom, with the figure taking up a full page.}\tianqing{With our comments taken away, the caption should fit in the page okay.} 

% % figure of generation field
% %\rachel{This next part is a technical digression, which I suggest you put into an appendix with title like `Generating PSF higher-moment residual maps'.} 
% % \rachel{as per MNRAS convention, you should move the figure definition into this appendix so that it is labeled figure D1}\done, 

% %\rachel{You cannot assume that people will go straight from the appropriate section of the text to here, and refer to groups without defining them.}\tianqing{Fixed}. 
% %\rachel{Need to say where these functional forms come from!}\done \rachel{I was actually looking for a much more basic and high-level statement that these are purely empirically determined fitting formulae based on visual inspection.  That was still missing, so I have now added it.}\tianqing{I see, thanks.}






% %\rachel{what process is being alluded to here?  You do a Hankel transform?  Should be specific.} 
% %\rachel{Your readers are new to this project, so you need to connect the dots: why are you doing all this stuff?  Why can you not just use the HSC survey data for this?  You have to walk through the logic.}\tianqing{I add a couple of sentenses in this paragraph and the previous one to walk through the whole story.} 
% %\rachel{What is being referred ot here?  The inherent resolution limit of the \textsc{HEALPix} grid you've used?}\tianqing{Referring to the \textsc{HEALPix} pixel scale, fixed.} \rachel{So it's not a cutoff -- that generally implies that you have made a cut, not that you have used a grid with limited resolution.  Should reword accordingly.}\tianqing{Fixed}, 



% %\rachel{what does excessive mean here?  that's a comparative term - it's excessive compared to something, so what is the something?  the WL requirements on shear bias?  or do you just mean there was {\em excess} bias in addition to the 2nd moment formalism predictions?  also i think it's relevant that this is for a space telescope -- i.e. the context of that study differs from yours}\tianqing{Excess bias in addition to the 2nd moment formalism predictions} 


% %\rachel{citation}\tianqing{Done, also added this citation at other positions.}, 
% %\input{desc-tex/ack/standard} 


% %\bibliographystyle{mnras}

% %\rachel{Reading this, I think we have some sections out of place.  I thought that section 2 was `background' and 3 was `methods' but the content of section 2.3 is a method developed for this paper.  Are those out of place?}\tianqing{Yes, section 2.3 should be a method. The reason I put it in this section is for continuity purposes. I have moved moment-shapelet relation to Section 3 and refer to 2.1 and 2.2 in it. } \rachel{OK, thanks, but then it should not be mentioned in an outline of section 2!}\tianqing{Fixed}


% %\rachel{why is that not true for $n=2$?}\tianqing{Fixed. We are presenting 2\textsuperscript{nd} moment differently, but that doesn't affect the moment definition.}  %\rachel{Should say explicitly what values $p$ and $q$ can take.}\done 

% %\rachel{I don't understand what it means - all profiles have a shape, you can define it based on the second moments.}\tianqing{It should be ``zero second moment shape''.} 

%  %\rachel{$\sigma$, $e_1$, and $e_2$ have not been defined, however.  Need to either define them or say how/where they will be defined.}\tianqing{Fixed} 


% %\rachel{Need to use consistent notation; you are switching between $\mathbf{M}$ and $\boldsymbol{M}$, which look different in the compiled PDF.  Should pick one and stick to it throughout the paper.}\tianqing{Change all $\boldsymbol{M}$ to $\mathbf{M}$.}

% %\rachel{below you use $b_{pq}$ in contrast to here where it is $b_{p,q}$ -- need to be consistent throughout the paper}\tianqing{Fixed},

% %\rachel{of what?}\tianqing{fixed}\rachel{I don't understand the above statement - the x axis of the pixel grid is generally fixed.  I thought you were going to say it is the polar angle of the major axis defining the shear direction}\tianqing{Nah, I was thinking how to align the $g_1, g_2$ notation with the $g_+, g_\times$ notation. I think it's best not to bring in this extra quantity.}\rachel{OK, so I think all that's left is to say what xy axis you are talking about - what is this coordinate system?} 


% %\rachel{I understand you've tried to simplify terminology by not defining both $(g_1, g_2)$ and $(g_t, g_\times)$.  But the problem is that it means Eq.~\eqref{eq:2pcf_def} is incorrect; $\xi_\pm$ is defined in terms of the latter, not the former as you've currently written.} \tianqing{Yeah, it is tricky. I think that I should define $(g_t, g_\times)$ before I define $\xi_\pm$, since that's what happening inside \textsc{TreeCorr}. } \rachel{Yes, I think that is necessary.}\tianqing{Defined underneath here.}

% %\rachel{if it is a vector, it should be $\boldsymbol{\theta}$}\tianqing{Fixed} 

% %\rachel{Hmm, this is notationally a little weird.  Typically in MNRAS vector quantities are bold, so a vector would be $\boldsymbol{\theta}$ and $\theta$ would already be a scalar.}\tianqing{So it should be $\xi_\pm (\theta)$  and $\boldsymbol{\theta}$}

% %\rachel{citation needed, and need to say what the requirement means in a technical sense}\tianqing{Fixed.}\rachel{What you added is useful, but it is not what I meant.  What does it mean that there is a requirement on the upper bound of something?  Does it mean that if the quantity exceeds the requirement, nobody can do science with that dataset?  Or\dots?}\tianqing{Yes, I need to elaborate the message in \citep{2013MNRAS.429..661M}. By accident, I also realize that our $m_{\text{total}} = 0.001$ (or 1/3 of the budget), should only cause $0.1\sigma$ in cosmology. Because the error budget is set at $0.3 \sigma$. } \rachel{Not everybody sets it the same way.  I'm not sure it's worth focusing on the precise numerical choices made in Massey et al, because different surveys have different strategies for defining the numerical values of requirements with respect to statistical uncertainties. I would suggest avoiding those details. Rather, I was hoping you could comment on the {\em conceptual} meaning of `requirements' consistent across all studies -- i.e., that you must reduce the residual systematic uncertainty to below a certain level, or you must explicitly include that systematic in your model when performing the cosmological analysis.  Not everybody is familiar with this concept and so it is worth stating.}\tianqing{Ok, I changed the text a little bit so that it is not specific to the criteria chosen in the paper. But I think `systematic biases must not exceed a certain portion of the statistical error in order to remain correct overlap between ideal and reported constraints' is generally correct, yes?} \rachel{no, let's talk - it's more like `systematic biases must not exceed a certain portion of the statistical error in order to remain correct overlap between ideal and reported constraints {\em without explicitly modeling that source of bias}' - i.e., failing some requirement doesn't mean your result is always biased, it means you have to account for and model that bias rather than pretending it doesn't exist}\tianqing{Okay, I have added `{\em without explicitly modeling that source of bias}' to the statement.}. 

% %\rachel{Hmm, let me check.  You've written $\Delta g'$ in the numerator, no hat, so this is the true value, i.e., 0.01.  It seems to me that the numerator then includes both additive and multiplicative bias generated by the changes in PSF higher moments, which we don't want.  I think you have to remove the additive bias by making the numerator $\Delta \hat{g}' - \Delta \hat{g}$?  Can you please check this and, if I am right, fix the equation / plots / tables / etc.?}\tianqing{You are correct. I have checked all $\Delta g$ and make them $\Delta \hat{g}$, etc.}

% %\rachel{Has $R$ been defined?}\tianqing{Fixed}

% %\rachel{You already talked about 90 degree rotated pairs in the previous subsubsection about the overall workflow, so perhaps this entire paragraph can be omitted?  You could simply insert the reference to Massey et al and one sentence about reducing simulation volume through this approach into that previous subsubsection. }\tianqing{Yup.} \rachel{where is the sentence inserted earlier?  i can't find it} \tianqing{Sorry now it's there.}

% %\rachel{not clear what `shapelet moment' means - should this be `the coefficient of a shapelet basis function as defined in equation 8'?}\tianqing{Fixed}. 

% %\rachel{Why is notation changed from subscript $ij$ to $k \times q$?  I am not used to subscripts being used to indicate dimensionality and I don't think it is common notation.  I would suggest just saying `we need to calculate the Jacobian $T_{ij}$ with shape $k\times q$' or something like that. }\tianqing{Nah, I am trying to indicate the shape of the matrix by $k\times q$, it's not needed as long as I say what the sizes are. }

% %\rachel{$M_{0i}$ is ambiguous notation: you want it to mean `initial value of moment $i$' but since you sometimes use $M_{pq}$ for moments, it looks like it could be a specification of $p=0$.  I suggest changing this notation to avoid the ambiguity.}\tianqing{Yes, I think it is not necessary to say the moments are initial, since T can be calculated at any stage. So I just changed $M_{0i}$ to $M_i$} \rachel{OK, but your notation for $b_j$ is also inconsistent.  Above you said it was starting with $b_j$ but the next line refers to $b_{0j}$ etc.  I think the next sentence needs to say $b_j' = b_j + \Delta b_j$, no?}\tianqing{Done} 

% %\KwResult{Write here the result }

% %\rachel{Should the condition in the `while' loop use the L$^2$ norm, i.e., $|\mathbf{\Delta M}|_2$?  It was introduced but not used, and I think if you are introducing it then it should appear in this algorithm.}\tianqing{Yeah, make sense, fixed. }
% %\rachel{A few comments on this formalism: first, you write $|\mathbf{\Delta M}|$.  This notation is confusing because it could either be a vector with entries equal to the absolute value of the entries in the $\mathbf{\Delta M}$ vector -- or, it could be the length of the vector, i.e., $|\mathbf{\Delta M}| = \sqrt{\mathbf{\Delta M}^T \cdot \mathbf{\Delta M}}$.  The notation is therefore ambiguous as to whether you do this test entry-wise, or for the total length of the vector. I suggest clarifying this.  Second, I suggest defining a symbol rather than putting $threshold$ in math mode, i.e., `$< t_0$ (threshold value)', and you can use the symbol in the text to more concretely connect to the algorithm.  Third, I think that the $\mathbf{\Delta m}$ in the algorithm should be $\mathbf{\Delta M}$.}
% %\tianqing{I have changed the notation in the Algorithm and in the text as follow: (1) We have used $B[M_{pq}]$ through out the paper to represent the biases on the higher moments, so I assign it here to the `target moment change'. (2) In Section 3.1.3, we use $\Delta M$ as the desired moment change in \textit{one iteration}, which is equivalent to `difference of the target and current moments' in this Section. So I made them the same notation. }

% %\rachel{should this be the target moment bias vector $\mathbf{\Delta M_0}$?}\tianqing{Your original comment is correct. Now that I have changed the notation, it should be $B[\mathbf{M}]$.} 

% %\rachel{I feel this does not precisely define how you got the images in that figure.}\tianqing{Moved this paragraph from Section 3.1.3 to here.} \rachel{This still doesn't say how those images are constructed.  Is it that you had some default PSF, then you modified one moment, and took the difference between the modified and original image?}\tianqing{Add {\em `by taking the difference between the images before and after one moment is slightly biased'}.}

% %\rachel{Notation change: in many cases it's $M_{pq}$ but here there is a comma.  Should homogenize format (search/replace other instances too).}\done \rachel{no, it is still inconsistent}\tianqing{Okay, I have searched ``p,q'' and make sure there is none of them in the text, and looked through the figures. }

% %\rachel{Should comment briefly on how this compares with the \textsc{PSFEx} star selection: is it much higher density?}\tianqing{Resolved.}

% %\rachel{Should the $\sum_{pq} \langle m_{pq}\rangle$ be replaced by $\langle m_\text{total}\rangle$, in which case the next sentence might not be needed?}
% %\tianqing{Yeah, we can also remove the $\langle \rangle$ for the multiplicative bias, just $m_{\text{total}}$. }

% %\rachel{It might be useful to clarify how this can come about: it's because the response to a given PSF higher moment depends on the galaxy properties, so the galaxy ensemble in each tomographic bin might respond differently to the same level of PSF higher moment error.}\tianqing{Yes, added. } 

% %\rachel{Is there a reason to switch notation from $m_\text{total}$ to just $m$ as you've done here?  I could understand using $m_{pq}$ if you want to focus on specific moments, but when talking about the total I think it would be better to maintain consistent notation.}\tianqing{Fixed here and in Results Section.}

% %\rachel{How was the $\sigma$ measured?}\tianqing{It is the pre-PSF second moment sigma, fixed. } \rachel{How did you measure the pre-PSF second moment sigma?}\tianqing{It is the size before our (atmospheric PSF), but after the Optical PSF of the Hubble ST. I change the text to make this clear.} 

% %\rachel{this number 41,000 is oddly specific but unexplained}\tianqing{Define the ensemble and update the actual numbers} 

% %\rachel{Should there be a $1/N$ to indicate you're taking the average $\partial g/\partial M_{pq}$ across the sample?  Should $g$ be $\hat{g}$?  How does this equation get rid of the additive biases associated with $M_{pq}$, which will also enter into the estimated shear?} \tianqing{Sorry, I have changed $g$ to $m_{pq}$. The multiplicative biases are measured with two shears -- $g$ and $g'$, and $m$ is estimated by $(\hat{g'} - \hat{g})/ (g' - g) B[M_{pq}^{-1}]$. This is totally non-trivial, so I have added a description in Section~\ref{sec:sim_workflow} and refer to it here. }

% %\rachel{for what range of $\theta$?}\tianqing{Fixed.}. 

% %\rachel{That previous sentence seemed like a notation change.  In equation 12 you called it $\Delta \hat{g}/B[M_i]$.  Should be consistent in notation and refer back to that equation if possible, otherwise carefully consider and explain notation change.}\tianqing{I have change all the $M_i$ to $M_{pq}$ except for the Jacobian derivation part, since there $M$ is treated like a vector so it makes more sense to use one index.} 

% %\rachel{What happens to those that are outside the grid?}\tianqing{The uncovered galaxies are all large galaxies, and they are discarded from the ensemble. } 

% %\rachel{Grid is linear in all of these dimensions?}\tianqing{Yup.} 

% %\rachel{Should the x axis be $B[M_{pq}]$ rather than $\Delta M_{p,q}$?  Should the y axis be $\Delta\hat{g}$ rather than $\Delta g$?  I'm not sure the notation is currently consistent with the paper.}  \rachel{Put a dotted black line at $\Delta g=0$ for reference?}\tianqing{Fixed and checked consistency for $M_{pq}$ for text and other plots.}\tianqing{Also change how order or magnitude is displayed in this plot, is this better?} \rachel{The y axis label is very small and it's really hard to see that the two rows have 3 orders of magnitude difference.  I would suggest explicitly calling out in the caption something like `As indicated in the y-axis labels, the orders of magnitudes in the additive shear biases are very different for the two rows.'  (Same suggestion applies to other figures with this issue.)}\tianqing{Yeah, it is easy to misread the message here. }

% %\rachel{I think there was a big gap in the narrative.  I have tried to fill it in with a new phrase here, but please check this carefully for accuracy.}\tianqing{Thanks, I think they are exactly right. } 

% %\rachel{4th?}\tianqing{Fixed}

% %\rachel{What is the change in colors and legend ordering in the top and bottom panel meant to signify?  To me it's not obvious, and I think it might be better for top and bottom panel to use consistent colors and legend ordering.  Also, should consistently use accent on Sersic (currently the legend in one panel uses it and the other does not).} \rachel{y axis in one panel has $M_{pq}$ and in another, $M_{p,q}$.  Should be consistent.} \rachel{x axis labels are also inconsistent between the top and bottom panels; should unify.} \rachel{Conceptual concern/question: is this plot consistent with figure 4?  There, it seemed that 4th moments generated larger shear responses than 3rd moments. Here, the m's and c's for 3rd and 4th moments appear to be comparable orders of magnitude.}\tianqing{Sorry this is confusing: there was a little $\times 10^3$ on the top of the first row, which means the axis is multiplied by 1000. Now I have removed that and just multiply the third moment responses by 1000 (100 for multiplicative), and change their y-label to $\dots \times 10^3$ ($\dots \times 10^2$ for multiplicative). Fixed $M_{pq}$. Unify the color and show legend once. Fixed S\'ersic accent. Also add a y=0 reference line here. }

% %\rachel{notation consistency?}\tianqing{I have changed all $\partial g$ to $\partial \hat{g}$}

% %\rachel{But you aren't simulating each galaxy.  So how do you do this cut in practice?  Estimate $R_2$ for each grid point, estimate it for a given galaxy via interpolation, and cut on the estimates?}\tianqing{Yes, exactly. I have added a footnote here.} 

%  %\rachel{citation/explanation needed}\done,

% %\rachel{I personally think it would be more meaningful/useful to give a number density than a total number; people would probably relate to it more.}\done \tianqing{Should} \rachel{That number is very high, by maybe a factor of 2.  Are you sure this is what you get for all of cosmoDC2 with those cuts, after accounting for the ~450 sq degree area?  It seems inconsistent with other papers.}\tianqing{For some reason I always thought the area is 300 sq degree. Now the density is reduced. } \rachel{The DC2 image simulations are 300 sq deg but cosmoDC2 is larger.}

% %For each galaxy used, we obtain its true shear $g$, and apply multiplicative and additive biases by linearly interpolating its properties in the simulation grid. In the case of additive bias, we generate the observed shear $\hat{g}$ by,
% %\begin{equation}
% %\label{eq:g_obs_add}
% %\hat{g} = g + \sum_{pq} \frac{\partial c_{pq}}{\partial M_{pq}} B[M_{pq}],
% %\end{equation}
% %where $B[M_{pq}]$ is the PSF model bias on $M_{pq}$, and $c_{pq}$ is the additive bias associated with $M_{pq}$. \rachel{Weren't those terms already defined?} In the case of the %multiplicative bias, similarly, the observed shear is,
% %\begin{equation}
% %\label{eq:g_obs_mul}
% %\hat{g} =  (1+ \sum_{pq} \frac{\partial m_{pq}}{\partial M_{pq}} B[M_{pq}])g,
% %\end{equation}
% %where $m_{pq}$ is the multiplicative bias associated to $M_{pq}$. \rachel{Already defined?} 

% %\rachel{Based on what - true redshift, photo-z, \dots?}\tianqing{It's the true redshift.} 

% %\rachel{Since you mention these IA parameters in words and give symbols in Table~\ref{tab:cosmology_parameters}, I think you need to say where does the model come from.  Without giving a reference, it's not obvious how one should interpret the $A_0$ etc.  The ref to Husni's paper in prep does not suffice because readers cannot review it -- you would need to cite the paper that defines this IA model.} \tianqing{I have cited the NLA model, and briefly describe what the parameters are. A quantitative definition of them are not needed here?} \rachel{The linear alignment model in that paper doesn't have the parameters you are using (it's not nonlinear and it doesn't have the same redshift dependence etc.).  You should cite a paper that uses that actual parameterization, so readers can refer to it for a precise model definition, and then no more information is needed here.}\tianqing{Is this one okay? I don't find the high redshift parameter here though. } \rachel{No, it's not correct.  As a rule, if you are using the same model as some paper, you should cite that specific paper, or follow the papers it cites until you have the right one.  So: look at the DESC SRD, which you are following very closely in your modeling.  It says it uses the IA model formulation from section 4.4 of a Krause \& Eifler paper.  Therefore that paper defines your model, and it is the one you should cite.}\tianqing{Change to Krause \& Eifler. } 

% %\rachel{I just noticed the fiducial model has zero intrinsic alignments.  Can you remind me why that is the case?  There are intrinsic alignments in reality, and the forecast for the impact of PSF modeling errors may depend on location in parameter space (because IA looks like an additive shear term, just like the PSF higher moments).}\tianqing{This is an error, I have re-run the Fisher code with $A_0 = 5.0$ and no redshift dependency, same as Husni's setup. }

% %\rachel{if this is a purely empirical fitting function then should say so, and mention how well it fits the data}\tianqing{Done.} 

% %\rachel{This equation is now significantly improved, thanks.  However, the $I_{ij}^{-1}$ is ambiguous: it could be interpreted as `take the inverse of the Fisher matrix, then take the $ij$ element' -- or, it could simply be the reciprocal of the $ij$ element of the Fisher matrix.}\tianqing{It is the former one. I add a parenthesis to $I^{-1}$.} \rachel{Your new notation in this equation is fine but you need to propagate it in the rest of the text, i.e., there should be no more $b_p$ in the rest of the paper since you have removed that quantity in favor of $B[p_i]$.  This is a general statement: whenever you edit the notation in an equation, you need to look for impacts in the paper text and figures.}\tianqing{Copy.}

% %\rachel{In the last round you started introducing a notation $\sigma_p$ instead of $\sigma$ for uncertainties.  I would like to discourage this -- you've used $B[p_i]$ for the bias on parameter $i$.  But $\sigma_p$ doesn't specify anything; it's presumably the uncertainty on a parameter, but not a specific one (wouldn't that be $\sigma_i$ or $\sigma(p_i)$)?  So the additional subscript doesn't seem to have a purpose.  I tried to eliminate these and simply leave it at uncertainty $\sigma$ but might have missed some. Alternatively you could use a notation specific to parameter $i$.}\tianqing{That's fine, I have change other $\sigma_p$ to $\sigma$}

% %\rachel{It looks like there are some moments for which the IQR is very different for the two methods: (4,0), (0,4), (6,0), (0,6).  Does this deserve a comment?} \tianqing{I have added the comments.}

% %We experiment with $3^{\text{rd}}$ to $6^{\text{th}}$ moments, with $(p,q)$ shown on top of each sub-plot. 

% % \rachel{notational consistency: no comma in subscript?}\tianqing{Fixed},

% %\rachel{This is very confusing, because figure 4 shows that the 3rd moments have significant additive bias, while the table says they have only multiplicative bias and no additive bias.  Can you clarify how these are consistent?}\tianqing{I have addressed in Figure 4 about the order-of-magnitude confusion. I hope it is now a bit more clear.}  \rachel{Another thing I am not sure about: when the responses are nonlinear, how did you determine the numbers in the table?  I mean, for a linear response it doesn't matter, but if the response is quadratic then you would get a different value for this ratio depending on your fiducial assumption about the typical PSF moment residual.}\tianqing{Yes, the response is nonlinear to the 3\textsuperscript{rd} moments. The value in this table is computed by the average PSF moment residuals.}

% % \rachel{Please check table 4 caption; I have some basic methodology questions here.}\tianqing{Yes, it is addressed in Table 4. }  

% %\rachel{The way you refer to this ratio here is not the same as in the figure itself.  Should be consistent.} \tianqing{The notation in the figure is aligned to this one now. }

% %\rachel{I don't think this is the average $ \langle B[M_{pq}]\rangle$ -- I thought it was a box plot showing the distribution of the $B[M_{pq}]$ values.  If it's an average, what is the average taken across, and how do you still have a distribution to show a box plot?}\tianqing{Yes, fixed here and in the plots. } 
% %\rachel{No, this paper did not compare \textsc{Piff} and \textsc{PSFEx} so cannot be used as a supporting citation for the statement that both are positive.  Need to rearrange the sentence if you want to say the results for \textsc{PSFEx} (only) are qualitatively similar to that paper.}  \tianqing{Change to `as observed for \textsc{PSFEx} in ...'.}

% %\rachel{Please see previous sentence, which I have added as I think it's a key point.}\tianqing{Thanks for adding this, I find it extremely hard for me to write constructive criticism in the paper. } 

% %Future \textsc{Piff} development should include these critical 4\textsuperscript{th} and 6\textsuperscript{th} moments as part of the modeling and interpolation schemes. \rachel{Previous sentence implies that the two methods may produce different 3rd and 5th moments, but that does not appear to be true.  Also, please see my comments in the figure caption for potential discrepancies worth discussing for 4th and 6th moments.}\tianqing{Yes, the result is changed. I have change the description here.}  
% %The radial kurtosis can be expressed as 
% %\begin{equation}
% %    \rho^{\text{(4)}} = M_{04} + M_{40} + 2 M_{22}.
% %\end{equation}
% %\rachel{should not have commas in subscripts for consistency with rest of paper in the above equation?}
% %As a consistency check, we have confirmed that the average bias on the radial kurtosis  $B[\rho^{\text{(4)}}] \approx 0.004$ may be obtained from the $B[M_{pq}]$ as in the above equation for \textsc{PSFEx}, consistent with the findings of \citet{2021arXiv210705644Z}. \rachel{Is this a non-trivial check since you have moved from using one HSC field to all 6?}

% %\rachel{I think you need some commentary on the \textsc{Piff} results as suggested by Mike on Slack.}\tianqing{Yeah, I have added a few sentences at the end of the last paragraph.  }

% %\rachel{I am a bit confused by this: when I look at true vs residual as suggested by the previous sentence (i.e. the off-diagonal blocks) I see  negative correlations, not positive ones.  It's only true-true and residual-residual that seem to have the kind of positive correlations you mentioned resulting in the pattern you are flagging.  Can you check the language here?  Perhaps it should be `The true moments with a same parity for both $p$ and $q$ are usually positively correlated, and likewise for the residuals.'}\tianqing{Thanks, I meant what you have proposed.} 

% %\rachel{Should the y axis be $m_{pq}$?  Legend should have 1 and 2 as subscripts.  I'm not sure that the plot title needs `in Preliminary Tests' for the reasons I've outlined in a comment on the subsection title (I think it's quite confusing since you had some tests before this that could also be considered preliminary).}\tianqing{Fixed y label, title and subscripts. True, the previous test is using a single galaxy and this one using COSMOS, but both can be considered preliminary.}

% %\rachel{Next sentence does not seem to be describing this figure:}\tianqing{Fixed} 

% %\rachel{But the COSMOS population is not Gaussian - need some clarification}\tianqing{Yeah, we use them as the input of second moment size. }, 

% %\rachel{should this be $\hat{g}$?  And how to remove the additive bias associated with $M_{pq}$ from this? (same questions as for Eq.~\ref{eq:multiplicative_approx})}\tianqing{Change to $\partial m_{pq}/\partial M_{pq}$}. 

% %\rachel{notation change; shouldn't this be $\langle B[M_{pq}]\rangle$?}\tianqing{Fixed}. 

% %\rachel{That's not what the figure says?}\tianqing{Fixed.}. 

% %\rachel{I think you have to remind the reader here that you do this for one moment at a time and always with second moment residuals set to zero?}\done 

% %\rachel{I am fairly lost about where the 22 comes from.}\tianqing{22 higher moments.} \rachel{But the previous paragraph talked about only needing 11?  So in the narrative flow, I don't understand why we went from 22 to 11 and then back to 22.}, 

% % \rachel{it is scale dependent, so I'm not sure this is that meaningful unless you specify that's on tens of arcmin scales?}\tianqing{Fixed} 

% %% RM: next line commented because it seemed redundant with remarks above
% %This shows that the additive shear biases associated with PSF higher moment errors significantly affect the $\xi_+$ component of the weak lensing 2PCF. 

% %\rachel{Sometimes you call this ``$g_1$ group'' and sometimes ``group-1'' and sometimes `group-1'.  Should homogenize, and likewise for the other component.}\tianqing{Fixed} 

% %\rachel{But in real life, we want to use $\xi_\pm$, which depends on $g_t$ and $g_\times$, linear combinations of $g_1$ and $g_2$.  So I am not sure this point is very important in practice?  For each galaxy we'll need to assign $c_1$ and $c_2$ to get the total systematic bias in $\xi_\pm$.}\tianqing{Right. I remove the point that this 11 moments can be further reduce.}

% %\tianqing{I add this transitional paragraph, and move the description of Figure 10 to the former text, where additive biases on 2PCF are just introduced. }

% %\rachel{Should y axis have a $\Delta$?}\tianqing{Yeah, put a $\Delta$ in the parenthesis. } 

% %\rachel{with what source redshift distribution?}\tianqing{Combined} 

% %\rachel{paper sometimes uses `bulge-disk', sometimes `bulge-disc' -- should standardize via search/replace.  I would personally suggest `bulge+disc' (a + sign) as more standard, with the `disc' being the accepted spelling for MNRAS.}\tianqing{Fixed.} 

% %Additionally, the 11 moments for the additive bias can further separate into two group that solely contribute to the $g_1$ and $g_2$, namely, the `$g_1$ group'  and the `$g_2$ group'. We also learnt that the two groups are barely correlated, because none of the moment-pair picked from the two groups have the same parity for both $p$ and $q$. 

% %\rachel{Have you checked whether the legend would look cleaner if written instead as $10^4 m(z) = -3 z^2 + $\dots?  You are carrying around a lot of small numbers and it might look cleaner to get rid of them.}\tianqing{Fixed}  


% %\rachel{The y-axis label should be $\xi_\pm$, not just $\xi_+$.} \rachel{Is the y-axis range changing for the rows?  Can you check how it looks with the same range, which might make changes in values more clear?  Or if you really want to retain a different scale then you should flag this in the caption.}\tianqing{Fixed label, change y-scale to uniform.}

% % Note the $B[p]$ below was inconsistent with notation from section 3, so I fixed it to $B[p_i]$.

% %\rachel{This section was organizationally a bit strange, because it went over the same processes several times at different levels of detail.  Example: the ability to manipulate individual moments came up in the 1st and 2nd paragraph.  Measuring PSF moments in HSC was in the 1st paragraph and the 3rd paragraph.  I have suggested some edits to centralize the description of methods and results in a single place and reduce repetition.  As a result, it looks like I have deleted/add a lot of stuff - but mostly it is rearranging.  Please reread carefully as a sanity check.}


% % given the typical magnitude of PSF higher moment errors. %\rachel{Is this finding contingent on assumptions about the typical magnitude of PSF higher moment errors?}\tianqing{Yes, I think we should add this specification to the text.}

% %\rachel{Here would be a good place to reiterate the constructive wording re: \textsc{Piff} from the section 4.2.} 

% %\rachel{MNRAS requires a data/software availability statement, and DESC requires some documentation regarding software as per the new software policy.  For the former, please draft something (you can look at the author guide or your last paper for examples).  For the latter, please review the policy, but at minimum your code for this project should live in a DESC GitHub repo that is readable by others in the collaboration.  Perhaps you could point me to it and we can discuss other things that might be needed (documentation etc.).}\tianqing{I have scripted a data availability statement with a little tweak to the previous paper's. For the latter, I uploaded the key python code that we are using + notebooks. They are not complete and (not at all) clean, but I want to talk first about what standard they should be meeting. }

% %\rachel{For notational consistency with the paper, should the $M_{pq}$ below be $B[M_{pq}]$?  You are talking about residuals.}\tianqing{Yeah, sure. Although I want to stress that $B[M_{pq}](x,y)$ here is a functional basis of the higher moments, different from the main text.} \rachel{Then you should add a sentence that explicitly states this.}\tianqing{Done.}

% %\rachel{In some other places you've replaced the use of $^{\circ}$ notation with `deg'.  Should that be done here and elsewhere systematically?}\tianqing{Yes, they are fixed. Also fixed $\arcmin$ and $\arcsec$, should be arcmin and arcsec. }

% %\rachel{Equation is too long in compiled PDF - should break across lines (and same for the next 3 equations)}\tianqing{Fixed}

% %\rachel{I am not sure what this last sentence means.}\tianqing{Should make sense now.}

% %\rachel{Isn't the precision tunable, depending on your threshold?  Or is this an intrinsic limitation of the method?}\tianqing{Yes, it is tunable. So I change the sentence so that it means what we are doing here.} 

% %\rachel{How do we see this from the plot?  I don't see how we can know what regions have better seeing just by looking at the 4th and 6th moments.}\tianqing{It would take too much space to add the second moments plot, so I refer to \cite{2018PASJ...70S..25M} for it. } 

% %\rachel{refer explicitly to figure for this}\done. 


% %\rachel{The logic in the rearranged text was a bit unclear, so I have made some edits below.  Please check them out and confirm or suggest further edits.  Also, the rearranged text now talks about figure 10 before figure 9, so you should reorder the figures to match the order in which the text discusses them.} \tianqing{The rearrangement seems reasonable. Thanks!} 
% %\rachel{Figures 9 and 10 appear in the wrong order in the text, so should reorder the figures to fix this.}\tianqing{Fixed.}


% %\rachel{Hmm, really?  In the DESC SRD, the data vectors changed as well, because the redshift distribution changed (shallower data = shallower redshift distribution).}\tianqing{Oh my bad, the code only changed the covariance so I thought... I have change the number density to Y1 as well. } \rachel{It's the redshift distribution (not just the density) that matters for the data vectors.  Perhaps we should talk about this in our next meeting just to make sure we're on the same page?}


% %\rachel{Were you at some point going to comment on LSST Y1?}\tianqing{I have added a new paragraph for additive biases with LSST Y1 covariance + a paragraph describing LSST Y1. I also introduce a new way to compare the overall parameter biases: computing the average abs(bias/sigma) over parameters. Do you think we should switch to this expression in other occasions?} \rachel{Which parameters did you use?  I think some people would say that, for example, it's not worth including parameters like $n_s$ and $h$ since WL does not constrain them well and we rely primarily on external data (e.g., CMB) for them.  But once you exclude them, I agree it's useful to convey the information this way.}\tianqing{Yes, agreed. I switch to only calculate the parameter that WL has constraints on. }



% % \begin{tcolorbox}

% % Remaining issues

% % \begin{itemize}
% % \item Author list: who else?
% % \item Opportunities for authors to review before initiating internal review
% % \item Updating conveners about status
% % \item Contribution statements
% % \item What to do with software
% % \item SSD, following \url{https://lsstdesc.org/assets/pdf/policies/LSST_DESC_Software_Policy.pdf}
 
% % \end{itemize}
% % \end{tcolorbox}

% %There are several PSF modeling algorithm, such as \textsc{PSFEx} \citep{2011ASPC..442..435B} and \textsc{Piff} (PSF in Full FOV; \citealt{2021MNRAS.501.1282J}). 


% %\tianqing{***The next section need to be completely re-written to clearly show the layout of the paper.}

% % We introduce background material, including the PSF higher moments, shapelet decomposition, and weak lensing shear in Section~\ref{sec:background}. In Section~\ref{sec:method}, we describe our image simulations in detail, including the input galaxy catalog, the cosmoDC2 catalog \citep{Korytov:2019xus}. 
% % We also introduce how we propagate the resulting weak lensing shear biases to cosmological analysis through Fisher forecasting, and the datasets for which we measure the level of PSF higher moments error using two PSF modeling algorithms,  \textsc{PSFEx} \citep{2011ASPC..442..435B} and PSF in Full FOV \citep[\textsc{Piff};][]{2021MNRAS.501.1282J}. In Section~\ref{sec:results}, we show the impact on weak lensing shear of errors in the PSF higher moments, from the level of individual galaxy shapes to the full cosmological analysis. In Section~\ref{sec:conclusions}, we discuss the implications of our results for weak lensing with future imaging surveys. 

% %\citet{2013MNRAS.429..661M} demonstrated that controlling redshift-dependent shear biases is crucial for recovering accurate constraints on the dark energy equation of state parameters, without having to explicitly model that source of bias. 


% %\rachel{That equation does not have an index $i$.  Is there any reason not to simply state that you are going to plot the real parts only, and then show all values of $(p,q)$, rather than showing only some $(p,q)$ and introducing a new index for real/imaginary parts?  Or if you want to do it this way, could you simply refer to them as e.g. $\text{Re}[\psi_{pq}]$ and so on?}\tianqing{Change the first sentence and the label in the basis. Please check.}  

% %\rachel{I think this logical step is confusing.  You went from $(p,q)$ to now having $(p,q,m)$, whereas earlier you said you would not be using a convention that had $m=p-q$.  So you haven't said what is this $m$, leaving it by implication either undefined, or defined using $p-q$.}\tianqing{Right, I think we should just keep $N$ and $m$ and properly define them (as the order and the spin number). They've all made their appearance later.} \rachel{Can we discuss this?}

% %\rachel{not sure what `PSF several overestimated means' - should this be about some moments of the PSF?}\tianqing{Yes, thanks for pointing this out.} 



% % \section{Methods}
% % \label{sec:method}

% % In this section, we describe the methods we used for propagating the error in the PSF higher moments to cosmological parameter estimates from weak lensing shear measurements. We accomplish this by combining image simulations with measurements of PSF higher moments error in real data. The image simulation is introduced in Section~\ref{sec:im_sim_method}. The real data we use for PSF characterization is introduced in Section~\ref{sec:real_data}.
% % We describe the formalism used to quantify weak lensing 2PCF additive and multiplicative biases in Section~\ref{sec:analyses}.  


% % Therefore, Eq.~\eqref{eq:linear_eq_1} becomes
% % \begin{equation}
% % \label{eq:linear_eq_2}
% %     \sum_{j,k = (0,0)} ^{j_{\text{max}}} \frac{\partial M_i}{\partial b_j}  \Delta b_j  = \Delta M_i.
% % \end{equation}
% % To change the first $k$ moments using the first $q$ shapelet modes, we need to calculate the Jacobian $T$. 



%  %\rachel{I don't understand the value in the next sentence.  Haven't we already said that the true and model PSFs are the effective ones, in the first paragraph of this section?  And saying that we will `sometimes' do that is not useful at all, because then it's ambiguous.  We should do it always, or never (with my vote being for always).}\tianqing{Remove `sometime'.} \rachel{That means the sentence is consistent with what you said at the start of the section. But I still don't understand its purpose within the logic of this paragraph, given that you've already stated that model and true PSFs include the pixel response function, and given that it seems like a different topic from the rest of the paragraph?  What is the logical connection?} \tianqing{Okay, got it. This sentence do seems out of place. I think it is safe to remove it. }
% %Throughout the rest of this paper, we refer to the effective true/model PSF as the `true/model PSF'.


% %As we will show later, the sets of higher moments that contribute most to biases in these two quantities are distinct. 

% % As described in Section~\ref{sec:analyses:reduction}, we aim to reduce the dimensionality of the problem by identifying which PSF higher moments contribute most to additive and multiplicative shear biases, and for those contributing to additive biases, we also must understand their spatial correlation function. 


% % For the multiplicative shear bias, the task is relatively simple. We showed in Section~\ref{sec:analyses:reduction} that the multiplicative biases associated with PSF modeling errors in one single moment $B[M_{pq}]$ 
% % can be approximated by Eq.~\eqref{eq:multiplicative_approx}, which relates to the average PSF moment biases across the field. 
% % We use the COSMOS, as the second moment $\sigma$ input of our artificial Gaussian galaxies,  
% % to estimate $\langle \partial m_{pq} / \partial M_{pq} \rangle$.  
% % We use the average moment residual of \textsc{PSFEx} from Section~\ref{sec:data:psfex} as $\langle B[{M}_{pq}] \rangle$. 

 


% % The dimensionality reduction process for additive shear bias is more complex than for multiplicative bias. As described in Section~\ref{sec:analyses:reduction}, our goal is to assess the level of additive bias in the shear correlation functions $\xi_\pm$ and then identify the leading moments that contribute to them.  Therefore, our starting point is to simulate one artificial Gaussian galaxy with some average size and shape at every selected bright star position in the HSC PDR1 field, and assign a Gaussian PSF with moment residuals $B[M_{pq}](\mathbf{x})$ to these galaxies based on the moments of the true and \textsc{PSFEx} model PSFs from Section~\ref{sec:data}, modifying one higher moment bias at a time with zero second moment error.
% % We then estimate the additive shear bias for each artificial galaxy, with Eq.~\eqref{eq:additive_approx}, and use those to estimate the total additive bias on the shear 2PCF $\Delta \xi_\pm$ from all 22 higher moments estimated using Eq.~\eqref{eq:additive_deriv}. As shown in  Fig.~\ref{fig:two_groups}, the additive bias on $\xi_+$ has a magnitude $\sim 10^{-7}$ on tens of arcmin scales, 
% % which corresponds to a $\sim 1$ per cent additive systematics contribution at small scales, and a few per cent at large scales, which is significant enough to potentially affect cosmological inference. The sharp decrease at $\theta \sim 100$ arcmin suggests that physical effects associated with the HSC field of view (FOV) are the cause of structural PSF systematic biases. However, $\Delta \xi_-$ is effectively zero.  


% % In this section, we propagate the systematic residuals in the PSF higher moments to the weak lensing observable, i.e., the 2PCF $\xi_{\pm}$, with fewer simplifying assumptions than in the previous section. As described in Section~\ref{sec:analyses:mock}, we use the galaxy positions and properties from cosmoDC2 \citep{Korytov:2019xus} as the simulation inputs.  We propagate the reduced set of PSF moments obtained through the dimensionality reduction process in  Section~\ref{sec:analyses:reduction}, to the additive and multiplicative shear bias separately. To do so, we use the bulge+disc profile as the galaxy model and the Kolmogorov PSF with constant size as the PSF model. We make image simulations to calculate the shear responses $ \partial m_{pq}/ \partial M_{pq} $ and $ \partial c_{pq}/ \partial M_{pq} $ as a function of the galaxy properties on a grid. 

% % Since the PSF higher moments and residuals are measured on  the HSC fields, with smaller area than cosmoDC2, we generate synthetic PSF residual fields with similar one- and two-point statistics to the HSC data following the method described in Section~\ref{sec:analyses:moment_generation}. From the previous section, we learnt that the 22 higher-moments from $3^{\text{rd}}$ to $6^{\text{th}}$ order can be compressed to 7 (11) moments that determine the  multiplicative (additive) shear bias. 

% % We calculate the additive and multiplicative shear response $\partial c_{pq} / \partial M_{pq}$ and $\partial m_{pq} / \partial M_{pq}$ by interpolating the image simulation for the bulge+disc galaxies described in Section~\ref{sec:analyses:mock}, using the linear N-dimensional interpolation \textsc{LinearNDInterpolator}\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.interpolate.LinearNDInterpolator.html}} in \textsc{SciPy}. 
% % The moment residuals for each galaxy are the values of the GRFs in the  \textsc{HEALPix} pixel in which the galaxy is located. The details of the GRF generation process are described in Appendix~\ref{ap:grf}. Given the shear responses and the assigned PSF moment residuals, the additive and multiplicative shear biases for individual galaxies are evaluated using Eqs.~\eqref{eq:multiplicative_approx} and~\eqref{eq:additive_approx}. 

% %\tianqing{Can I ask why at some places it's `cosmoDC2', while the others are `CosmoDC2'. Is there a reason they should not be the same?} \rachel{Of course!  It should be cosmoDC2 unless it's at the start of a sentence, in which case it's capitalized because of its position -- so basically like a standard noun rather than a proper noun. You can see this convention in, for example, the abstract of \url{https://arxiv.org/abs/1907.06530}. If the text isn't already like that, perhaps some more edits are needed.  I didn't do a systematic search, just corrected a few when I saw them.}\tianqing{Okay, I did a search and replace for other places. } 

% %In this subsection, we use the Fisher forecast technique described in Section~\ref{sec:analyses:fisher}. 





% % \section{Results}
% % \label{sec:results}

% % In this Section, we present the results of propagating the systematics from PSF model higher moment errors to the cosmological parameter analysis. 
% %   We identify which higher moments have a direct and significant impact on weak lensing shear biases in Section~\ref{sec:res:prelim}, which enables us to use only the important higher moments in the remaining analysis. The results of emulating the weak lensing measurement with the cosmoDC2 galaxy catalog and generated PSF residual field are shown in Section~\ref{sec:res:dc2}. In Section~\ref{sec:res:cosmo}, we present the predicted cosmological parameter biases caused by errors in the PSF higher moments.




% % \subsection{Shear Response to PSF Higher Moment Errors}
% % \label{sec:res:image_simulation}





% % \subsection{PSF HME in Real Data}
% % \label{sec:res:real_data}

% % We measure the $2^{\text{nd}}$ to $6^{\text{th}}$ moments (25 moments) of selected bright stars in six HSC PDR1 \citep{2018PASJ...70S...8A} fields for \textsc{PSFEx} and tract 9813 in HSC Release Candidate 2 (RC2) for the \textsc{Piff} data. We use postage stamp images of the bright stars as the true PSF, and the PSF model at the stars' position as the model PSF, as described in Section~\ref{sec:data:psfex} (\textsc{PSFEx}) and Section~\ref{sec:data:piff} (\textsc{Piff}). The bias $B[M_{pq}]$, defined in Eq.~\eqref{eq:bias_define}, is measured for a given moment and position on the sky by the difference between that moment for the model and true PSF at that position. 





% % \subsection{Dimensionality Reduction}
% % \label{sec:res:prelim}


% % \subsection{Testing on Mock Galaxy Catalogs}
% % \label{sec:res:dc2}


% % \subsection{Impact on Cosmological Parameters}
% % \label{sec:res:cosmo}











% %\RequirePackage{desc-tex/styles/docswitch}
% % \flag is set by the user, through the makefile:
% %    make note
% %    make apj
% % etc.
%  %\setjournal{\flag}


% %\documentclass[]{emulateapj}
% \documentclass[fleqn,usenatbib]{mnras}

% % Custom commands from LSST DESC, see texmf/styles/lsstdesc_macros.sty
% \usepackage{desc-tex/styles/lsstdesc_macros}
% \usepackage{subfig}
% \usepackage{graphicx}
% \usepackage{threeparttable}
% \usepackage{tcolorbox}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{amsmath,amssymb}
% \usepackage{lineno}
% \linenumbers
% %\usepackage{subcaption}
% \usepackage{hyperref}
% \graphicspath{{./}{./figures/}}
% \bibliographystyle{apj}

% % Add your own macros here:
% \newcommand{\rachel}[1]{{\textcolor{magenta}{(RM: #1)}}}
% \newcommand{\tianqing}[1]{{\textcolor{cyan}{TQ: #1}}}
% \newcommand{\done}{{\textcolor{cyan}{Done.}}}
% \newcommand{\note}[1]{\textcolor{magenta}{#1}}
% \newcommand{\change}[1]{{\textcolor{green}{#1}}}


% \title[PSF Higher Moments Error and WL II]{Impact of Point Spread Function Higher Moments Error on Weak Gravitational Lensing II: A Comprehensive Study}

% \author[]{Tianqing Zhang$^1$, Husni Almoubayyed$^1$, Rachel Mandelbaum$^1$,  Joshua~E.~Meyers$^2$, \newauthor Mike Jarvis$^3$,  Arun Kannawadi$^4$, Morgan~A. Schmitz$^5$,  \newauthor The LSST Dark Energy Science Collaboration.
%  \\
% $^1$ McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, 5000 Forbes Ave, Pittsburgh, PA 15213, USA.\\
% $^2$ Lawrence Livermore National Laboratory, Livermore, CA 94551. \\
% $^3$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA.\\
% $^4$ Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08544, USA.\\
% $^5$ Universit\'e C\^{o}te d’Azur, Observatoire de la C\^{o}te d’Azur, CNRS, Laboratoire Lagrange, Bd de l’Observatoire, CS 34229, 06304 Nice \\Cedex 4, France.
% }

% \date{\today}

% \begin{document}


% \label{firstpage}
% \pagerange{\pageref{firstpage}--\pageref{LastPage}}
% \maketitle


% \begin{abstract}
% Weak gravitational lensing, or weak lensing, is one of the most powerful probes for dark matter and dark energy science, although it faces increasing challenges in controlling systematic uncertainties as measurements become more precise. The Point Spread Function (PSF) needs to be precisely modeled to avoid systematic error on the weak lensing measurements. The weak lensing biases induced by errors in the PSF model second moments, i.e., its size and shape, are well-studied. However, \citet{2021arXiv210705644Z} showed that errors in the higher moments of the PSF may also be a significant source of systematics for upcoming weak lensing surveys. Therefore, the goal of this work is to comprehensively investigate the modeling quality of PSF moments from the $3^{\text{rd}}$ to $6^{\text{th}}$ order, and estimate their impact on cosmological parameter inference. We propagate the \textsc{PSFEx} higher moments modeling error in the HSC survey dataset to the weak lensing data vector $\xi_\pm$ and its cosmological parameter inference. We find that the overall multiplicative shear bias associated with errors in PSF higher moments can cause a $\sim 0.1 \sigma$ shift on the cosmological parameters for LSST Y10. PSF higher moment errors also cause additive biases in the weak lensing shear, which, if not accounted for in the cosmological parameter analysis, can induce cosmological parameter biases comparable to their $1\sigma$ uncertainties for LSST Y10. We compare the \textsc{PSFEx} model with PSF in Full FOV (\textsc{Piff}), and find similar performance in modeling the PSF higher moments. We conclude that PSF higher moment errors of the future PSF models should be reduced from those in current methods to avoid a need to explicitly model these effects in the weak lensing analysis.
% \end{abstract}

% \begin{keywords}
%   methods: data analysis; gravitational lensing: weak 
% \end{keywords}

% % \begin{tcolorbox}

% % Remaining issues

% % \begin{itemize}
% % \item Author list: who else?
% % \item Opportunities for authors to review before initiating internal review
% % \item Updating conveners about status
% % \item Contribution statements
% % \item What to do with software
% % \item SSD, following \url{https://lsstdesc.org/assets/pdf/policies/LSST_DESC_Software_Policy.pdf}
 
% % \end{itemize}
% % \end{tcolorbox}





% \section{Introduction}
% \label{sec:introduction}

% Weak gravitational lensing, or weak lensing, is the slight deflection of the light from distant objects by the gravitational effect of nearby objects. Weak lensing leads to a mild change in the object's shape, size and flux, and it is a powerful probe of the dark matter distribution of the Universe due to its sensitivity to the gravitational potential along the line of sight \citep{Hu:2001fb, 2010GReGr..42.2177H, 2013PhR...530...87W}. To date, the most promising way of measuring  weak lensing is to measure its coherent effects on the galaxy shape, i.e., the weak lensing shear.  Weak lensing can be caused by a nearby massive galaxy or cluster, i.e.,  as measured using galaxy-galaxy lensing \citep[e.g.,][]{2014MNRAS.437.2111V, 2015MNRAS.454.1161Z, 2018PhRvD..98d2005P}; or by the large-scale  structure of the Universe, as measured using cosmic shear \citep[e.g.,][]{2020PASJ...72...16H, 2021A&A...645A.104A, 2021arXiv210513543A}. 

% The coherent galaxy shape distortions caused by weak lensing are measured using millions, even billions, of galaxies in large astronomical surveys. The ``Stage III'' cosmological surveys \citep{Albrecht:2006um} that started in the previous decade provided weak lensing observation that moved the field forward substantially; these include the Dark Energy Survey \citep[DES;][]{des_review}, the Kilo-Degree Survey \citep[KiDS;][]{deJong:2017bkf}, and the Hyper Suprime-Cam survey \citep[HSC;][]{2018PASJ...70S...4A}. In the near future, ``Stage IV'' surveys will begin to observe at greater depth and/or area than the previous generation; the Stage IV surveys include the Vera C. Rubin Observatory Legacy Survey of Space and Time \citep[LSST;][]{Ivezic:2008fe, 2009arXiv0912.0201L}, the \textit{Nancy Grace Roman} Space Telescope High Latitude Imaging Survey \citep{2015arXiv150303757S, 2019arXiv190205569A} and \textit{Euclid} \citep{Euclid_overview}. These new surveys will provide greater statistical precision in the measurements, and therefore demand greater control of systematic uncertainties in weak lensing.

% The Point Spread Function (PSF) is a function that describes the blurring of images induced by atmospheric blurring, telescope optics, and some detector effects \citep{2000PASP..112.1360A, 2013A&A...551A.119P}.  PSF modeling algorithms reconstruct the PSF as a function of position on the sky using images of stars, and interpolate that model to arbitrary positions on the image \citep{2008A&A...484...67P}.  There are several PSF modeling algorithm, such as \textsc{PSFEx} \citep{2011ASPC..442..435B} and \textsc{Piff} (PSF in Full FOV; \citealt{2021MNRAS.501.1282J}). 

% The PSF is convolved with the raw light profile of the galaxies, changing their observed shapes and sizes. Since measuring weak lensing signals relies heavily on measuring the coherent galaxy shape distortions, modeling the PSF correctly is fundamental for controlling weak lensing systematics. Failure of the PSF model to represent the true PSF causes systematic errors in the inferred galaxy shapes and weak lensing shears. Previous studies have developed a formalism that cleanly describes how the errors in modeling PSF second moments, i.e., the shape and size, affect the galaxy shape measurement and weak lensing shear inference \citep[e.g.,][]{Hirata:2003cv, PaulinHenriksson:2007mw, 2010MNRAS.404..350R,2016MNRAS.460.2245J}. There is also a formalism that describe how the PSF second moment errors further propagate to the weak lensing observables (shear-shear correlations), using the ``$\rho$-statistics'' \citep{2010MNRAS.404..350R, 2016MNRAS.460.2245J}. 

% However, the aforementioned formalism, which is commonly used for quantifying the quality of PSF modeling, does not consider the impact on weak lensing shear caused by errors in the higher moments, i.e., moments with order higher than the second, of the PSF model. In \citet{2020A&A...636A..78S}, excess multiplicative and additive shear bias is found in addition to the predictions of the second moment formalism, for \textit{Euclid}'s PSF. 
% A previous study by \citet{2021arXiv210705644Z} (ZM21) explored this topic by carrying out shape measurement experiments, with the radial kurtosis of the PSF intentionally mis-modeled, while preserving the PSF second moments. It found that errors in the PSF radial kurtosis can induce a multiplicative bias in the inferred weak lensing shear. It found that for parametric galaxy models based on the COSMOS survey, and for PSF radial kurtosis errors as in the HSC public data release 1 \citep[PDR1;][]{2018PASJ...70S...8A} PSF models from \textsc{PSFEx} \citep{2011ASPC..442..435B}, the PSF radial kurtosis error can cause a redshift-dependent multiplicative shear bias at the level of the LSST Y10 requirement \citep{2018arXiv180901669T},  
% thus motivating further research in this topic. 

% In this paper, we want to extend the understanding from ZM21 in several ways:  (a) include a wider range of PSF higher moments, which might induce both multiplicative and additive shear biases; (b) propagate the biases into the common weak lensing data vector, the two point correlation function (2PCF), and to cosmological parameter estimates; (c) include a newer PSF modeling algorithm, \textsc{Piff} \citep{2021MNRAS.501.1282J}, which might provide some estimate of how algorithm-dependent the errors in PSF higher moments are, and might serve as a better example of an algorithm that will be used for LSST.


% We introduce background material, including the PSF higher moments, shapelet decomposition, and weak lensing shear in Section~\ref{sec:background}. In Section~\ref{sec:method}, we describe our image simulations in detail, including the input galaxy catalog, the cosmoDC2 catalog \citep{Korytov:2019xus}. 
% We also introduce how we propagate the resulting weak lensing shear biases to cosmological analysis through Fisher forecasting, and the datasets for which we measure the level of PSF higher moments error using two PSF modeling algorithms,  \textsc{PSFEx} \citep{2011ASPC..442..435B} and PSF in Full FOV \citep[\textsc{Piff};][]{2021MNRAS.501.1282J}. In Section~\ref{sec:results}, we show the impact on weak lensing shear of errors in the PSF higher moments, from the level of individual galaxy shapes to the full cosmological analysis. In Section~\ref{sec:conclusions}, we discuss the implications of our results for weak lensing with future imaging surveys. 





% \section{Background}
% \label{sec:background}


% In this section, we describe the background of this paper. In Section~\ref{sec:mom_measure_mtd}, we introduce the formalism describing and method for measuring the higher moments of PSFs. We then introduce the radial shapelet decomposition, used as a basis in which we expand any given PSF light profile,  in Section~\ref{sec:shapelet_method}. In Section~\ref{sec:wl_background}, we introduce the formalism to quantify the weak lensing shear.  



% \subsection{Moment Measurement}
% \label{sec:mom_measure_mtd}


% In this subsection, we introduce the methods for measuring higher moments of the PSF. First, we define the adaptive second moment $\mathbf{M}$ for a light profile,
% \begin{equation}
% \label{eq:second_moment}
%     M_{pq} = \frac{\int \mathrm{d}x \, \mathrm{d}y \, x^p \, y^q \, \omega(x,y) \, I(x,y)}{\int \mathrm{d}x \, \mathrm{d}y \, \omega(x,y) \, I(x,y) }.
% \end{equation}
% Here $I(x,y)$ is the image intensity, where $\mathbf{x} = (x,y)$ is the image coordinate with origin at the centroid of $I(x,y)$. $\omega(x,y)$ in Eq.~\eqref{eq:second_moment} is the adaptive Gaussian weight, which has the same second moments as the light profile $I(x,y)$ \citep{Hirata:2003cv}, defined by 
% \begin{equation}
% \label{eq:def_weight_function}
% \omega(\mathbf{x}) = \text{exp}[-\mathbf{x}^T \mathbf{M}^{-1} \mathbf{x}].
% \end{equation}

% The second moment size $\sigma$ and shape $e_1$ and $e_2$ can then be calculated from the second moments $\mathbf{M}$ using
% \begin{align}
% \label{eq:def_sigma}
%     \sigma &= \left[\text{det}(\mathbf{M})\right]^{\frac{1}{4}}\\\label{eq:def_e1}
%     e_1 &= \frac{M_{20} - M_{02}}{M_{20}+ M_{02}}\\\label{eq:def_e2}
%     e_2 &= \frac{2 M_{11}}{M_{20} + M_{02}}.
% \end{align}
% Here $\text{det}(\mathbf{M}) = M_{02} M_{20} - M_{11}^2$ is the determinant of the second moment matrix. From Eqs.~\eqref{eq:def_sigma}--\eqref{eq:def_e2}, we can solve for the weighted second moments $M_{ij}$ given the weighted shape $(e_1, e_2)$ and size $\sigma$, which are measured using the  \textsc{HSM} module\footnote{\url{https://galsim-developers.github.io/GalSim/_build/html/hsm.html}} \citep{Hirata:2003cv,Mandelbaum:2005wv} in \textsc{GalSim} \citep{Rowe:2014cza}. 

% Based on the second moments, we also define a standardized coordinate system $(u,v)$ in Eq.~\eqref{eq:moment_define}; this is the coordinate system where the profile $I(u,v)$ has zero second moment shape $e_1=e_2=0$, defined in Eqs.~\eqref{eq:def_e1}--\eqref{eq:def_e2}, 
% and second moment size $\sigma = 1$, defined in Eq.~\eqref{eq:def_sigma}.
% The standardized coordinate system can be determined via a linear transformation of the image coordinate system as follows:
% \begin{equation}
% \begin{pmatrix}
% u\\
% v
% \end{pmatrix} = \mathbf{M}^{-\frac{1}{2}} \begin{pmatrix}
% x\\
% y
% \end{pmatrix}=
% \begin{pmatrix}
% M_{20} & M_{11}  \\
% M_{11} & M_{02}
% \end{pmatrix}^{-\frac{1}{2}}
% \begin{pmatrix}
% x\\
% y
% \end{pmatrix}.
% \end{equation} 


% The standardized adaptive higher moment, $M_{pq}$, is then defined by
% \begin{equation}
% \label{eq:moment_define}
%     M_{pq} = \frac{\int \mathrm{d}x \, \mathrm{d}y \, [u(x,y)]^p \, [v(x,y)]^q \, \omega(x,y) \, I(x,y)}{\int \mathrm{d}x \, \mathrm{d}y \, \omega(x,y) \, I(x,y) }.
% \end{equation}
% For the $n$\textsuperscript{th} moments, $p$ takes any value between $0$ to $n$, and $q=n-p$. 
 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\columnwidth]{plot/shapelet_basis.pdf}
%     \caption{The first 15 unique real and imaginary parts of the shapelet basis functions in Eq.~\eqref{eq:def_shapelet_basis}. %\rachel{That equation does not have an index $i$.  Is there any reason not to simply state that you are going to plot the real parts only, and then show all values of $(p,q)$, rather than showing only some $(p,q)$ and introducing a new index for real/imaginary parts?  Or if you want to do it this way, could you simply refer to them as e.g. $\text{Re}[\psi_{pq}]$ and so on?}\tianqing{Change the first sentence and the label in the basis. Please check.}  
%     We plot the first 5 orders of this basis, i.e., $p+q=0$ through $4$. The color scale for each base covers $[-A,A]$, where $A$ is the maximum of the absolute value of that basis function. }
%     \label{fig:laguerre_basis}
% \end{figure}


% Throughout this paper, we define the biases on the moment $M_{pq}$ as
% \begin{equation}
% \label{eq:bias_define}
%     B[M_{pq}] = M_{pq,\text{model}} - M_{pq,\text{true}},
% \end{equation}
% where $M_{pq,\text{model}}$ is the moment of the PSF model, and $M_{pq,\text{true}}$ is the moment of the true PSF. Note that we refer to the standardized higher moments as the ``higher moments'' throughout this paper.


% \subsection{Shapelet Decomposition}
% \label{sec:shapelet_method}



% The shapelet decomposition is an expansion of a two-dimensional image with the eigenfunctions of the 2D quantum harmonic oscillator as the basis functions. This basis function is also referred to as the Laguerre Function with Gaussian weight. This method is used to expand the galaxy and PSF profile in \citet{2005MNRAS.363..197M} and used to measure weak lensing shear in \citet{2007MNRAS.380..229M}. For detailed explanations of shapelet expansions, see also \citet{Bernstein:2001nz}. In this study, we use the shapelet decomposition implemented in \textsc{GalSim}\footnote{\url{https://github.com/GalSim-developers/GalSim}} \citep{Rowe:2014cza}.

% The shapelets basis functions are parameterized by a single parameter: the length scale $L$. After determining the value of $L$ for the image, the image can be decomposed into a series of shapelet coefficients $b_{pq}$, indexed by $p$ and $q$. We also define two more indices, i.e., the order  $N = p+q$ and the spin number $m = p-q$. The PSF image $I(r,\theta)$ can be expanded by the basis functions of the shapelet coefficients$b_{pq}$, 
% \begin{equation}
% \label{eq:shapelet_expansion}
% I(r, \theta) = \frac{1}{L ^ 2} \sum_{pq} b_{pq} \, \psi_{pq}\left(\frac{r}{L}, \theta\right),
% \end{equation}
% where $\psi_{pq}\left(\frac{r}{L}, \theta\right)$ is the Laguerre Function with Gaussian weight, i.e., the radial shapelet basis, 
% \begin{equation}
% \label{eq:def_shapelet_basis}
%     \psi_{pq}(r,\theta) = \frac{-1^q}{\sqrt{\pi}} \sqrt{\frac{q!}{p!}} \, r^m \, e^{im\theta} \, e^{-\frac{r^2}{2}} \, \mathbf{L}_q^{(m)}(r^2).
% \end{equation}
% %\rachel{I think this logical step is confusing.  You went from $(p,q)$ to now having $(p,q,m)$, whereas earlier you said you would not be using a convention that had $m=p-q$.  So you haven't said what is this $m$, leaving it by implication either undefined, or defined using $p-q$.}\tianqing{Right, I think we should just keep $N$ and $m$ and properly define them (as the order and the spin number). They've all made their appearance later.} \rachel{Can we discuss this?}
% The $\mathbf{L}_q^{(m)}(r^2)$ is the Laguerre Polynomial. Fig.~\ref{fig:laguerre_basis} shows the first 15 basis images of $\psi_{pq}$ that we use to decompose the PSF. 
% For a given order $N$, there are $2N+1$ shapelet basis functions. Due to conjugate pairings, $N$ of the shapelet coefficients $b_{pq}$ are identical to $b_{qp}$. Therefore, to expand a real image, we have $N+1$ distinct shapelet basis functions for order $N$. 


% To determine the length scale $L$, we carry out the following experiment: Decompose the PSF with different length scales $L$; only keep the 40 leading $b_{pq}$s of the shapelet series; reconstruct the image using the first forty $b_{pq}$; and measure the residual of this reconstruction. We find that to minimize the absolute value of the residual 
% of the reconstruction, the length scale $L$ should be set to the weighted second moment $\sigma$ of the PSF defined in Eq.~\eqref{eq:def_sigma}. We have therefore adopted this approach throughout this work.




% \subsection{Weak Lensing}
% \label{sec:wl_background}

% Weak gravitational lensing, or weak lensing, is the coherent gravitational distortion on background (source) galaxy flux, size, and shape by foreground (lens) objects. The lens can be any massive object, e.g., a galaxy cluster, or the cosmic large-scale structure.  
% Weak lensing is a powerful observable because of its sensitivity to the matter distribution along the line of sight \citep{Hu:2001fb,2010GReGr..42.2177H,2013PhR...530...87W}. 
% In this paper, we are interested in the cosmic shear, which is the coherent distortion of the source galaxy shapes by the large-scale structure of the Universe, resulting in a nonzero two-point correlation function of galaxy shapes. The distortion of the galaxies by the weak lensing shear is commonly parametrized  
% in its reduced form as $g  = g_1 + i g_2$. 
% $g_1$ describes the shear along the x- and y-axes, 
% while $g_2$ describes the shear at an angle $\pi/4$ with respect to the x- and y-axes. Here the x-y axes are aligned with the local (RA, Dec) axes on the sky. 

% For a cosmological weak lensing analysis, it is useful to measure the weak lensing two-point correlation function \citep{1991ApJ...380....1M}, also referred to as the 2PCF. We can calculate the shear along a chosen angular vector $\boldsymbol{\theta}$  
% connecting two galaxies, with polar angle $\phi$, by $g_t = -\mathcal{R}(g e^{-2i\phi})$, and $\pi/4$ to $\boldsymbol{\theta}$ by $g_\times = -\mathcal{I}(g e^{-2i\phi})$. The shear 2PCF is computed by
% \begin{equation}
% \label{eq:2pcf_def}
% \xi_\pm (\theta) = \langle g_t g_t \rangle (\theta) \pm \langle g_\times g_\times \rangle (\theta).
% \end{equation}
% Since the weak lensing shear is isotropic (statistically speaking), the $\xi_\pm (\theta)$ is integrated over the polar angle and presented as a function of the angular distance $\theta=|\boldsymbol{\theta}|$. 

% The weak lensing shear 2PCF as measured though $\xi_\pm$ is sensitive to the coherent change in galaxy shapes due to large-scale structure  \citep{2002A&A...396....1S}, though it is contaminated by intrinsic alignments  \citep[e.g.,][]{2000ApJ...545..561C, 2000MNRAS.319..649H}, i.e., the correlated galaxy alignments due to local effects such as tidal fields. 

% Estimating shear accurately is a key step in any cosmological analysis of weak lensing data. Shear biases are commonly  
% modeled as two terms, the multiplicative bias $m$ and the additive bias $c$ \citep{2006MNRAS.368.1323H,Massey:2006ha}, which enter the estimated shear as
% \begin{equation}
% \label{eq:shear_biases_def}
%     \hat{g} = (1+m)g + c,
% \end{equation}
% where $\hat{g}$ denotes the estimated shear. Systematic biases in the estimated shear must not exceed a certain portion of the statistical error to avoid substantial biases in the reported constraints on the cosmological parameters compared to those that would ideally be recovered. \citet{2013MNRAS.429..661M} demonstrated that controlling redshift-dependent shear biases is crucial for recovering accurate constraints on the dark energy equation of state parameters, without having to explicitly model that source of bias. As a results, error budget requirements are placed on the upper bound of the absolute value of multiplicative biases for weak lensing surveys \citep{2016MNRAS.460.2245J, 2018PASJ...70S..25M}.  
% Taking LSST Y10 as an example \citep{2018arXiv180901669T}, the requirement on the redshift-dependent multiplicative bias, which is the difference in $m$ across the full source redshift range, is 0.003. This motivates detailed studies on the connection between weak lensing shear systematics and other factors, including the PSF higher-moment modeling error (ZM21 and this work). 

% \section{Methods}
% \label{sec:method}

% In this section, we describe the methods we used for propagating the error in the PSF higher moments to cosmological parameter estimates from weak lensing shear measurements. We accomplish this by combining image simulations with measurements of PSF higher moments error in real data. The image simulation is introduced in Section~\ref{sec:im_sim_method}. The real data we use for PSF characterization is introduced in Section~\ref{sec:real_data}.
% We describe the formalism used to quantify weak lensing 2PCF additive and multiplicative biases in Section~\ref{sec:2pcf_deriv}. We introduce the mock galaxy catalog we use for estimating systematics, the cosmoDC2 catalog \citep{Korytov:2019xus}, in Section~\ref{sec:dc2_method}. We further propagate the weak lensing shear systematics to cosmological parameter analysis using Fisher forecasts as  described in Section~\ref{sec:fisher_method}. 

% \subsection{Image simulation}
% \label{sec:im_sim_method}

% In this subsection, we introduce the image simulations used in this study. We will briefly cover the parts that are similar to the image simulation process in Section~3.3 of ZM21 
% and focus on the details that are different from the previous paper. There are three main aspects to address: the general simulation workflow in Section~\ref{sec:sim_workflow}, the galaxy profiles in Section~\ref{sec:gal_profile}. In Section~\ref{sec:mom_shapelet_method}, we introduce our method of manipulating PSF higher moments by changing the coefficients of the shapelet decomposition. We introduce the PSF profiles in Section~\ref{sec:psf_profile}.

% There are some general settings in our image simulation. We use \textsc{GalSim} \citep{Rowe:2014cza} to render the simulated images, all of which are noise-free postage stamp images with a pixel scale of $0.2$ arcsec, similar to the pixel scale of the Rubin Observatory LSST Camera (LSSTCam).

% \subsubsection{Simulation Workflow}
% \label{sec:sim_workflow}


% In this section, we introduce the simulation workflow, shown in Fig.~\ref{fig:process_workflow}. In the top part of the figure, we show the steps of the image simulation process for one parametric galaxy and PSF. We start with a galaxy profile and its 90-\deg rotated pair \citep{Massey:2006ha}, an approach we use to reduce simulation volume, for which the parameters will be introduced in Section~\ref{sec:gal_profile}. The two galaxy profiles are convolved with the true effective PSF, introduced in detail in Section~\ref{sec:psf_profile}; it includes the convolution with a pixel response function ($0.2$ arcsec).  The convolved profiles are then sampled at the centers of pixels, generating the postage stamp images. 
% A similar set of images is generated using the effective model PSF.  Both sets of images are fed into the shear measurement algorithm. The shears of the galaxy pairs in this paper are estimated using re-Gaussianization \citep{Hirata:2003cv} method implemented in the HSM module \citep{Mandelbaum:2005wv} in \textsc{GalSim} \citep{Rowe:2014cza}.. We use the average of the measured shears for the galaxy and its 90-\deg rotated pair as the shear estimate for a given PSF. Finally, the difference between the two shear estimates $\Delta\hat{g}$, measured using the true PSF and the model PSF, provides an estimate of the shear bias associated with the PSF higher moment bias $B[M_{pq}]$. 

% The additive shear response to the higher moment error $M_{pq}$ is estimated at $g=0$ by
% \begin{equation}
% \label{eq:shear_response}
% \frac{\partial c_{pq}}{\partial M_{pq}} = \frac{\Delta \hat{g}}{B[M_{pq}]}.
% \end{equation}
% When we estimate the multiplicative shear bias generated by the PSF higher moment errors, we introduce another shear $g' = g + 0.01$. Its estimated value $\hat{g}'$ for the true and model PSF, and their  difference $\Delta \hat{g}'$, are used to estimate the multiplicative biases as
% \begin{equation}
% \label{eq:m_pq_estimate}
% \frac{\partial m_{pq}}{\partial M_{pq}} = \frac{\Delta \hat{g}' -\Delta \hat{g}}{0.01B[M_{pq}]}  .
% \end{equation}


% \begin{figure}
%     \includegraphics[width = 1.05\columnwidth]{plot/Workflows.pdf}
%     \caption{The workflow of the image simulation for one parametric galaxy and PSF model with one of the higher moment biased compared to the true PSF. The top part shows this workflow, while the bottom orange box shows the process that generates the true and model PSF. 
%     }
%     \label{fig:process_workflow}
% \end{figure}




% \subsubsection{Galaxy Profile}
% \label{sec:gal_profile}

% Two types of galaxy profiles are used in this study. The simpler galaxies are simulated as elliptical Gaussian light profiles. Gaussian galaxies are used in preliminary tests to develop basic intuition about the shear biases induced by errors in the PSF higher moments. The more complex galaxy model is a bulge+disc galaxy, consisting of a bulge and a disc component. The bulge+disc 
% model is used for more sophisticated tests that attempt to represent a more realistic galaxy population as in the cosmoDC2 catalog \citep{2019ApJS..245...26K}.

% The Gaussian profiles are parameterized by their size $\sigma$ and ellipticity $(e_1, e_2)$. We use them for initial tests to understand the relationship between shear bias and PSF higher moment bias (linear or non-linear?), the type of induced shear bias (multiplicative or additive?), and to determine which PSF higher moments actually contribute to weak lensing shear biases. 
% The galaxy and PSF parameters for these preliminary single galaxy simulations are shown in Table~\ref{tab:single_parameters}, with results shown in Section~\ref{sec:res:image_simulation}. All base PSFs used in these initial simulations are Gaussian profiles, except for the last row, which is a Kolmogorov PSF.

% A more sophisticated galaxy profile we use is the bulge+disc galaxy, a classic model used by many studies \citep[e.g.,][]{2006MNRAS.371....2A,2011ApJS..196...11S}. The bulges and disks in this work have common centroids. The bulge component is a de Vaucouleurs profile \citep{1948AnAp...11..247D}, a S\'ersic profile \citep{1963BAAA....6...41S} with $n = 4$, which means the surface brightness is proportional to $\exp(-R^{1/4})$, where $R$ is the distance from the centroid in units of its scale radius.  
% The disk component is a exponential profile, i.e., the surface brightness is proportional to $\exp(-R)$. Both components have independent size and shape parameters. The luminosity profile of the components of the bulge+disc galaxy is governed by two parameters: total luminosity and the bulge fraction ($B/T$). The bulge+disc simulations allow us to estimate the shear response to error in the PSF higher moments as a function of galaxy properties, which is an important input to the catalog-level simulations later in this work.





% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\columnwidth]{plot/moment_basis.pdf}
%     \caption{The moment basis for a Gaussian PSF. We only show the second to fourth moments here, with index $(p,q)$ in Eq.~\eqref{eq:moment_define} labelled in each box. We use $e_1, e_2$, and $\sigma$ to represent the second moments. The color scale for each base covers $[-A,A]$, where $A$ is the maximum of the absolute value of the basis function. 
%     }
%     \label{fig:moment_basis}
% \end{figure}




% \subsubsection{Moment-Shapelet Relation}
% \label{sec:mom_shapelet_method}

% Before introducing the PSF profile, we need a way to generate light profiles that differ in higher moments, introduced in Section~\ref{sec:mom_measure_mtd}, from the base PSF in ways that we can specify. Unfortunately, we do not know the analytical expression for a basis that has a one-to-one mapping with the higher moments. However, since the shapelet basis and the unknown ``moment basis'' can be used to describe the same linear space, we can reconstruct the unknown basis through linear combinations of the known shapelet basis, described in Section~\ref{sec:shapelet_method}. 

% To do so, we define the Jacobian matrix
% \begin{equation}
% \label{eq:jaco_def}
%     T_{ij} := \frac{\partial M_i}{\partial b_j},
% \end{equation}
% which is the generalized gradient of the moments $M_i$ with respect to the shapelet coefficients $b_j$ defined in Eq.~\eqref{eq:shapelet_expansion}.  Notice that we rank the shapelet coefficients and PSF higher moments according to the orders in Fig.~\ref{fig:laguerre_basis} and Fig.~\ref{fig:moment_basis} 
% We can then directly estimate the change in moment $\Delta M_i$ given the change in all shapelet coefficients $b_j$,
% \begin{equation}
% \label{eq:linear_eq_1}
%     \sum_{j = 0} ^{\infty} \frac{\partial M_i}{\partial b_j} \Delta b_j = \Delta M_i.
% \end{equation}
% Since $b_j$ converges to zero at large $j$ for Gaussian-like profiles including ground-based PSFs, 
% we can truncate the shapelet expansion at some finite order, making $\Delta b_j$ and $T_{ij}$ finite-sized vectors and matrices. Therefore, Eq.~\eqref{eq:linear_eq_1} becomes
% \begin{equation}
% \label{eq:linear_eq_2}
%     \sum_{j = 0} ^{j_{\text{max}}} \frac{\partial M_i}{\partial b_j}  \Delta b_j  = \Delta M_i.
% \end{equation}
% To change the first $k$ moments using the first $q$ shapelet modes, we need to calculate the Jacobian $T$. 

% To numerically measure $T_{ij}$ of the PSF with higher moment $M_{i}$, we first decompose the PSF into a set of shapelet coefficients $b_j$. 
% Then we perturb $b_j' = b_j + \Delta b_j$, and measure the higher moment $M'_i$ after the perturbation. The Jacobian element is then estimated by
% \begin{equation}
% \label{eq:jaco_cal}
%     T_{ij} = \frac{M'_i - M_{i}}{\Delta b_j}.
% \end{equation}
% In Appendix~\ref{ap:shapelet_moment}, we show a visualization of the Jacobian matrix that describes how PSF moments can be modified through changes in the shapelets coefficients. 

% In the next section, we introduce the PSF profiles in this paper, and describe how we use the Jacobian $T_{ij}$ defined in this section to change the PSF higher moments. 


% \subsubsection{PSF Profile}
% \label{sec:psf_profile}

% In the image simulation, we create the true and model PSF based on a ``base PSF''. We consider two base PSFs: Gaussian and Kolmogorov. Note that the base PSFs do not include the pixel response function, but the model and true PSFs do include it. 
% The process to create the true and model PSF is shown in the orange box in Fig.~\ref{fig:process_workflow}.

% To change the PSF moments using the technique described above, we first render an image of the base PSF including convolution with the pixel response function, and expand that image by the shapelet decomposition implemented in \textsc{GalSim} \citep{Rowe:2014cza}.  
% We carry out the shapelet decomposition up to order $10$, which corresponds to determining $66$ shapelet basis coefficients. To test that the shapelets decomposition is effectively representing the higher moments of the PSF profile, we have confirmed that the fractional kurtosis error measured using the adaptive moments of the shapelets-reconstructed PSF compared to the original image is $10^{-5}$ for Kolmogorov and $10^{-9}$ for Gaussian, which is an acceptable precision for this study. The kurtosis is a good quantity for comparing higher moments, since (a) it is a combination of three moments ($M_{04}$, $M_{22}$, and $M_{40}$); (b) many other higher moments are zeros, and are not suitable for comparing fractional differences.

% Now that we have represented the true PSF as an order $10$ shapelet series, we calculate the Jacobian $\boldsymbol{T}$ that links the $66$ shapelet coefficients with the PSF higher moments. The Jacobian is defined by Eq.~\eqref{eq:jaco_def} and estimated by Eq.~\eqref{eq:jaco_cal}. In this study, we investigate the higher moments from $3^{\text{rd}}$ to $6^{\text{th}}$ order, corresponding to $22$ moments. Together with the three second moments, the Jacobian is a $25 \times 66$ matrix. As an example, the Jacobian for the first 15 moments and first 15 shapelet modes is shown in Fig.~\ref{fig:Tij}.

% Before describing how to use $\boldsymbol{T}$ to construct images with precisely modified higher moments, we first define our notation. The true and model PSF are represented as vectors of shapelet expansion coefficients $\mathbf{b}$ and $\mathbf{b'}$. The corresponding moment vectors are $\mathbf{M}$ and $\mathbf{M'}$.  

% Ideally, we only change one higher moment of the PSF at a time, by solving for $\mathbf{\Delta b}$ in  Eq.~\eqref{eq:linear_eq_2}. 
% However, because of the non-linearity of the moment-shapelet relationship, the higher moments will not change exactly according to $B[\mathbf{M}]$ when we add $\mathbf{b}$ and $\mathbf{\Delta b}$. Therefore, we introduce multiple iterations until the target moment biases $B[\mathbf{M}]$ are achieved, specified in Algorithm~\ref{alg:change_moment}. We define $\mathbf{\Delta M}$ as the difference between our target moment vector and the current moment vector, which is the quantity we want to minimize. 
% We use the L$^2$ norm to quantify the magnitude of $\mathbf{\Delta M}$, i.e., $||\mathbf{\Delta M}||_2 = \sqrt{\mathbf{\Delta M}^T \cdot \mathbf{\Delta M}}$.
% \begin{algorithm}
% \SetAlgoLined
%  Initialize: $\mathbf{b}$, $\boldsymbol{T}$\;
%  Target moment bias: $B[\mathbf{M}]$\;
%  Target final moment vector: $\mathbf{M'} \leftarrow \mathbf{M} + B[\mathbf{M}]$\;
%  $\mathbf{\Delta M} \leftarrow B[\mathbf{M}]$\;
%  \While{$||\mathbf{\Delta M}||_2 > t_0$}{
%   Solve $\boldsymbol{T} \mathbf{\Delta b} = \mathbf{\Delta M}$ for $\mathbf{\Delta b}$ \;
%   Generate new model PSF: $\mathbf{\tilde{b}} =\mathbf{b} + \mathbf{\Delta b} $, measure its moments vector $\mathbf{\widetilde{M}}$ \;
%   Update the $\mathbf{\Delta M}$: $\mathbf{\Delta M} \leftarrow \mathbf{M'} - \mathbf{\widetilde{M}} $ \;
%   Update Jacobian: $\boldsymbol{T} \leftarrow  \frac{\partial \mathbf{\widetilde{M}}}{\partial \mathbf{\tilde{b}}}$
%  }
%  \caption{Moment Change}
% \label{alg:change_moment}
% \end{algorithm}


% We use this algorithm to ensure that the moments of the new PSF model approach the target moments $\mathbf{M} + B[\mathbf{M}]$, so the new PSF model has moment biases that differ from those of the true PSF by $B[\mathbf{M}]$. 
% We set the default threshold $t_0$ for the error in moment change to be $10^{-6}$, and the algorithm usually takes less than 5 iterations to converge for Gaussian and Kolmogorov PSFs. Note that we include the second moments in the moment bias vector $B[\mathbf{M}]$  
% and set them to zero. In this way, we ensure that the model and true effective PSF have the same second moments. %\rachel{I don't understand the value in the next sentence.  Haven't we already said that the true and model PSFs are the effective ones, in the first paragraph of this section?  And saying that we will `sometimes' do that is not useful at all, because then it's ambiguous.  We should do it always, or never (with my vote being for always).}\tianqing{Remove `sometime'.} \rachel{That means the sentence is consistent with what you said at the start of the section. But I still don't understand its purpose within the logic of this paragraph, given that you've already stated that model and true PSFs include the pixel response function, and given that it seems like a different topic from the rest of the paragraph?  What is the logical connection?} \tianqing{Okay, got it. This sentence do seems out of place. I think it is safe to remove it. }
% %Throughout the rest of this paper, we refer to the effective true/model PSF as the `true/model PSF'.

% By introducing one component of $B[\mathbf{M}]$ at a time, we can inspect the moment basis from second to sixth order by taking the difference between the images before and after one moment is slightly biased, in Fig.~\ref{fig:moment_basis}. 
% We can also quantify the impact on weak lensing shear associated with errors in the PSF model for a specific moment.

% \begin{table*}
% \begin{tabular}{ccccccc}
% \hline
% Index & Galaxy Type & Galaxy Parameters & $(g_1, g_2)$                   & PSF Parameters                      & $B[M_{pq}]$                          \\\hline
% 1     & Gaussian    & $\sigma_{\text{gal}} = 0.17$ arcsec &  $(0, 0)$  & $\sigma_{\text{PSF}} = 0.24$ arcsec & $ -0.01 \sim 0.01$   \\
% 2 & Gaussian & $\sigma_{\text{gal}} = 0.17$ arcsec & $(0 \sim 0.01, 0 \sim 0.01)$  & $\sigma_{\text{PSF}} = 0.24$ arcsec & $0.005$ \\
% 3 & Gaussian    & $\sigma_{\text{gal}} = 0.1 \sim 0.9$ arcsec & (0.0, 0.0)                                                                                                                & $\sigma_{\text{PSF}} = 0.3$ arcsec & 0.005\\
% 4 & Sérsic, n=3 & $R_{\text{gal}} = 0.1 \sim 0.9$ arcsec      & (0.0, 0.0)                                                                                                                & $\sigma_{\text{PSF}} = 0.3$ arcsec & 0.005\\
% 5 & Gaussian    & $\sigma_{\text{gal}} = 0.1 \sim 0.9$ arcsec & $(0 \sim 0.01, 0 \sim 0.01)$                                                                                                                & $\sigma_{\text{PSF}} = 0.3$ arcsec & 0.005\\
% 6 & Sérsic, n=3 & $R_{\text{gal}} = 0.1 \sim 0.9$ arcsec      & $(0 \sim 0.01, 0 \sim 0.01)$                                                                                                                & $\sigma_{\text{PSF}} = 0.3$ arcsec & 0.005\\
% 7 & Bulge+Disc & $R_{h,b}, R_{h,d}, B/T, e_b, e_d$ in Table~\ref{tab:bpd_parameter}      & $(0 \sim 0.01, 0 \sim 0.01)$  & FWHM$ = 0.6$ arcsec & 0.005\\\hline
% \end{tabular}
% \caption{The specification of galaxies, PSFs, and higher-moments error applied to the PSFs for the single galaxy image simulations in this paper. The $M_{pq}$ in the last column stands for all viable moments from $3^{\text{rd}}$ to $6^{\text{th}}$ order.  
% All base PSFs in the single galaxy simulations are Gaussian PSFs, except for the last row with Kolmogorov PSFs. Note that the PSF $\sigma$ values in the table describe the pixel-convolved true and model PSFs, not the base PSFs.
% }
% \label{tab:single_parameters}
% \end{table*}


% \subsection{HSC Data}
% \label{sec:real_data}

% In this work, we also use data from the Hyper Suprime-Cam survey \citep[HSC;][]{2018PASJ...70S...4A} to study how well current PSF models recover PSF higher moments. We inspect two datasets, one for \textsc{PSFEx} and one for \textsc{Piff}, described below. 

% For both datasets, we use the coadded images of bright stars as the true effective PSF, and compare them with the PSF model at the bright stars' positions. The \textsc{PSFEx} and \textsc{Piff} star catalogs   
% are described in Sections~\ref{sec:star_selection_psfex} and~\ref{sec:star_selection_piff}, respectively, while we describe the measurements of the PSF higher moments error in Section~\ref{sec:hsc_measure}. 

% \subsubsection{\textsc{PSFEx} Dataset}
% \label{sec:star_selection_psfex}


% The dataset for \textsc{PSFEx} is the star catalog of the first HSC public data release  \citep[PDR1;][]{2018PASJ...70S...8A}. The \textsc{PSFEx} model in this study is generated by the HSC pipeline \citep{2018PASJ...70S...5B} with a modified version of \textsc{PSFEx} \citep{2011ASPC..442..435B}; see Section~3.3 of \citet{2018PASJ...70S...5B} for more details. We use all six fields in the PDR1 survey to inspect the PSF higher moments, instead of just the \code{GAMA\_15H} field in ZM21.
% Our star selection process for the \textsc{PSFEx} is detailed in Section~3.4.1 in ZM21, so we summarize it briefly here. 

% We adopt the ``basic flag cuts'' from Table~3 of \citet{2018PASJ...70S..25M}, with \code{iclassification\_extendedness} set to 0 to identify non-extended objects. These flag cuts eliminate objects that are contaminated or affected by exposure edges, bad pixels, saturation or cosmic rays, and reduce the number of selected stars to $1.1 \times 10^7$.  
% We adopt a signal-to-noise ratio (SNR) cut $\text{SNR} > 1000$ to reduce noise in the PSF higher moments measurement, which further reduces the sample size to $3.1 \times 10^5$. In the previous work, we identified the need for a cut \code{iblendedness\_abs\_flux}$ > 0.001$ to address the fact that the moment measurements of blended objects are biased. 
% In this work, that cut reduces the sample size to $2.6 \times 10^5$. Finally, we also exclude stars with a close neighbor within $2$ arcmin of their centroids using a k-d tree. 
% At the end of the selection process, we have $2.4 \times 10^5$ stars, around four times the amount in ZM21 since we use all six HSC fields. The number density of the \textsc{PSFEx} star dataset is $0.62$ arcmin$^{-2}$. 


% \subsubsection{\textsc{Piff} Dataset}
% \label{sec:star_selection_piff}

% We measure the performance of \textsc{Piff} \citep{2021MNRAS.501.1282J} on the HSC data in order to compare with \textsc{PSFEx}. \textsc{Piff} is used as the PSF modeling algorithm for the DES Y3 dataset  
% and performed  better than previous DES PSF models, especially at modeling continuous trend across multiple detectors \citep{2021MNRAS.501.1282J}.  
% \textsc{Piff} has been run on the HSC Release Candidate 2 (RC2)\footnote{Detailed description of the RC2 dataset can be found in \url{https://dmtn-091.lsst.io/v/DM-15448/}.}, which consists of two HSC SSP-Wide tracts and one HSC SSP-UltraDeep tract. The RC2 dataset is reprocessed biweekly using the latest version of Rubin's LSST science pipelines \citep{2017ASPC..512..279J}. We inspect the PSF modeling quality on the two wide field tracts, 
% which correspond to  $\sim 6$~deg$^2$ (each tract of the HSC data is roughly $3$~\deg$^2$). 
% %\rachel{Does that mean one of the tracts corresponds to an UltraDeep field?  I'm not sure that should be compared with the Wide fields.} \tianqing{Yeah, we should only use the wide field, even though they are not performing very well. I have checked that the wide and deep fields have quite different PSFs.}

% The star selection differs from that used for the \textsc{PSFEx} dataset: we use the PIFF candidate stars with SNR$>1000$, without making the blending flux cut and close-neighbor detection. By this criterion, we have in total 11366 stars and PSF models to compare. The number density of the \textsc{Piff} dataset is $0.55$ arcmin$^{-1}$, about 13 per cent lower than that for \textsc{PSFEx}. 

% \subsubsection{Measuring PSF Higher Moment Error}
% \label{sec:hsc_measure}

% After we select stars, we use their postage stamp images as measures of the true PSF. We also obtain the PSF models evaluated at the position of the stars, as the model PSF. We use coadded star images, and the PSF models are a weighted coaddition of the PSF model in each exposure \citep{2018PASJ...70S...5B}.  
% We measure the 22 higher moments, defined in Eq.~\eqref{eq:moment_define}, from the $3^{\text{rd}}$ to the $6^{\text{th}}$ order with the method described in Section~\ref{sec:mom_measure_mtd}.  We also measure the weighted second moments with the \textsc{HSM} \citep{Mandelbaum:2005wv}  module of \textsc{GalSim}. 


% We measure the moment biases $B[M_{pq}]$ by subtracting the true PSF moments $M_{pq,\text{true}}$ 
% from the model PSF moments $M_{pq, \text{model}}$, as in Eq.~\eqref{eq:bias_define}. We calculate the ``bias fluctuation'' field $\widetilde{B}[M_{pq}](\mathbf{x})$ by
% \begin{equation}
% \label{eq:bias_fluctuation}
% \widetilde{B}[M_{pq}](\mathbf{x}) = B[M_{pq}](\mathbf{x}) - \langle B[M_{pq}](\mathbf{x}) \rangle.
% \end{equation}
% We then use the two-point correlation function (2PCF) to measure the cross-correlation of the bias fluctuations 
% $\widetilde{B}[M_{pq}](\mathbf{x})$ and $\widetilde{B}[M_{uv}](\mathbf{x})$,
% \begin{equation}
% \label{eq:moment_2pcf}
% \xi^{pq,uv}(\theta) = \langle \widetilde{B}[M_{pq}](\mathbf{x}) \widetilde{B}[M_{uv}](\mathbf{x} + \theta)  \rangle.
% \end{equation}
% When $p=u$ and $q=v$, Eq.~\eqref{eq:moment_2pcf} becomes the auto-correlation function of $\widetilde{B}[M_{pq}](\mathbf{x})$. The 2PCFs of the PSF higher moments errors are measured using \textsc{TreeCorr}\footnote{\url{https://github.com/rmjarvis/TreeCorr}} \citep{2004MNRAS.352..338J}.

% Because of the relatively small area of the \textsc{Piff} dataset, we only measure  its one-point statistics (mean, covariance matrix, etc.), not its two-point statistics. Therefore, \textsc{Piff} is only compared with \textsc{PSFEx} at the early analysis stage, rather than propagating to the weak lensing data vector contamination and biases in cosmological parameter estimates. 


% \subsection{Weak Lensing 2PCF biases}
% \label{sec:2pcf_deriv}

% In this subsection, we discuss the formalism that propagates the errors in the PSF higher moments to biases in the weak lensing 2PCF. We first provide a general derivation of our approach in Section~\ref{sec:mtd:general_deriv}, and then describe an important practical issue -- reducing the number of moments -- in Section~\ref{sec:mtd:moment_reduction}.

% \subsubsection{General Error Propagation}
% \label{sec:mtd:general_deriv}

% Our discussion of how errors in the PSF higher moments affect the weak lensing 2PCF is based on two assumptions: (a) Each PSF higher moment may produce additive shear biases $c_{pq}$  and multiplicative biases $m_{pq}$ on the observed shear, $\hat{\gamma}  = (1+m_{pq}) \gamma +c_{pq}$.  (b) The total multiplicative and additive bias $m_{\text{total}}$ and $c_{\text{total}}$ produced by simultaneous errors in multiple higher moments of the PSF can be expressed as the sum of the individual multiplicative and additive biases $m_{pq}$,
% \begin{align}
%     \label{eq:add_property_1}
%     m_{\text{total}} & \approx \sum_p \sum_q m_{pq}\\\label{eq:add_property_2}
%     c_{\text{total}} & \approx \sum_p \sum_q c_{pq},
% \end{align}
% with uncertainties that are negligible for this work.  
% The assumption (a) will be illustrated in Section~\ref{sec:res:image_simulation}, 
% and (b) is confirmed with an image simulation test, where 100 galaxies sampled from cosmoDC2 are assigned random PSF higher-moments residuals. That test shows that the absolute value of the differences between the two sides of Eqs.~\eqref{eq:add_property_1} and~\eqref{eq:add_property_2} for individual galaxies are $\le 10\%$. 
% We have explicitly confirmed that for  ensemble shear estimation, the error due to assumptions of linearity is further reduced to $\le 2$\%. 
% For the multiplicative biases, since $m_{pq} \ll 1$, we can ignore the high-order correlations, and just focus on the first order expansion of the observed 2PCF of weak lensing shear. Additive biases can be written as the sum 
% of their averages and fluctuations, $c_{pq}(\mathbf{x}) = c_{0, pq} + \tilde{c}_{pq}(\mathbf{x})$. Combining the additive and multiplicative terms, we get the full expression for the observed weak lensing 2PCF,
% \begin{align}
% \label{eq:additive_deriv}
% \langle \hat{\gamma}(\mathbf{x}) \hat{\gamma}(\mathbf{x+\theta})\rangle = & (1 + 2   m_{\text{total}}) \langle  \gamma(\mathbf{x}) \gamma(\mathbf{x+\theta})\rangle\\\nonumber 
%     & +  \sum_{pq} \sum_{uv} \langle \tilde{ c}_{pq}(\mathbf{x}) \tilde{c}_{uv}(\mathbf{x+\theta})\rangle +  c_{0,pq}  c_{0,uv}.
% \end{align}
% We are particularly interested in a redshift-dependent multiplicative bias; as suggested in \citet{2013MNRAS.429..661M}, 
% a redshift-dependent multiplicative bias can bias the inferred dark energy equation of state parameter from weak lensing. This is motivated since ZM21 found that the shear response to the PSF higher moment errors depends on the galaxy properties, which means that the galaxy ensemble in each tomographic bin will respond differently to the same PSF higher moment error.  
% In \citet{2018arXiv180901669T}, the redshift-dependent multiplicative bias is parameterized by $m_0$ in 
% \begin{equation}\label{eq:m0}
%     m(z) = m_0 \left(\frac{2z - z_\text{max}}{z_\text{max}}\right) + \bar{m}.
% \end{equation}
% The requirement for LSST Y10 is  $|m_0| \le 0.003$. 

% As shown in Eq.~\eqref{eq:additive_deriv}, the additive shear bias terms have two effects. First, the observed 2PCF is shifted by a constant $c_{0,pq}  c_{0,uv}$.  Second, it is also shifted by the scale-dependent auto-correlation function of the zero-mean additive bias field $\langle \tilde{c}(\mathbf{x}) \tilde{c}(\mathbf{x+\theta})\rangle$. We explore the impact of these changes in subsequent sections.



% \subsubsection{Dimensionality Reduction for PSF Higher Moments}
% \label{sec:mtd:moment_reduction}



% There are 22 correlated PSF moments from $3^{\text{rd}}$ to $6^{\text{th}}$ order, and the high dimensionality of this dataset can pose challenges in understanding the main issues determining the weak lensing systematic biases. Therefore, dimensionality reduction to only the PSF higher moments that induce substantial shear biases is an important first step. Since this task is based on a rough estimate of the importance of individual PSF higher moments, we use simple models for this: both the galaxy and PSF in the dimensionality reduction process are Gaussian profiles. 

 
% Eq.~\eqref{eq:additive_deriv} shows that multiplicative bias affects the weak lensing 2PCF through its total $m_{\text{total}}$, which is a summation over all $m_{pq}$.  We use the methods described in Section~\ref{sec:sim_workflow} to calculate $\partial m_{pq} / \partial M_{pq} (\sigma_\text{gal})$ as a function of the galaxy's second moment $\sigma_\text{gal}$. To roughly estimate $m_{pq}$, we use the $\sigma_\text{gal}$ of 44386 COSMOS galaxies with magnitude $< 25.2$, and galaxy resolution factor $R_2 > 0.3$ (later defined in Eq.~\eqref{eq:resolution_factor}) as the input galaxy sizes. The second moments are computed after convolving with the Hubble PSF, but before convolving with our Gaussian PSF.
% The Gaussian PSF size is fixed at a Full Width at Half Maximum (or FWHM) of $0.78~\text{arcsec}$. 
% Assuming the shear bias is proportional to the PSF moment bias, the multiplicative bias should be proportional to the moment bias as well. Therefore, we estimate the multiplicative bias $m_{pq}$ with
% \begin{equation}
% \label{eq:multiplicative_approx}
%     m_{pq}  = \left(\frac{1}{N}\sum_{i=1}^N \frac{\partial m_{pq}}{\partial M_{pq}} (\sigma_{\text{gal},i}) \right)\, \langle B[M_{pq}] \rangle,
% \end{equation}
% where the COSMOS galaxies are indexed by $i$, and $\langle B[M_{pq}] \rangle$ is the average moment bias of $M_{pq}$ in the HSC data, as described in Section~\ref{sec:real_data}. The method to estimate $\partial m_{pq}/ \partial M_{pq}$ is described in Section~\ref{sec:sim_workflow}.
% We rank the magnitude of the values of $\langle m_{pq} \rangle$ to estimate the importance of individual PSF moments. The importance is expected to be different for $g_1$ and $g_2$, given the different spatial patterns involved in different moments. 

% The additive biases are more complicated, since we must calculate the weak lensing 2PCF $\xi_{+/-}$ to understand the importance of the moments.  We design the preliminary tests for the additive biases as follows. We use the PSF higher moments and their errors as a function of position in the HSC PDR1 dataset, and for the positions of bright stars used for our HSC analysis, we put a synthetic Gaussian galaxy with the average size and shape of the population from COSMOS catalog. We then measure the shear biases of the Gaussian galaxies with the PSF higher moments biases at these positions. We obtain the biases on the shear 2PCF directly from the shear bias at position $\mathbf{x}$, estimated by 
% \begin{equation}
% \label{eq:additive_approx}
%     c_{pq} (\mathbf{x}) = \frac{\partial c_{pq}}{\partial M_{pq}} B[M_{pq}] (\mathbf{x}).
% \end{equation}


% Since each term in the additive biases on the 2PCF is associated with two different PSF moments (Eq.~\ref{eq:additive_deriv}), the ranking of importance for the PSF moments is more complex in this case. We design two different ranking system: (a) the \textbf{front-to-back} approach and (b) the \textbf{back-to-front} approach. In the \textbf{front-to-back} approach, we calculate the contribution of each $\langle c_{pq} c_{uv} \rangle$ term to the total additive bias $\Delta \langle g g \rangle$, by integrating over $\theta$ from $1$ to $200$ arcmin. 
% We rank the contribution of a given moment $M_{pq}$ by the total reduction in additive bias if we remove all terms that involve $M_{pq}$. After removing the highest-contributing PSF moment, we perform the same calculation and remove the next highest-contributing moment, until only one moment remains.

% Similarly, for the \textbf{back-to-front} approach, we remove the least-contributing PSF moment first, after performing the same contribution calculation described above. We then remove the next least-contributing moment, until we have only one moment. These two approaches provide two rankings of the PSF moments that contribute from most to least to the weak lensing additive shear bias. We expect to obtain a reasonably consistent set of PSF moments from these two approaches. 
% In the case where the two results disagree, we take the inclusive set of moments that is considered important by either method. 

% We rank the moments separately for $\langle g_1 g_1 \rangle$ and $\langle g_2 g_2 \rangle$. As we will show later, the sets of higher moments that contribute most to biases in these two quantities are distinct. 




% \subsection{Mock Catalog Simulations}
% \label{sec:dc2_method}



% To connect PSF higher moment errors with weak lensing systematics, we need a realistic galaxy catalog with galaxy properties and positional information. For this purpose, we use the cosmoDC2 catalog \citep{2019ApJS..245...26K}, as it is designed to match the galaxy population LSST is going to observe with multiple validation tests against real datasets \citep{2021arXiv211003769K}, and has sufficient area ($\sim$440 \deg$^2$) for our purposes.  
% We access the cosmoDC2 catalog using \textsc{GCRCatalogs}\footnote{\url{https://github.com/LSSTDESC/gcr-catalogs}} \citep{2018ApJS..234...36M}.

% We estimate the multiplicative and additive shear biases for each individual galaxy in cosmoDC2 using two pieces of information: shear response to PSF higher moment errors, and a synthetic catalog of PSF higher moment errors, both described below. 

% \subsubsection{Shear Response}

% The shear response to errors in PSF higher moments, $\partial \hat{g} / \partial M_{pq}$, is based on the galaxy and PSF properties. 
% We use a bulge+disc decomposition model for the galaxy, and determine the shear response as described in Section~\ref{sec:im_sim_method}. To reduce the computational expense, we carry out simulations for a grid of bulge+disc model parameters that covers the majority of the cosmoDC2 galaxies, discarding $\lesssim 1$~per cent (large galaxies that do not contribute significant shear bias) outside of the grid.   
% The free parameters in the grid are the half-light radius of the bulge $R_{h,b}$, the half-light radius of the disc $R_{h,d}$, and the bulge fraction $B/T$, and the grid is linear in all three dimensions. 
% We use the same bulge and disc shapes for all galaxies\footnote{Our tests show that using the same ellipticity for all galaxies generates $<$1 per cent error on the prediction of the ensemble shear biases, while saving tremendous computational time.}. We set the size and shape of the Kolmogorov PSF to be constant. The pixel size is $0.2$ arcsec, like that of the Rubin Observatory LSST Camera. The range of bulge+disc parameters in the image simulation is in Table~\ref{tab:bpd_parameter}.


% \begin{figure*}
%     \centering
%     \includegraphics[width=1.7\columnwidth]{plot/shear_response.pdf}
%     \caption{The additive shear bias generated by errors in the 3\textsuperscript{rd} and 4\textsuperscript{th} moments of the PSF. Both the galaxy and PSF have constant sizes. The shear biases for odd moments are well-fitted by a quadratic function, while those for even moments are linear. The quadratic fits are shown as lines,  
%     while individual simulation results are shown by dots. The quadratic terms for the 4\textsuperscript{th} moments are $\approx 0$, so the fitting functions appear to be linear. As indicated in the y-axis labels, the order-of-magnitude difference in the additive shear biases between the 3\textsuperscript{rd} and 4\textsuperscript{th} moments is $10^3$.  } 
%     \label{fig:shear_response}
% \end{figure*}


% \begin{table}
% \begin{tabular}{ccc}
% \hline
% Parameter          & Range\\\hline
% Bulge $R_{h,b}$       & $0.1 \sim 1.0~\text{arcsec}, \text{interval} = 0.1~\text{arcsec}$            \\
% Disc $R_{h,d}$       & $0.2 \sim 2.0~\text{arcsec}, \text{interval} = 0.2~\text{arcsec}$            \\
% Bulge-to-total ratio $B/T$  & $0.0 \sim 1.0, \text{interval} = 0.2$           \\
% Bulge shape & $e_1 = \pm 0.05, e_2 = \pm 0.05$\\
% Disc shape & $e_1 = \pm 0.16, e_2 = \pm 0.16$\\
% PSF FWHM & $0.6~\text{arcsec}$\\\hline
% \end{tabular}
% \caption{The parameters used in the bulge+disc image simulation. The top three rows define the parameter grid used for the simulation, while the bottom three rows are fixed parameters. We use the average absolute values of ellipticity for the bulges and disks. The $\pm$ signs indicate that the ellipticities of the galaxies in the 90-\deg rotated pairs have opposite signs.  The PSF FWHM shown is the size for the effective true and model PSFs.
% } 
% \label{tab:bpd_parameter}
% \end{table}


% After estimating a multiplicative and additive shear response to PSF higher moment errors $B[M_{pq}]$ at each grid point, we then use multi-dimensional linear interpolation from \textsc{SciPy}\footnote{\url{https://www.scipy.org/}} to estimate the multiplicative and additive shear biases for galaxies in cosmoDC2 using this grid. The \textsc{SciPy} routine performs a piece-wise interpolation in the 3-D parameter space\footnote{Our tests compare predictions for the ensemble shear bias of a sample of 100 simulated galaxies as estimated with the linear interpolation and with direct image simulations. We find no significant numerical difference between the two methods. }. 


% \subsubsection{PSF Moment Biases}
% \label{sec:mtd:moment_generation}


% Given the position for each galaxy in cosmoDC2, we need to assign PSF higher moment biases that reflect the average PSF higher moment biases and their correlation functions in the \textsc{PSFEx} dataset. Since cosmoDC2 is larger in area than any of the six HSC fields, it is impossible to directly cover the cosmoDC2 area with HSC fields. Therefore, we generate a PSF moment residual field $B[M_{pq}](x)$ with the same statistical properties as the \textsc{PSFEx} dataset, specifically the  average moment residuals and auto- and cross-correlation functions. The averages of the residuals are important for determining the multiplicative shear biases, and the correlation functions are important for the additive biases (see Section~\ref{sec:2pcf_deriv}). 

% As is described in Section~\ref{sec:hsc_measure}, the biases of PSF moments $M_{pq}$ and $M_{uv}$ are described by the average of the moment biases: $\langle B[M_{pq}] \rangle$,  $\langle B[M_{uv}] \rangle$, and the correlation function of the fluctuation $\xi^{pq,uv}(\theta)$. For the PSF moments that are of interest, we fit the correlation functions in the \textsc{PSFEx} dataset and Hankel transform them to get the angular power spectrum using \textsc{SkyLens}\footnote{\url{https://github.com/sukhdeep2/Skylens\_public/tree/imaster\_paper/}} \citep{2021MNRAS.508.1632S}, by computing
% \begin{equation}
% \label{eq:hankel_trans}
%     C_\ell^{pq, uv} = 2 \pi \int \mathrm{d} \theta \,  \theta \, \xi^{pq,uv}(\theta) \, J_0(\ell, \theta), 
% \end{equation}
% where $J_0(\ell, \theta)$ is the Bessel function of order 0. Assuming the residual field is a Gaussian field, we can generate the n-d correlated Gaussian field by these $n (n+1) /2$ angular power spectra. We use the python package \textsc{Healpy}\footnote{\url{https://github.com/healpy/healpy}} \citep{Zonca2019}, a python wrapper of the  \textsc{HEALPix}  
% software\footnote{\url{http://healpix.sourceforge.net}} \citep{2005ApJ...622..759G},  
% to generate a synthetic spherical harmonic decomposition $a_{\ell m}$ with $\ell_{\text{max}} = 3072$ and $-\ell \leq m \leq \ell$. With the $a_{\ell m}$, we generate an n-d Gaussian Random Field (GRF) evaluated at the centers of  \textsc{HEALPix} pixels with $N_{\text{side}} = 2048$, which corresponds to a pixel size of $1.7$ arcmin. The details of the GRF generation process are described in Appendix~\ref{ap:grf}. We then add the average moment biases for the \textsc{PSFEx} dataset to the GRF fluctuations to generate the total PSF higher moment bias fields. The PSF moment biases of any cosmoDC2 galaxy are the values for the \textsc{HEALPix} pixel that the galaxy sits in. The disadvantage of this method is that we cannot accurately evaluate $\langle\tilde{c}_{pq}(\mathbf{x})  \tilde{c}_{uv}(\mathbf{x+\theta})\rangle$ for angular bins below the \textsc{HEALPix} pixel size, i.e., $\theta \lesssim 1.7$ arcmin, though those scales make a negligible contribution to biases in cosmological parameters. 




% \subsubsection{Galaxy Selection and Weak Lensing Measurement}


% \begin{figure*}
%     \centering
%     \includegraphics[width=1.7\columnwidth]{plot/additive_size_ratio.pdf}
%     \includegraphics[width=1.7\columnwidth]{plot/multiplicative_size_ratio.pdf}
%     \caption{Additive (top) and multiplicative (bottom) bias responses to errors in the 3\textsuperscript{rd} and 4\textsuperscript{th}  
%     PSF moments as a function of the ratio of the galaxy and PSF half light radii $R_{h}^{\text{gal}}/R_{h}^{\text{PSF}}$. We show results for both Gaussian galaxies and S\'ersic galaxies with $n = 3.0$, both with a Gaussian PSF. The size ratio is the primary factor determining the response, and the S\'ersic index of the galaxy is an important secondary parameter. As indicated in the y-axis labels, the order-of-magnitude differences in the additive (multiplicative) shear biases between the 3\textsuperscript{rd} and 4\textsuperscript{th} moments are $10^3$ ($10^2$).  
%     }
%     \label{fig:size_ratio_bias}
% \end{figure*}

% The process outlined in the previous sections provides the galaxy responses $\partial \hat{g} / \partial M_{pq}$   
% and the correlated PSF higher moment biases  $B[M_{pq}](\mathbf{x})$ for each galaxy in the cosmoDC2 catalog. However, not all of galaxies in this catalog will be used for lensing science in LSST. Similar to the practice in the previous study, we cut on how well-resolved a galaxy is based on its resolution factor $R_2$,  
% which is calculated by
% \begin{equation}
% \label{eq:resolution_factor}
%     R_2 = 1- \frac{T_P}{T_I},
% \end{equation}
% where $T_P$ and $T_I$ are the trace of the second moment matrix for the PSF and the galaxy, respectively. The galaxy is well resolved when $R_2 \rightarrow 1$, and poorly resolved when $R_2 \rightarrow 0$. Consistent with the approach used by the HSC survey  \citep{2018PASJ...70S..25M}, we only retain galaxies with $R_2 > 0.3$, eliminating $\sim$9 per cent of the sample\footnote{Since we do not simulate each cosmoDC2 galaxy, we estimate their resolution factors by interpolation from the galaxies on the grid.}.  
% We exclude galaxies fainter than an i-band magnitude of $25.3$ for similar magnitude distribution as the LSST-`gold' samples \citep{2009arXiv0912.0201L}, and those outside the bounds of our grid of size values in Table~\ref{tab:bpd_parameter}. The lower limit of the size cut does not exclude any galaxies after the resolution factor cut, and the upper limit excludes $\sim 1 $ per cent of the galaxies.  After the cuts, the total number density of the catalog is $31.8$ arcmin$^{-1}$. 



% The bias on the 2PCF of the weak lensing shear $\Delta \xi_{+/-}$ is measured by
% \begin{equation}
% \label{eq:bias_2pcf}
% \Delta \xi_{+/-}^{ij}(\theta) = \langle \hat{g}^i(x) \hat{g}^j(x+\theta) \rangle - \langle g^i(x) g^j(x+\theta) \rangle,
% \end{equation}
% where $i$ and $j$ are the tomographic bin index. In our measurement, we split the galaxies based on their true redshifts into three tomographic bins, centred at $0.5$, $1.06$, and $1.85$. 
% The ensemble biases on the weak lensing 2PCFs $\Delta \xi_{+/-}^{ij}(\theta)$ are measured using \textsc{TreeCorr} \citep{2004MNRAS.352..338J}. 
% In the next section, we use Fisher forecasts to understand the impact of these shear biases on cosmological parameter constraints. 



% \subsection{Fisher Forecast}
% \label{sec:fisher_method}



% The ultimate goal of assessing the impact of PSF higher moment errors is to quantify their impact on a cosmological analysis using weak lensing shear, assuming that they are not explicitly accounted for in the analysis through modeling and marginalization. Since we only need an approximate estimate of the magnitude of induced cosmological parameter biases, we carry out a Fisher forecast on shear-shear data with 5 tomographic bins for the full LSST dataset (Y10). 


% In practice, we compute the Fisher information matrix $I_{ij}$ using the following equation:
% \begin{equation}
%     I_{ij} = \frac{\partial C_{\ell}}{\partial p_i}^T \text{Cov}^{-1} \frac{\partial C_{\ell}}{\partial p_j} + \delta_{ij} (\sigma_i \sigma_j)^{-1},
% \end{equation}
% where $i$ and $j$ are indices of the vector of parameters $\mathbf{p}$ (including both cosmological and nuisance parameters), $C_{\ell}$ is the angular power spectrum of the cosmic shear, and Cov$^{-1}$ is the inverse covariance matrix. The prior on each  parameter $p_i$ is added to its diagonal element in the Fisher information matrix as $1/\sigma_i^2$, where $\sigma_i$ is the standard deviation of the Gaussian prior.
% We use the DESC Science Requirements Document (SRD) covariance matrix \citep{2018arXiv180901669T}.

% The forward model in this forecast includes 7 cosmological parameters ($\Omega_m$ the matter density, $\Omega_b$ the baryonic matter density, $h$ the Hubble parameter, $n_s$ the spectral index, the power spectrum normalization parametrized as $\sigma_8$ and the dark energy equation of state parameters $w_0$ and $w_a$), 4 intrinsic alignment (IA) parameters of the non-linear alignment model \citep[NLA;][]{2017MNRAS.470.2100K}, i.e., the IA amplitude $A_0$, redshift-dependent power-law index $\eta_l$, redshift-dependent power-law index at redshift $z > 2$ $\eta_h$, and luminosity dependent parameter $\beta$.  
% The Fisher forecast code and setup is adapted from and explained more thoroughly in Almoubayyed, et al., {\em in prep}. The fiducial values and priors of all parameters are shown in Table~\ref{tab:cosmology_parameters}. 

% \begin{table}
% \centering
% \begin{tabular}{cccccc}
% \hline
% Parameter           & Value & Prior $\sigma$  & Parameter & Value & $\sigma$ \\\hline
% $\Omega_m$          & 0.3156 & 0.2 & $A_0$ & 5.0 & 2.0    \\
% $\sigma_8$       & 0.831 & 0.14  & $\eta_l$ & 0.0 & 2.0      \\
% $\Omega_b$  & 0.049 & 0.006     & $\eta_h$ & 0.0 & 2.0   \\
% $h$ & 0.6727 & 0.063  & $\beta$ & 0.0 & 2.0\\
% $n_s$ & 0.9645 & 0.9645   &  &  &   \\
% $w_a$ & 0.0 & 2.0  & & & \\
% $w_0$ & -1.0  & 0.8 & & &\\\hline
% \end{tabular}
% \caption{The fiducial values of and priors on the cosmological and intrinsic alignment parameters we use as the baseline of the Fisher forecasting. 
% }
% \label{tab:cosmology_parameters}
% \end{table}

% Derivatives of the angular power spectrum with respect to these parameters were taken using \texttt{numdifftools} \citep{numdifftools} with an absolute step-size of 0.01, which was validated to be stable through a convergence test in  Almoubayyed, et al., {\em in prep}, 
% and for the cosmological parameters, was also shown to be stable in \citet{2021arXiv210100298B}.  

% The $C_{\ell}$ values were computed in 20 $\ell$ bins, consistent with the binning used in the DESC SRD, using the Core Cosmology Library \citep{CCL}. The additive shear 2PCF biases for the tomographic weak lensing signal for redshift bins $i$ and $j$ measured in cosmoDC2 are parameterized by
% \begin{equation}
% \label{eq:fitting_function}
% \Delta \xi_+^{ij} (\theta) = a_1^{ij} e^{-s_1^{ij} \theta} + a_2^{ij} e^{-s_2^{ij} \theta},
% \end{equation}
% where the parameters $a_1^{ij}$, $a_2^{ij}$, $s_1^{ij}$, and $s_2^{ij}$ are linear functions to $z_i + z_j$, the sum of the mean redshifts of the tomographic bins being correlated. This fitting function was empirically selected based upon visual inspection, and all fractional fitting residuals are within $3\%$ of the true values. 
% The model for the additive biases associated with PSF higher moment errors has in total 8 parameters. The multiplicative biases are modeled for each tomographic bin, using a quadratic function to fit $m(z)$. Our model for the 2PCF with multiplicative biases is 
% \begin{equation}
% \label{eq:multiplicative_tomo}
% \hat{\xi}_+^{ij} = (1+m^i(z_i) + m^j(z_j))\xi_+^{ij},
% \end{equation}
% where $\hat{\xi}_+^{ij}$ and $\xi_+^{ij}$ are the observed and true cosmic shear 2PCFs. Since the multiplicative shear biases for individual bins are determined from a quadratic fitting formula,  only 3 parameters are needed to model the multiplicative biases. The 2PCF additive biases for the 15 tomographic bin-pairs are calculated using the best-fitting parameters for the linear functions of $z_i + z_j$. 
% Next, they are Hankel transformed to obtain biases in the angular power spectra, $\Delta C_\ell$. The forecasted biases on the cosmological and intrinsic alignment parameters $p_i$ are calculated using \citep{10.1111/j.1365-2966.2005.09782.x}
% \begin{equation}
% \label{eq:param_bias}
% B[p_i] = \sum_j (I^{-1})_{ij}  \frac{\partial C_{\ell}}{\partial p_j}^T  \text{Cov}^{-1}  \Delta C_{\ell}.
% \end{equation}
% We compare the bias $B[p_i]$ on each parameter with its forecasted 1$\sigma$ uncertainties from the Fisher matrix formalism in order to determine the relative importance of the systematic biases on cosmological parameter constraints due to PSF higher moment errors, if not corrected or removed. 





% \section{Results}
% \label{sec:results}

% In this Section, we present the results of propagating the systematics from PSF model higher moment errors to the cosmological parameter analysis. 
% We begin with the results of the shear response to the PSF higher moment errors with image simulations, in Section~\ref{sec:res:image_simulation}. We show the higher moments errors of the PSF model in real data from the HSC survey PDR1 in Section~\ref{sec:res:real_data}. We identify which higher moments have a direct and significant impact on weak lensing shear biases in Section~\ref{sec:res:prelim}, which enables us to use only the important higher moments in the remaining analysis. The results of emulating the weak lensing measurement with the cosmoDC2 galaxy catalog and generated PSF residual field are shown in Section~\ref{sec:res:dc2}. In Section~\ref{sec:res:cosmo}, we present the predicted cosmological parameter biases caused by errors in the PSF higher moments.




% \subsection{Shear Response to PSF Higher Moment Errors}
% \label{sec:res:image_simulation}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.8\columnwidth]{plot/mean_residual.pdf}
%     \caption{Box plot showing the PSF moment biases from the $2^{\text{nd}}$ to the $6^{\text{th}}$ moments, with the whiskers showing the $2\sigma$ range (from 3rd to 97th percentile), the boxes showing the interquartile range, and the bars showing the median. The \textsc{PSFEx} and \textsc{Piff} results are shown side-by-side. The y-axis is symmetrical log-scaled, with the linear region shown in grey. Although \textsc{PSFEx} and \textsc{Piff} were used to model two different HSC datasets, we observe a comparable order of magnitude in PSF model residuals for the two methods. However, \textsc{Piff}'s median residuals on $M_{40}$, $M_{04}$, $M_{60}$ and $M_{06}$ are a few times larger than those of \textsc{PSFEx}. These are the main contributing higher moments to the shear biases, thus motivating further development of \textsc{Piff}.  
%     }
%     \label{fig:box_plots}
% \end{figure*}

% In this subsection, we show the results of the image simulation and shear measurement experiments described in Section~\ref{sec:im_sim_method}, using Gaussian PSFs and 90-\deg rotated galaxy pairs. 
% Using these simulations, we can learn the following: (a) the form of the shear response to PSF higher moment errors -- are they linear, quadratic, or even more complicated; and (b) the pattern of shear biases associated with PSF higher moment errors, including magnitude of the biases and symmetry in the response to particular moments. Item (b) is particularly useful as it will permit dimensionality reduction to focus on only the key PSF moments in later experiments. 


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/full_correlation_psfex.pdf}
%     \includegraphics[width=1.0\columnwidth]{plot/full_correlation_piff.pdf}
%     \caption{The correlation matrix of \textsc{PSFEx} (upper) and \textsc{Piff} (lower) moments from the 2\textsuperscript{nd} to the 4\textsuperscript{th} moments, where ``t'' denotes  the true values of the moments and ``r'' denotes the moment residuals.}
%     \label{fig:correlation_matrix}
% \end{figure}
% ZM21 found only multiplicative biases associated with the radial kurtosis error of the PSF model. In this study, we cannot assume that all biases will be multiplicative, since we introduce other moment errors. In Fig.~\ref{fig:shear_response}, we show the additive shear biases due to errors in the $3^{\text{rd}}$ and $4^{\text{th}}$ moments of the PSF model, with $(p,q)$ shown on top of each sub-plot.  The galaxy and PSF parameters are given in row~1 of Table~\ref{tab:single_parameters}. 
% Fig.~\ref{fig:shear_response} shows that the $4^{\text{th}}$ moments induce shear biases that are linear in the moment residuals, while $3^{\text{rd}}$ moments induce shear biases that are non-linear in the moment residuals across the range of higher moment residuals seen in real data. We find that these curves can be fit with a quadratic form. 
% The  shear response to the even moments is 2-3 orders of magnitude higher than to the odd moments, at a fixed $B[M_{pq}]$. 
% We also note that the shear responses to conjugate higher moments, such as $M_{12}$ and $M_{21}$,  
% have opposite signs. 
% This is expected since the two moments are related through a 90-\deg rotation, causing an opposite effect on the shear. The symmetries in the shear responses to PSF higher moment errors is further discussed in Appendix~\ref{sec:app:symmetry}.  
% To reduce the size of the figure, we do not show results for the 5\textsuperscript{th} and 6\textsuperscript{th} moments, but they exhibit the same trends as the 3\textsuperscript{rd} and 4\textsuperscript{th} moments in terms of parity symmetry and different order of magnitude between shear biases for odd and even moments. 

% \begin{table}
% \begin{center}
% \begin{tabular}{ccc}
% \hline
% Moment & $\frac{ m_{pq}}{ B[M_{pq}]}$ & $\frac{c_{pq}}{  B[M_{pq}]}$ \\\hline
% (0,3)  & ($0.009, 0.001$)         & ($0.000, 0.000$)        \\
% (1,2)  & ($-0.005, 0.000$)        & ($0.000,0.000$)         \\
% (2,1)  & ($0.004,0.005$)          & ($0.000,0.000$)         \\
% (3,0)  & ($0.002,0.000$)          & ($0.000,0.000$)         \\
% (0,4)  & ($2.223,1.550$)          & ($-0.255,0.002$)        \\
% (1,3)  & ($-0.216,-0.166$)        & ($-0.005,0.376$)        \\
% (2,2)  & ($1.940,5.367$)          & ($0.000,0.000$)         \\
% (3,1)  & ($0.193,0.219$)          & ($-0.002,0.377$)        \\
% (4,0)  & ($2.248,1.543$)          & ($0.255,-0.002$)        \\
% (0,5)  & ($0.002,0.000$)          & ($0.000,0.000$)        \\
% (1,4)  & ($0.001,0.000$)          & ($0.000,0.000$)        \\
% (2,3)  & ($0.003,0.005$)          & ($0.000,0.000$)        \\
% (3,2)  & ($-0.001,0.005$)          & ($0.000,0.000$)        \\
% (4,1)  & ($0.001,0.002$)          & ($0.000,0.000$)        \\
% (5,0)  & ($0.000,0.000$)          & ($0.000,0.000$)        \\
% (6,0)  & ($-0.360,-0.078$)          & ($0.110,-0.007$)        \\
% (5,1)  & ($0.477,0.480$)          & ($-0.003,-0.206$)        \\
% (4,2)  & ($0.072,-1.266$)          & ($0.105,0.028$)        \\
% (3,3)  & ($0.029,0.012$)          & ($0.064,-0.413$)        \\
% (2,4)  & ($0.060,-1.95$)          & (-$0.105,-0.028$)        \\
% (1,5)  & ($-0.479,0.478$)          & ($-0.002,-0.206$)        \\
% (0,6)  & ($-0.358,-0.071$)          & ($-0.110,0.008$)        \\
% \hline      
% \end{tabular}
% \end{center}
% \caption{Table of multiplicative and additive shear biases per unit of PSF higher moment residuals, $m_{pq}/ B[M_{pq}]$ and $c_{pq}/B[M_{pq}]$ , for the 3\textsuperscript{rd} to 6\textsuperscript{th} moments. Since the shear biases respond nonlinearly to the odd moment errors, values in this table are computed with the average PSF higher moment error of \textsc{PSFEx}, shown in Section~\ref{sec:res:real_data}.
% }
% \label{tab:mul_add_single}
% \end{table}

% Next, to measure both additive and multiplicative shear biases,  
% we use the same galaxy and PSF sizes as in the previous plot  (specified in row~2 of Table~\ref{tab:single_parameters}), but we vary the lensing shear applied to the galaxies. In Table~\ref{tab:mul_add_single}, we show the multiplicative and additive shear biases per unit of PSF higher moments biases $m_{pq}/ B[M_{pq}]$ and $c_{pq}/ B[M_{pq}]$ for the 3\textsuperscript{rd} to 6\textsuperscript{th} moments, at the average PSF higher moment biases. Similar to Fig.~\ref{fig:shear_response}, the shear responses to the odd moments are at least two orders of magnitude smaller than the responses to the even moments. All even moments generate multiplicative shear biases, and they also strongly determine the additive biases. Notice that since the shear responds nonlinearly to the odd moments, the values for those moments in Table~\ref{tab:mul_add_single} depend on the PSF moment residuals. 


% ZM21 showed that the galaxy-to-PSF size ratio is the most important factor that determines the shear response to the errors in modeling the PSF radial kurtosis.  Here we check the sensitivity of the additive and multiplicative shear biases induced by individual PSF higher moment errors to that size ratio.  We explore this relationship by simulating Gaussian and S\'ersic galaxies with various sizes, specified in rows~3 to~6 in Table~\ref{tab:single_parameters}. In  Fig.~\ref{fig:size_ratio_bias},  we show the additive (multiplicative) shear biases  in the upper (lower) panel, as a function of the galaxy-to-PSF size ratio measured by the half light radii $R_{h}^{\text{gal}}/R_{h}^{\text{PSF}}$. 
% We can see that the size ratio plays an important role, but the S\'ersic index also affects the shear responses significantly, especially for large size ratios. This is consistent with the findings in ZM21. 





% \subsection{PSF HME in Real Data}
% \label{sec:res:real_data}

% We measure the $2^{\text{nd}}$ to $6^{\text{th}}$ moments (25 moments) of selected bright stars in six HSC PDR1 \citep{2018PASJ...70S...8A} fields for \textsc{PSFEx} and tract 9813 in HSC Release Candidate 2 (RC2) for the \textsc{Piff} data. We use postage stamp images of the bright stars as the true PSF, and the PSF model at the stars' position as the model PSF, as described in Section~\ref{sec:star_selection_psfex} (\textsc{PSFEx}) and Section~\ref{sec:star_selection_piff} (\textsc{Piff}). The bias $B[M_{pq}]$, defined in Eq.~\eqref{eq:bias_define}, is measured for a given moment and position on the sky by the difference between that moment for the model and true PSF at that position. Examples of moment residual maps for \textsc{PSFEx} and \textsc{Piff} are shown in Appendix~\ref{ap:moment_example}. 



% In Fig.~\ref{fig:box_plots}, combining the measurements of the PSF higher moments for all of the selected stars in these datasets, we show the distributions of the \textsc{PSFEx} and \textsc{Piff} moment errors $B[M_{pq}]$ with box plots side by side. 
% The whiskers of the plot show the $2\sigma$ ranges of the distributions, the boxes show the interquartile ranges, and the bars show the median. We can see from the box plots that the two PSF models have similar PSF second moment residuals, and the PSF sizes are positively biased in both models, as observed for \textsc{PSFEx} in \citet{2018PASJ...70S..25M}.  

% \textsc{Piff} produces similar order-of-magnitude PSF moment residuals as \textsc{PSFEx} from the 2\textsuperscript{nd} to the 6\textsuperscript{th} moments. However, its median residuals on $M_{40}$, $M_{04}$, $M_{60}$ and $M_{06}$ are several times larger than those for \textsc{PSFEx}, which is important because those are the primary moments contributing to the shear bias. This finding is not surprising because the implementation of \textsc{Piff} integrated with Rubin's LSST Science Pipelines has not been thoroughly tuned, and in particular, none of its testing has focused on its optimization for accurate recovery of PSF higher moments.  
% The results for \textsc{Piff} in Fig.~\ref{fig:box_plots} motivate further algorithm development and tuning, by providing additional metrics toward which to optimize in addition to the 2\textsuperscript{nd} moments. 

% In Fig.~\ref{fig:correlation_matrix}, we show the correlation matrix between the true PSF moments and their residuals for \textsc{PSFEx} (upper) and \textsc{Piff} (lower panel). We see a chequered-flag pattern in the correlation matrices. The true  moments with the same parity 
% for both $p$ and $q$ are usually positively correlated, and likewise for the residuals. 
% This results in a chequered pattern within the same order $n = p+q$ -- the ($p,q$) and the ($p\pm 2, q \mp 2$) moments are correlated -- as well as a bigger chequered pattern across the orders -- between $n$ and $n\pm 2$ orders, though the latter cannot be seen in our plots, since we are only showing $n=3$ and $n=4$ moments. There is an even larger scale pattern: the true moments and residuals for a given $(p,q)$ are typically anti-correlated with each other due to the impact of noise on the true moments. We also observe a significant anti-correlation between ``t$\sigma$'' and ``r04''/ ``r40'' for \textsc{PSFEx}. This  indicates that $M_{04}$ and $M_{40}$ are preferentially overestimated in areas of the survey with good seeing.  
% This result is consistent with the findings of ZM21, but it is not seen in the \textsc{Piff} results. However, the correlation matrix of \textsc{Piff} shows stronger anti-correlations between the true and the residual moments, which suggest that the model is relatively unresponsive to the true values. 



% \subsection{Dimensionality Reduction}
% \label{sec:res:prelim}

% As described in Section~\ref{sec:mtd:moment_reduction}, we aim to reduce the dimensionality of the problem by identifying which PSF higher moments contribute most to additive and multiplicative shear biases, and for those contributing to additive biases, we also must understand their spatial correlation function. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/multiplicative_preliminary.pdf}
%     \caption{An estimate of the weak lensing shear multiplicative biases, aimed at understanding which PSF higher moments are most important in generating multiplicative biases.  This plot is based on ensemble shear biases for a simulated COSMOS galaxy sample, given the average error on individual  higher moments of the PSF model in HSC PDR1.  
%     The orange areas are the even moments and the white areas are the odd moments. Both components of the multiplicative bias show the same set of 7 moments that contribute significantly. The y-axis is symmetrical log-scaled, with the grey area being the linear region. 
%     }
%     \label{fig:multi_prelim}
% \end{figure}

% For the multiplicative shear bias, the task is relatively simple. We showed in Section~\ref{sec:mtd:moment_reduction} that the multiplicative biases associated with PSF modeling errors in one single moment $B[M_{pq}]$ 
% can be approximated by Eq.~\eqref{eq:multiplicative_approx}, which  relates to the average PSF moment biases across the field. 
% We use the COSMOS population in ZM21, as the second moment $\sigma$ input of our artificial Gaussian galaxies,  
% to estimate $\langle \partial m_{pq} / \partial M_{pq} \rangle$.  
% We use the average moment residual of \textsc{PSFEx} from Section~\ref{sec:res:real_data} as $\langle B[{M}_{pq}] \rangle$.  
% The resulting multiplicative biases from this simplified simulation are shown in Fig.~\ref{fig:multi_prelim}. Both the $m_{\text{total},1} $ and $m_{\text{total},2} $ results indicate that PSF higher moments with both $p$ and $q$ even (seven in total) determine the  multiplicative shear bias. The total multiplicative biases are $m_{\text{total},1} = 0.0017$ and $m_{\text{total},2}  = 0.0019$, dominated by the contributions of 7 PSF higher moments.  

% %\rachel{The logic in the rearranged text was a bit unclear, so I have made some edits below.  Please check them out and confirm or suggest further edits.  Also, the rearranged text now talks about figure 10 before figure 9, so you should reorder the figures to match the order in which the text discusses them.} \tianqing{The rearrangement seems reasonable. Thanks!} 
% %\rachel{Figures 9 and 10 appear in the wrong order in the text, so should reorder the figures to fix this.}\tianqing{Fixed.}

% The dimensionality reduction process for additive shear bias is more complex than for multiplicative bias. As described in Section~\ref{sec:mtd:moment_reduction}, our goal is to assess the level of additive bias in the shear correlation functions $\xi_\pm$ and then identify the leading moments that contribute to them.  Therefore, our starting point is to simulate one artificial Gaussian galaxy with some average size and shape at every selected bright star position in the HSC PDR1 field, and assign a Gaussian PSF with moment residuals $B[M_{pq}](\mathbf{x})$ to these galaxies based on the moments of the true and \textsc{PSFEx} model PSFs from Section~\ref{sec:res:real_data}, modifying one higher moment bias at a time with zero second moment error.
% We then estimate the additive shear bias for each artificial galaxy, with Eq.~\eqref{eq:additive_approx}, and use those to estimate the total additive bias on the shear 2PCF $\Delta \xi_\pm$ from all 22 higher moments estimated using Eq.~\eqref{eq:additive_deriv}. As shown in  Fig.~\ref{fig:two_groups}, the additive bias on $\xi_+$ has a magnitude $\sim 10^{-7}$ on tens of arcmin scales, 
% which corresponds to a $\sim 1$ per cent additive systematics contribution at small scales, and a few per cent at large scales, which is significant enough to potentially affect cosmological inference. The sharp decrease at $\theta \sim 100$ arcmin suggests that physical effects associated with the HSC field of view (FOV) are the cause of structural PSF systematic biases. However, $\Delta \xi_-$ is effectively zero.  


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/total_additive.pdf}
%     \caption{ The total additive bias on the weak lensing 2PCF $\xi_\pm$ for the simulated galaxies used for dimensionality reduction. The expected shear-shear correlation functions $\xi_\pm$ for our fiducial cosmological parameters (across all redshift bins combined) are shown as dashed lines. While $\Delta \xi_+$ is positive on all scales shown, $\Delta \xi_-$ is consistent with zero. 
%     }
%     \label{fig:two_groups}
% \end{figure}

% In Fig.~\ref{fig:add_prelim}, we show the results of executing the dimensionality reduction process for additive shear bias outlined in Section~\ref{sec:mtd:moment_reduction}. In the upper and middle panel, we show the ranking of the PSF moments' contribution to $\langle g_1 g_1 \rangle$ and $\langle g_2 g_2 \rangle$. We show both the ``front-to-back method'' and ``back-to-front method'', described in Section~\ref{sec:mtd:moment_reduction}. The relative rankings given by the two methods are slightly different, 
% but the methods agree about which moments we should discard. The moments that contribute the most strongly are four of the five $4^{\text{th}}$ moments: (4,0), (3,1), (1,3), (0,4), and all seven 
% $6^{\text{th}}$ moments.  We further separate those 11 moments into two groups depending on which shear component they affect ($g_1$ or $g_2$). %\rachel{The next sentence is OK, but I wonder if it might help to replace it with one that identifies the commonalities within these groups explicitly: `The moments in the $g_1$ ($g_2$) group are those with even (odd) values for both $p$ and $q$.'  What do you think of that as a replacement?} \tianqing{This makes perfect sense. Fixed.} 
% The moments in the $g_1$ ($g_2$) group are those with even (odd) values for both $p$ and $q$. In the bottom panel, we show the additive biases on $\langle g_1 g_1 \rangle$ and $\langle g_2 g_2 \rangle$ contributed by all PSF higher moments, compared to just the contributions of the `$g_1$ group' and the `$g_2$ group'. The plot shows that the `$g_1$ group' and `$g_2$ group' moments  dominate the total additive shear biases, and therefore we can focus on just these higher moments.  

% After the dimensionality reduction of PSF higher moments, we only propagate the errors on the reduced moment set to the lensing signal in the analysis in subsequent sections.  In other words, from this point on we only consider errors in 7 (11) PSF higher moments for the multiplicative (additive) biases. 






% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/moment_ranking_c1.pdf}
%     \includegraphics[width=1.0\columnwidth]{plot/moment_ranking_c2.pdf}
%     \includegraphics[width=1.0\columnwidth]{plot/two_groups.pdf}
%     \caption{The estimate of the additive shear biases given the \textsc{PSFEx} modeling quality in the HSC PDR1.   The upper and middle panels show the rankings of the cumulative contribution to the $\Delta \langle g_1 g_1 \rangle$ and $\Delta \langle g_2 g_2 \rangle$ (respectively) from $2$ to $200$ arcmin, %\rachel{on what scale?}, respectively, 
%     from both the front-to-back and back-to-front methods described in Section~\ref{sec:mtd:moment_reduction}. The light yellow region indicates the `$g_1$ group' moments that are most relevant to the $\Delta \langle g_1 g_1 \rangle$ term, and the pink region indicates the `$g_2$ group' moments that are most relevant to the $\Delta \langle g_2 g_2 \rangle$ term. The bottom panel shows the additive biases on $\langle g_1 g_1 \rangle$ and $\langle g_2 g_2 \rangle$ from all PSF higher moments, compared to just the `$g_1$ group' and the `$g_2$ group' -- confirming that these two groups dominate the additive shear biases.   
% }
%     \label{fig:add_prelim}
% \end{figure}



% \subsection{Testing on Mock Galaxy Catalogs}
% \label{sec:res:dc2}


% In this section, we propagate the systematic residuals in the PSF higher moments to the weak lensing observable, i.e., the 2PCF $\xi_{\pm}$, with fewer simplifying assumptions than in the previous section. As described in Section~\ref{sec:dc2_method}, we use the galaxy positions and properties from cosmoDC2 \citep{Korytov:2019xus} as the simulation inputs.  We propagate the reduced set of PSF moments obtained through the dimensionality reduction process in  Section~\ref{sec:res:prelim}, to the additive and multiplicative shear bias separately. To do so, we use the bulge+disc profile as the galaxy model and the Kolmogorov PSF with constant size as the PSF model. We make image simulations to calculate the shear responses $ \partial m_{pq}/ \partial M_{pq} $ and $ \partial c_{pq}/ \partial M_{pq} $ as a function of the galaxy properties on a grid. 

% Since the PSF higher moments and residuals are measured on  the HSC fields, with smaller area than cosmoDC2, we generate synthetic PSF residual fields with similar one- and two-point statistics to the HSC data following the method described in Section~\ref{sec:mtd:moment_generation}. From the previous section, we learnt that the 22 higher-moments from $3^{\text{rd}}$ to $6^{\text{th}}$ order can be compressed to 7 (11) moments that determine the  multiplicative (additive) shear bias. 




% We calculate the additive and multiplicative shear response $\partial c_{pq} / \partial M_{pq}$ and $\partial m_{pq} / \partial M_{pq}$ by interpolating the image simulation for the bulge+disc galaxies described in Section~\ref{sec:dc2_method}, using the linear N-dimensional interpolation \textsc{LinearNDInterpolator}\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.interpolate.LinearNDInterpolator.html}} in \textsc{SciPy}. 
% The moment residuals for each galaxy are the values of the GRFs in the  \textsc{HEALPix} pixel in which the galaxy is located. The details of the GRF generation process are described in Appendix~\ref{ap:grf}. Given the shear responses and the assigned PSF moment residuals, the additive and multiplicative shear biases for individual galaxies are evaluated using Eqs.~\eqref{eq:multiplicative_approx} and~\eqref{eq:additive_approx}. 


% In Fig.~\ref{fig:redshift_mul}, we show the total multiplicative biases of the cosmoDC2 galaxies in redshift bins after including all relevant PSF higher moment errors. We use a quadratic function to fit the 10 data points, and overplot the best-fitting curve as the dashed line. As suggested by \citet{2013MNRAS.429..661M}, a linear form for the redshift dependence of the multiplicative biases affects the estimate of the dark energy equation of state using weak lensing. 
% The linear coefficient of our best-fitting $m(z)$ suggests that $m_0$ in Eq.~\eqref{eq:m0} is 0.0015, which is about half of the error budget in the LSST Y10 requirement \citep{2018arXiv180901669T}. Since the linear term of $m(z)$ can potentially cause significant cosmological parameter biases, and the impact of the quadratic term is unclear, we carry out a Fisher forecast for the impact of the redshift-dependent multiplicative biases on the inferred cosmological parameters, using the full quadratic $m(z)$. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/mz_dc2.pdf}
%     \caption{The redshift-dependent multiplicative shear biases for cosmoDC2  %\tianqing{Can I ask why at some places it's `cosmoDC2', while the others are `CosmoDC2'. Is there a reason they should not be the same?} \rachel{Of course!  It should be cosmoDC2 unless it's at the start of a sentence, in which case it's capitalized because of its position -- so basically like a standard noun rather than a proper noun. You can see this convention in, for example, the abstract of \url{https://arxiv.org/abs/1907.06530}. If the text isn't already like that, perhaps some more edits are needed.  I didn't do a systematic search, just corrected a few when I saw them.}\tianqing{Okay, I did a search and replace for other places. } 
%     galaxies, due to PSF higher moment residuals comparable to those in HSC PDR1, in 10 redshift bins. We fit the data points to a quadratic function, shown as the dashed line. 
%     }
%     \label{fig:redshift_mul}
% \end{figure}



% For the additive biases, we measure the difference in the weak lensing 2PCF, i.e., $\Delta \xi_+ = \sum_{pq} \sum_{uv} \langle \tilde{ c}_{pq}(\mathbf{x}) \tilde{c}_{uv}(\mathbf{x+\theta})\rangle +  c_{0,pq}  c_{0,uv}$, derived in Eq.~\eqref{eq:additive_deriv}.
% In  Fig.~\ref{fig:additive_tomographic}, we show the additive biases $ \Delta \xi_{\pm}$, with galaxies split into three tomographic bins. Similar to the preliminary test, the additive biases on $\xi_+$ are positive, with magnitudes increasing at higher redshifts. $\xi_-$ is consistent with zero everywhere. We parameterize  $\Delta \xi_+$ as a double-exponential function, $\Delta \xi_+ = a_1 e^{-s_1 \theta} + a_2 e^{-s_2 \theta}$, as shown in orange.

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{plot/additive_dc2.pdf}
%     \caption{The additive biases on the weak lensing 2PCF $\xi_{\pm}$ for the cosmoDC2 galaxies when subjected to PSF higher moment residuals comparable to those in HSC PDR1. The galaxies are split into three tomographic bins based on their true redshifts, centred at $z=0.5$, $1.06$, and $1.85$. The tomographic bin combination is labeled by the central redshifts of the corresponding pair of bins at the center of each panel. The y-axis uses a symmetric-log scale, with linear scale $= 3.0 \times 10^{-7}$; the linear region is shaded grey. $\Delta \xi_-$ is still consistent with zero, as for the preliminary results. We fit $\Delta \xi_+$ with a double-exponential function, shown as orange lines. 
%     }
%     \label{fig:additive_tomographic}
% \end{figure}

% In the next section, we propagate the estimated multiplicative and additive on the shear 2PCF, parameterized by the double-exponential function, to the cosmological parameter analysis using Fisher forecasts. 



% \subsection{Impact on Cosmological Parameters}
% \label{sec:res:cosmo}

% In this subsection, we use the Fisher forecast technique described in Section~\ref{sec:fisher_method}. 




% \begin{figure}
%     \includegraphics[width=1.0\columnwidth]{plot/cosmology_parameters.pdf}
%     \caption{The $1\sigma$ constraint contours from the Fisher forecast for the fiducial (black) and shifted by additive shear biases (orange) cosmological parameters for LSST Y10. The centroids of the forecasts are shown by the ``x''. If not accounted for in the analysis, the additive shear biases caused by errors in the PSF higher moments at the level produced by \textsc{PSFEx} for HSC PDR1 are predicted to shift the inferred cosmological parameters by $\sim 1\sigma$, at the LSST Y10 level.  
%     }
%     \label{fig:xi_fitting}
% \end{figure}

% In Fig.~\ref{fig:xi_fitting}, we show the cosmological parameter shifts induced by failure to account for the additive shear biases caused by PSF higher moment residuals when interpreting cosmic shear measurements at the level of LSST Y10 \citep{2018arXiv180901669T}.  In this forecast, we marginalize over the intrinsic alignment parameters $A_0$, $\beta$, $\eta_l$, and $\eta_h$. The shifts in cosmological parameters $B[p_i]$ caused by errors in the PSF higher moments correspond to $\sim 60$ to $\sim 100$ per cent of their $1\sigma$ uncertainties. 




% Next, we apply redshift-dependent multiplicative biases $m(z)$ due to errors in the PSF higher moments to the cosmic shear $\xi_\pm$ in the Fisher forecasts. For LSST Y10 \citep{2018arXiv180901669T}, we find that these multiplicative biases only shift the cosmological parameters by a few per cent of their $1\sigma$ uncertainties. 
% As discussed in Section~\ref{sec:res:dc2}, the linear coefficient of $m(z)$ suggests that we have $m_0 = 0.0015$ in Eq.~\eqref{eq:m0},  
% which corresponds to around $50$ per cent of the systematic error budget for this parameter. This prediction overestimates the impact of the redshift-dependent multiplicative biases on the cosmological parameter estimates, compared to our Fisher forecasts. The most likely reason for this finding is that our $m(z)$ is dominated by the quadratic term rather than the linear term, and therefore the redshift-dependent multiplicative shear bias is less degenerate with structure growth than the linear shear bias in Eq.~\eqref{eq:m0}.  


% We repeat the Fisher forecast analysis for LSST Y1, with the differences in its redshift distribution and covariance matrix. 
% %\rachel{Hmm, really?  In the DESC SRD, the data vectors changed as well, because the redshift distribution changed (shallower data = shallower redshift distribution).}\tianqing{Oh my bad, the code only changed the covariance so I thought... I have change the number density to Y1 as well. } \rachel{It's the redshift distribution (not just the density) that matters for the data vectors.  Perhaps we should talk about this in our next meeting just to make sure we're on the same page?}
% The LSST Y1 forecast yields a larger $\sigma$ for all of the parameters $p_i$. For the additive biases, our analysis predicts that the average $|B[p_i]|/\sigma$ for LSST Y1 is 0.21, compared to 0.73 for LSST Y10, over the parameters that the cosmic shear constrains, i.e., $\Omega_m$, $w_0$, $w_a$, and $\sigma_8$. For the multiplicative biases, our analysis predicts that this average $|B[p_i]|/\sigma$ for LSST Y1 is 0.039, compared to 0.062 for LSST Y10. In general, the PSF higher moment errors affect the results for LSST Y1 less so than LSST Y10, but is still not small enough to be negligible in the analysis, if the PSF modeling is not improved. 

% In summary, our Fisher forecast analysis shows that the PSF higher moment errors of \textsc{PSFEx} as applied to HSC PDR1 (if not reduced in magnitude or marginalized over in the analysis) can cause up to a $1\sigma$ shift in the cosmological parameter estimates in an LSST Y10 cosmic shear analysis.  This result is dominated by additive biases; the multiplicative biases only shift the estimated cosmological parameters by $\sim 0.1\sigma$ according to the Fisher forecast.

% %\rachel{Were you at some point going to comment on LSST Y1?}\tianqing{I have added a new paragraph for additive biases with LSST Y1 covariance + a paragraph describing LSST Y1. I also introduce a new way to compare the overall parameter biases: computing the average abs(bias/sigma) over parameters. Do you think we should switch to this expression in other occasions?} \rachel{Which parameters did you use?  I think some people would say that, for example, it's not worth including parameters like $n_s$ and $h$ since WL does not constrain them well and we rely primarily on external data (e.g., CMB) for them.  But once you exclude them, I agree it's useful to convey the information this way.}\tianqing{Yes, agreed. I switch to only calculate the parameter that WL has constraints on. }

% \section{Conclusions}
% \label{sec:conclusions}


% In this paper, we have presented the results of a comprehensive study of the weak lensing shear biases associated with errors in modeling the PSF higher moments (beyond second moments) for ground-based telescopes, following the previous path-finding paper that identified the potential for non-negligible weak lensing systematics due to this effect for LSST (ZM21). We have quantified the additive and multiplicative shear biases due to errors in the 3\textsuperscript{rd} to 6\textsuperscript{th} moments of the PSF, including 22 moments in total, including estimating the typical magnitude of these errors when using current PSF modeling algorithms, and propagating them to the impact on cosmological parameter estimation. 

% To carry out this study, we developed an  iterative algorithm that uses a shapelet expansion to modify individual PSF  moments in our image simulations while preserving the other moments. Using this approach, we measured the multiplicative and additive shear responses, $\partial m_{pq} / \partial M_{pq}$ and $\partial c_{pq} / \partial M_{pq}$, to the individual PSF moment errors. We identified trends in these quantities with the galaxy-to-PSF size ratio and the S\'ersic index of the galaxy. The behavior of the shear responses can be summarized as follows: 

% \begin{enumerate}
%     \item Given the typical magnitude of modeling errors in PSF higher moments, the amplitude of the shear biases due to errors in the odd moments of the PSF is 2-3  magnitude smaller than those caused by the even moments, which means that they can be ignored. 
%     \item For the even moments, the multiplicative and additive shear biases are linear functions of the moment biases $B[M_{pq}]$, and the responses primarily depend on the galaxy-to-PSF size ratio and S\'ersic index. 
%     \item Other galaxy parameters, e.g., bulge fraction $B/T$ and galaxy shapes, play a more minor role in determining the shear biases due to PSF higher moment errors. 
%     \end{enumerate}

% As an example of the current state of the art, we have measured the modeling quality of the PSF higher moments with two different PSF modeling algorithms (\textsc{PSFEx} and \textsc{Piff}) applied to the HSC survey dataset.  We used high-SNR star images as the true PSF, and the interpolated PSF model at the stars' position as the model PSF.  To focus on the impact of errors in the PSF higher moments, we measured the true and model PSF higher moments in a regularized coordinate system, where $e_1 = e_2 = 0$, and the second moment $\sigma$ values are the same for the model and true PSF. 
% Overall, the PSF modeling quality is comparable for these methods. Our findings suggest there is value in further tuning and optimizing the PSF modeling performance for the 4\textsuperscript{th} and 6\textsubscript{th} moments for future versions of \textsc{Piff}. 

% To reduce the dimensionality of the higher moment data vector and develop a basic understanding of the impact of the PSF higher moments on weak lensing, we began with  preliminary tests. 
% We put an artificial Gaussian galaxy at each HSC bright star position to determine the leading PSF higher moments that affect shear measurement. Through these tests, we put 6 (5) moments into `$g_1$ group' (`$g_2$ group'), which generate additive biases on $g_1$ ($g_2$). These 11 moments also include the 7 leading moments that generate multiplicative shear biases. 

% We then used the mock galaxy catalog cosmoDC2 to propagate PSF modeling errors to the weak lensing shear 2PCF. We used Gaussian Random Field to generate realizations of PSF higher moments error of the 11 aforementioned leading moments, based on their means and correlation functions measured in the HSC \textsc{PSFEx} dataset. We adopted the bulge+disc model that cosmoDC2 provides, and interpolated the shear bias for each galaxy based on their bulge size, disk size, and B/T ratio. We subdivided the cosmoDC2 galaxies into three tomographic bins to measure redshift-dependent shear biases, and found that PSF higher moment errors only generate non-zero biases in $\xi_+$. 

% Finally, we have propagated the PSF higher moments error to systematic biases in inferred cosmological parameters using Fisher forecasting. We find that additive shear biases due to PSF higher moment errors can cause a $1\sigma$ systematic shift on key cosmological parameters, such as $\Omega_m$, $\sigma_8$ and $w_0$, at the LSST Y10 level -- implying that either PSF higher moment errors must be reduced from current levels for LSST Y10, or this effect must be explicitly modeled in the cosmological parameter analysis.  
% In contrast, the multiplicative shear biases only cause cosmological parameter shifts of at most $0.1\sigma$. The forecast shows that the impact of the PSF higher moment errors on LSST Y1 is smaller than that on LSST Y10, but the effect is still not negligible even for Y1.


% This results of this paper imply that future surveys, including LSST and the High Latitude Survey of the Roman Space Telescope, need to design null tests to ensure that the additive shear biases due to PSF higher moment errors do not cause an unacceptable level of contamination of the weak lensing shear data vectors. It also motivates the inspection of PSF higher moment modeling quality to drive the further development of  new PSF modeling algorithms. Finally, it suggests that requirements on PSF higher moment modeling quality, and/or mitigation methods, are needed for these surveys to recover unbiased cosmological constraints from the weak lensing shear data. 




% % ----------------------------------------------------------------------
% \section*{Contributors}

% TZ developed the simulation and measurement software, carried out analysis on the results, and led the writing of the manuscript. HA developed the code for the Fisher Information matrix and relevant parameter inference, and contributed writing for Section 3.5.  RM proposed the project, advised on the motivation, experimental design and analysis, and edited the manuscript. JEM advised and provided early access to HSC data processed using \textsc{Piff}.  MJ, AK and MAS provided feedback throughout the project and edited the manuscript. %\tianqing{(Other contributors needed!)}

% \subsection*{Acknowledgments}


% TZ and RM are supported in part by the Department of Energy grant DE-SC0010118 and in part by a grant from the Simons Foundation (Simons Investigator in Astrophysics, Award ID 620789). 

% The DESC acknowledges ongoing support from the Institut National de Physique Nucl\'eaire et de Physique des Particules in France; the Science \& Technology Facilities Council in the United Kingdom; and the Department of Energy, the National Science Foundation, and the LSST Corporation in the United States.  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S.\ Department of Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.

% Based in part on data collected at the Subaru Telescope and retrieved from the HSC data archive system, which is operated by Subaru Telescope and Astronomy Data Center at National Astronomical Observatory of Japan.

% The Hyper Suprime-Cam Subaru Strategic Program (HSC-SSP) is led by the astronomical communities of Japan and Taiwan, and Princeton University.  The instrumentation and software were developed by the National Astronomical Observatory of Japan (NAOJ), the Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU), the University of Tokyo, the High Energy Accelerator Research Organization (KEK), the Academia Sinica Institute for Astronomy and Astrophysics in Taiwan (ASIAA), and Princeton University.  The survey was made possible by funding contributed by the Ministry of Education, Culture, Sports, Science and Technology (MEXT), the Japan Society for the Promotion of Science (JSPS),  (Japan Science and Technology Agency (JST),  the Toray Science Foundation, NAOJ, Kavli IPMU, KEK, ASIAA, and Princeton University.

% This paper makes use of software developed for the Large Synoptic Survey Telescope. We thank the LSST Project for making their code available as free software at http://dm.lsst.org. 

% The Pan-STARRS1 Surveys (PS1) have been made possible through contributions of the Institute for Astronomy, the University of Hawaii, the Pan-STARRS Project Office, the Max-Planck Society and its participating institutes, the Max Planck Institute for Astronomy, Heidelberg and the Max Planck Institute for Extraterrestrial Physics, Garching, The Johns Hopkins University, Durham University, the University of Edinburgh, Queen’s University Belfast, the Harvard-Smithsonian Center for Astrophysics, the Las Cumbres Observatory Global Telescope Network Incorporated, the National Central University of Taiwan, the Space Telescope Science Institute, the National Aeronautics and Space Administration under Grant No. NNX08AR22G issued through the Planetary Science Division of the NASA Science Mission Directorate, the National Science Foundation under Grant No. AST-1238877, the University of Maryland, and Eotvos Lorand University (ELTE) and the Los Alamos National Laboratory.



% We thank the developers of \textsc{GalSim}, \textsc{ngmix}, and \textsc{TreeCorr} for making their software openly accessible. Some of the results in this paper have been derived using the \textsc{Healpy} and \textsc{HEALPix} package.


% \section*{Data Availability}

% The HSC-SSP data in this paper is publicly available at \url{https://hsc-release.mtk.nao.ac.jp/doc/index.php/tools-2/}. 
% The COSMOS catalog is available at \url{https://zenodo.org/record/3242143#.YF2bHK9KiUk}.
% The cosmoDC2 catalog is available at the LSST DESC Data Portal
% \url{https://data.lsstdesc.org/}.
% Simulation and analysis code will be shared on reasonable request to the authors.



% \bibliography{main}


% \appendix


% \section{Shapelet-Moment Relation}
% \label{ap:shapelet_moment}


% In Section~\ref{sec:mom_shapelet_method}, we explained that the key to changing the PSF moments through a shapelet decomposition is to compute the Jacobian matrix using Eq.~\eqref{eq:jaco_cal}.
% In Fig.~\ref{fig:Tij}, we show an example of the Jacobian matrix $T$ for PSF higher moment errors $B[M_{pq}]$ with respect to the shapelet modes $b_j$  
% for a Kolmogorov PSF. There is a block diagonal structure that shows the PSF second moments depend on the $\text{4}^{\text{th}}$ to $\text{5}^{\text{th}}$ shapelet modes. The PSF third moments 
% depend on the $\text{6}^{\text{th}}$ to $\text{9}^{\text{th}}$ shapelet modes. The PSF fourth moments
% depend not only on the $\text{10}^{\text{th}}$ to $\text{14}^{\text{th}}$ shapelet modes, but also on the shapelet modes that determine the second moments. This means that the n\textsuperscript{th} PSF higher moments basis can be approximately decomposed into shapelets components with the same order $n$. 

% With the Jacobian matrix shown in Fig.~\ref{fig:Tij} and the Algorithm~\ref{alg:change_moment}, we modify the individual PSF higher moments with moment error threshold $||\mathbf{\Delta M}||_2 = 10^{-6}$. 
% This precision is sufficient for exploring systematic shear biases associated with errors in the PSF higher moments. 

% \begin{figure*}
%     \centering
%     \includegraphics[width=2.0\columnwidth]{plot/Tij.pdf}
%     \caption{The Jacobian of PSF moments with respect to the shapelet coefficients, 
%     $T_{ij} = \frac{\partial M_i}{\partial b_j}$ for a Kolmogorov PSF. We show the first 12 PSF moments starting from the second moments (i.e., 3 second moments, 4 third moments, and 5 fourth moments) 
%     and the first 25 shapelet components starting from $n = 2$ for the shapelets decomposition.  The numbers that overlap the circle are the values of $T_{ij}$, with each row normalized by the $L^2$-norm $\sqrt{\sum_j T_{ij}^2}=1$. The sizes of the circles reflect the magnitude of the entry, and colors reflect the sign (blue for positive and yellow for negative).   The column on the left shows the postage stamp images of the difference in PSF with only one moment being changed. The bottom row shows the first 25 shapelet basis from the 2\textsuperscript{nd} order to 6\textsuperscript{th} order, as the basis for the moment modification. We rank the shapelet coefficients by increasing the order $n$. For each $n$, we start with the real part of $p = n$, then its imaginary part, and decrease $p$ until $p=q$ or $p=q+1$. The labels on the shapelet basis functions should be interpreted as follows: $pq$ is equivalent to Re$[\psi_{pq}]$, $pq^*$ is equivalent to Im$[\psi_{pq}]$.  We can see that the Jacobian matrix is very close to being a  block-diagonal matrix, which means that the PSF higher moments are linear combinations of the shapelet components with the same order $n$.
%     \label{fig:Tij}
%     }
% \end{figure*}



% \section{Symmetry in the response to PSF higher moments}
% \label{sec:app:symmetry}



% In Fig.~\ref{fig:shear_response}, it is clear that the shear response to the PSF higher moments exhibits symmetries among the different higher moments. In this section, we explore and explain this symmetry. We start by proposing four lemmas, and derive the symmetry of the shear response based on these four lemmas. 



% Lemma 1: For any two PSF modeling residual basis functions $B[M_{pq}](x,y)$ and $B[M_{uv}](x,y)$ such that $B[M_{pq}](x,y)$ can be obtained by rotating $B[M_{uv}](x,y)$ by $\pm90$~\deg, the corresponding shear biases $\Delta \hat{g}(B[M_{pq}])$ and $\Delta \hat{g}(B[M_{uv}])$ satisfy the following constraint:
% \begin{equation}
%     \Delta \hat{g}(B[M_{pq}]) = - \Delta \hat{g}(B[M_{uv}])
% \end{equation}
% Note that this Lemma is also the basis for the fact that a 90~\deg rotated galaxy pair has an average shape of $0$, a fact that we use in the single galaxy simulations. We also stress that the $B[M_{pq}](x,y)$ in this section is a functional basis of the higher moments error (see Fig.~\ref{fig:moment_basis} for examples), different from the moment biases $B[M_{pq}]$ elsewhere.

% Lemma 2: The PSF modeling residual function $B[M_{pq}](x,y)$ has the form
% \begin{align}
%     B[M_{pq}](x,y) &= B[M_{pq}](-x,y) \; \; \; \;& \text{if p is even}\\
%     B[M_{pq}](x,y) &= -B[M_{pq}](-x,y) \; \; \; & \text{if p is odd.}
% \end{align}
% This is due to the symmetry (asymmetry) in the even (odd) functions used in the moment measurement. 

% Lemma 3: Similar to Lemma 2, the PSF modeling residual function $B[M_{pq}](x,y)$ 
% has the form:
% \begin{align}
%     M_{pq}(x,y) &= M_{pq}(x,-y) \; \; \; \;& \text{if q is even}\\
%     M_{pq}(x,y) &= -M_{pq}(x,-y) \; \; \; & \text{if q is odd.}
% \end{align}

% Lemma 4: For any $p$ and $q$, the PSF modeling residual function satisfies the relationship 
% \begin{equation}
%     B[M_{qp}](x,y) = B[M_{pq}](y,x). 
% \end{equation}
% This is easily proved by substituting $y$ for $x$ and vice versa. 


% With these lemmas, we can identify  symmetry relationships between different moments, as long as the moment bases are rotations of each other. But first, we must define the rotation operators $\mathcal{R}$ and $\mathcal{R}'$,
% \begin{itemize}
%     \item $\mathcal{R}(B[M_{pq}](x,y)) = B[M_{pq}](y,-x)$ -- a function that rotates the moment basis by $90$~deg clockwise.  
%     \item $\mathcal{R}'(B[M_{pq}](x,y)) = B[M_{pq}](-y,x)$ -- a function that rotates the moment basis by $90$~\deg counter-clockwise.
% \end{itemize}


%  Fig.~\ref{fig:shear_response} shows that the symmetry between results for different moments depends on the parity of the moment index $p$ and $q$. Therefore, we consider four scenarios with different parities.

% Case 1: If both $p$ and $q$ are even:
% \begin{align}
%     B[M_{qp}](x,y) &= B[M_{pq}](y,x) \\\nonumber &= B[M_{pq}](y,-x) = \mathcal{R}(B[M_{pq}](x,y))
% \end{align}
% The first two steps use Lemma 4 and Lemma 3, respectively. The last step relies on the definition of  $\mathcal{R}$. Using Lemma 1 on the very left-hand-side (LHS) and very right-hand-size (RHS) of this equation, we infer that $\Delta\hat{g}(B[M_{pq}]) = -\Delta\hat{g}(B[M_{qp}])$, which is consistent with the results for $(p,q)=(0,4)$ in Fig.~\ref{fig:shear_response}. This case also implies that for even values of $p=q$, $\Delta\hat{g}$ must be 0, as is seen for the $(p,q)=(2,2)$ case in Fig.~\ref{fig:shear_response}. 


% Case 2: If $p$ is even and $q$ is odd:
% \begin{align}
%     B[M_{qp}](x,y) &= B[M_{pq}](y,x)\\\nonumber &= B[M_{pq}](-y,x) = \mathcal{R}'(B[M_{pq}](x,y)).
% \end{align}
% The first two steps utilize Lemma 4 and Lemma 2, respectively. The last step relies on the definition of $\mathcal{R}'$. With Lemma 1 applied to the very LHS and RHS, we infer that $\Delta\hat{g}B[(M_{pq}]) = -\Delta\hat{g}(B[M_{qp}])$ for this case. This finding is consistent with the results for $(p,q)=(0,3)$ and $(2,1)$ in Fig.~\ref{fig:shear_response}.


% Case 3: If $p$ is odd and $q$ is even, the only difference from Case 2 is to flip $x$ instead of $y$ in the second step:
% \begin{align}
%     B[M_{qp}](x,y) &= B[M_{pq}](y,x)\\\nonumber &= B[M_{pq}](y,-x) = \mathcal{R}(B[M_{pq}](x,y)).
% \end{align}
% The first two steps utilize Lemma 4 and Lemma 3. The last step relies on the definition of $\mathcal{R}$. With Lemma 1 applied to the very LHS and RHS, we infer that $\Delta\hat{g}(B[M_{pq}]) = -\Delta\hat{g}(B[M_{qp}])$. 

% Case 4: If both $p$ and $q$ are odd:
% \begin{align}
%   B[M_{qp}](x,y) &= B[M_{pq}](y,x)\\\nonumber &= -B[M_{pq}](y,-x) = - \mathcal{R}(B[M_{pq}](x,y)).
% \end{align}
% The first two steps use Lemma 4 and Lemma 3. The last step relies on the definition of $\mathcal{R}$. Applying Lemma 1 to the very LHS and RHS, we infer that $\Delta\hat{g}(B[M_{pq}]) = \Delta\hat{g}(B[M_{qp}])$. This finding is consistent with the results for $(p,q)=(1,3)$ in Fig.~\ref{fig:shear_response}. 

% In conclusion, only when both $p$ and $q$ are odd will we get $\Delta\hat{g}(B[M_{pq}]) = \Delta\hat{g}(B[M_{qp}])$. Otherwise, $\Delta\hat{g}(B[M_{pq}]) = -\Delta\hat{g}(B[M_{qp}])$, implying that pairings with even values of $p=q$ produce zero shear bias.  As described above, these symmetry patterns are displayed in Fig.~\ref{fig:shear_response}. While not shown in the plot, we have explicitly confirmed that the above conclusions apply to the 5\textsuperscript{th} and 6\textsuperscript{th} moments as well, and they should hold beyond that as well.   



% \section{Examples of Moment Residual Maps in HSC}
% \label{ap:moment_example}

% In Fig.~\ref{fig:moment_example}, 
% we show two example of the PSF moment maps that we measure in the 6 HSC fields. We show maps for the true moments and the residual $B[M_{pq}]$. We can see that the true PSF higher moments and their residuals clearly have real spatial structure, as is found in ZM21 for the radial kurtosis. The residuals are both correlated with the true moments, showing that \textsc{PSFEx} performs differently depending on the true underlying PSF, which suggests that one opportunity for improvement in future algorithms is greater performance stability.  
% Comparing to figure 1 in \cite{2018PASJ...70S..25M}, we observe that the better seeing parts of the area have PSF higher moment biases that are higher than other areas, especially for the 4\textsuperscript{th} and 6\textsuperscript{th} moments. Many of these good-seeing areas are eliminated from the HSC first-year shear catalog, described in section 4 of \cite{2018PASJ...70S..25M}, due to them failing various PSF modeling tests. 
% This is confirmed both visually and by the correlation matrix in Fig.~\ref{fig:correlation_matrix} for \textsc{PSFEx}. 

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.75\columnwidth]{plot/hsc_example1.png}
%     \includegraphics[width=2.0\columnwidth]{plot/hsc_example2.png}
%     \caption{Two examples of the maps of PSF higher moments for the HSC PDR1 data, as modeled by \textsc{PSFEx}. For both examples, we show the true value and the moment residual $B[M_{pq}]$. The top panel shows a map of the (0,4) moment measured in the GAMA09H field, and the bottom panel shows the (4,2) moment measured in the GAMA15H field. There is coherent structure in both the true moments and their residuals, suggesting that the measurement is not noise dominated.
%     \label{fig:moment_example}}
% \end{figure*}




% \section{Generating the Gaussian Random Fields}
% \label{ap:grf}


% \begin{figure*}
%     \centering
%     \includegraphics[width=1.3\columnwidth]{plot/group1_map.pdf}
%     \includegraphics[width=1.3\columnwidth]{plot/group2_map.pdf}
%     \caption{The original correlation function of the PSF higher moment residual fields measured from all six HSC PDR1 fields combined  
%     (blue dots), the ``round-trip transformation'' of the original correlation functions 
%     (orange curve), and the PSF moments residual correlation functions 
%     of the generated GRF. The upper panel shows the `$g_1$ group' moments, and the lower panel shows the `$g_2$ group' moments that we defined in Section~\ref{sec:mtd:moment_reduction}. 
%     The 2PCFs of the GRFs generally match those in the HSC data, except at angular scales $\le 1.7$ arcmin, corresponding to the scale of the \textsc{HEALPix} grid. 
%     \label{fig:generated_map}}
% \end{figure*}



% In Fig.~\ref{fig:generated_map}, 
% we show the correlation functions of the PSF higher moment residual maps, described in Eq.~\eqref{eq:moment_2pcf}, of the two groups of moments that determine the additive shear biases, defined in Section~\ref{sec:res:prelim}. These two groups of PSF higher moments are later used to propagate PSF higher moment error to the cosmoDC2 galaxies in Section~\ref{sec:res:dc2}. 
% The blue dots are the measurements based on the HSC bright stars and \textsc{PSFEx} in Section~\ref{sec:res:real_data}. 

% We have devised empirical fitting formulae to describe the measurements of the correlation functions shown as blue dots.  We fit the `$g_1$ group' correlation functions with a power-arctan function,
% \begin{equation}
%     \xi_{\text{fit}}(\theta) = a \theta^{-b} \left[\frac{1}{2}- \frac{ \text{tan}^{-1}(\theta - \theta_\text{cutoff})}{\pi} \right].
% \end{equation}
% This model is chosen because the correlation function takes the form of a power law on small scales (or a linear function when plotted on a log-log plot), and then rapidly drops to zero. The part in the parenthesis is designed to produce the rapid drop to zero on scales beyond  $\theta_\text{cutoff} = 1.7$~\deg, a scale that is comparable to the size of the Subaru FOV.  For the `$g_2$ group' correlation functions, we use a power law, 
% \begin{equation}
%     \xi_{\text{fit}}(\theta) = a \theta^{-b},
% \end{equation}
% as correlation functions in the `$g_2$ group' moments are visually consistent with a power law.


% Since the cosmoDC2 catalog has an area larger than any field in the HSC data we measure, we need to generate artificial PSF moment residual maps to cover the cosmoDC2 area.  We convert the above fitting functions to angular power spectra by carrying out a Hankel transform, using \textsc{SkyLens}\footnote{\url{https://github.com/sukhdeep2/Skylens\_public/tree/imaster\_paper/}} \citep{2021MNRAS.508.1632S}, 
% and use the power spectra to generate artificial Gaussian Random Fields (GRF) using \textsc{Healpy} \citep{Zonca2019,2005ApJ...622..759G}. 
% To ensure the integration is stable and bug-free, we do a round-trip transformation test, where we transform the power spectrum back to real space, shown in the orange curves in Fig.~\ref{fig:generated_map}. The round-trip transformations match the original data well in all cases, as a validation of the fitting function and the numerical accuracy of these transformations. The GRF is generated on the \textsc{HEALPix} sphere with $N_{\text{side}} = 2048$, with a pixel size $\sim 1.7$ arcmin. We measure the correlation function of the GRF, shown as the green curves in Fig.~\ref{fig:generated_map}. Except for the angular bins that are below the resolution of the \textsc{HEALPix} grid,  
% the GRF is shown to match the original field well in terms of the two-point statistics. 

% \label{LastPage}


% \end{document}





















